Checkpoint-based rollback recovery in session programming

To react to unforeseen circumstances or amend abnormal situations in communication-centric systems, programmers are in charge of "undoing" the interactions which led to an undesired state. To assist this task, session-based languages can be endowed with reversibility mechanisms. In this paper we propose a language enriched with programming facilities to commit session interactions, to roll back the computation to a previous commit point, and to abort the session. Rollbacks in our language always bring the system to previous visited states and a rollback cannot bring the system back to a point prior to the last commit. Programmers are relieved from the burden of ensuring that a rollback never restores a checkpoint imposed by a session participant different from the rollback requester. Such undesired situations are prevented at design-time (statically) by relying on a decidable compliance check at the type level, implemented in MAUDE. We show that the language satisfies error-freedom and progress of a session.

==> tex/add_rules.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex

\section{Omitted Rules}
\label{app:omitted}
For reviewers' convenience, we report in this appendix those rules that have been
omitted in the paper. 

The omitted operational rules of the auxiliary labelled relation $\auxrel{\actionLab}$
are in Fig.~\ref{fig:semantics_cherry_pi_aux_omitted}.
\begin{figure*}[!h]
	\centering
	\small
	\begin{tabular}{l@{\ \ }l@{\qquad\quad}l@{\ \ }l@{\ }l}
	%\\[-.7cm]
%	$\sendAct{k}{e}{P} \auxrel{\send{k}{v}} P$
%	\quad $\expreval{e}{v}$ 
%	& \rulelabel{P-Snd}
%	&
%	$\receiveAct{k}{x:S}{P} \auxrel{\receive{k}{x}} P$
%	& \rulelabel{P-Rec}
%	\\[.3cm]
%	$\selectAct{{k}}{l}{P} \auxrel{\select{k}{l}} P$
%	& \rulelabel{P-Sel}
%	&
%	$\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}
%	\auxrel{\branching{k}l_i} P_i$
%	\quad ($1 \leq i \leq n$) 
%	& \rulelabel{P-Brn}
%	\\[.3cm]
		$
	\infer{P_1 \ \auxrel{\actionLab}\ P_2}
	{P_1 \congr P_1'\ \auxrel{\actionLab}\ P_2' \congr P_2}
	$
	& \raisebox{.4cm}{\rulelabel{P-Str}}
	&
	\raisebox{.4cm}{
%	\begin{tabular}{l}
%	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_1$
%	\quad ($\expreval{e}{\ctrue}$) 
%	\\[.3cm]
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_2$ 
	\quad ($\expreval{e}{\cfalse}$) 
%	\end{tabular}
	}
	&
	\raisebox{.4cm}{
%	\begin{tabular}{@{\!}l}
%	\rulelabel{P-IfT} 
%	\\[.3cm]
	\rulelabel{P-IfF}
%	\end{tabular}
}
%	\\[.2cm]
%	\multicolumn{4}{l}{
%	$\commitAct{P} \auxrel{\commitLab} P$ 
%	\ \ \rulelabel{P-Cmt}
%	\qquad\qquad\quad
%	$\roll \auxrel{\rollLab} \inact$ 
%	\ \ \rulelabel{P-Rll}
%	\qquad\qquad\quad
%	$\abort \auxrel{\abortLab} \inact$ 
%	\ \  \rulelabel{P-Abt}}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: auxiliary labelled relation (omitted rules)}
	\label{fig:semantics_cherry_pi_aux_omitted}
	%\vspace*{-.1cm}	
\end{figure*}



The omitted rules defining the typing system for \cherry\ processes and expressions
are given in Fig.~\ref{fig:typingSystem_proc_omitted} and \ref{fig:typingSystem_exp_omitted}. 
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
	$
	\infer[$\rulelabel{T-Sel}$]{\basis;\sorting \judge \selectAct{x}{l}{P} \hasType 
	x:\selType{l}.\typeT}
	{\basis;\sorting  \judge P \hasType x:\typeT}
	$        
	\\[.2cm]			
	$
	\infer[$\rulelabel{T-Br}$]{\basis;\sorting \judge \branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType 
	x:\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}}
	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
	$\\
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Typing System for \cherry\ processes (omitted rules)}
	\label{fig:typingSystem_proc_omitted}
\end{figure}
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}r@{\qquad}r@{}}
	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{tt}}$}
	&
	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{ff}}$}
	\\[.4cm]	
	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{T-Int}	
	&
	$\sorting \judge\!\!``a" \hasType \strType$\ \ \rulelabel{T-Str}	
%	\qquad\qquad
%	$\sorting\comp x:S \judge x \hasType S$\ \ \rulelabel{T-Var}	
	\\[.4cm]
	$
	\infer[$\rulelabel{T-Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
	{\sorting \judge e_1 \hasType \intType & & \sorting \judge e_2 \hasType \intType}
	$
	&
	$
	\infer[$\rulelabel{T-And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
	{\sorting \judge e_1 \hasType \boolType & & \sorting \judge e_2 \hasType \boolType}
	$		
        \\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Typing system for \cherry\ expressions (excerpt of omitted rules)}
	%\vspace*{-.5cm}
	\label{fig:typingSystem_exp_omitted}
\end{figure}


The omitted rules defining the semantics of types and type configurations are given in Fig.~\ref{fig:typeSemantics_ext_omitted} (symmetric rules for configurations are omitted).
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}r@{\hspace*{-.7cm}}r@{\hspace*{-.7cm}}r@{}}
	$\outType{S}.\typeT \typeTrans{\outType{S}} \typeT$\ \ \rulelabel{TS-Snd}	
	&
	$\inpType{S}.\typeT \typeTrans{\inpType{S}} \typeT$\ \ \rulelabel{TS-Rcv}  
	&
	$\selType{l}.\typeT \typeTrans{\selTypeLabel{l}} \typeT$\ \ \rulelabel{TS-Sel}
	\\[.3cm]
	\multicolumn{2}{l}{
	\qquad
	\raisebox{.6cm}{$
	\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}
	\typeTrans{\branchTypeLabel{l_i}} \typeT_i$ \quad $(1 \leq i \leq n)$\ \ \ \ \rulelabel{TS-Br}
	\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!	}
	}
	&
	$
	\infer[$\rulelabel{TS-rec}$]
	{\recType{t}.\typeT \typeTrans{\typeLab} \typeT'}
	{\typeT\subst{\recType{t}.\typeT}{t} \typeTrans{\typeLab} \typeT'}
	$
\\[-.3cm]
	$
	\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_1$\ \ \rulelabel{TS-If$_1$}
	&
	$\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_2$\ \ \rulelabel{TS-If$_2$}
	&
%		\\[.3cm]
%	$\commitType.\typeT \typeTrans{\commitType} \typeT$\ \ \rulelabel{TS-Cmt}
%	&
%	$\rollType \typeTrans{\rollType} \inactType$\ \ \rulelabel{TS-Rll}
%	&
%	$\abortType \typeTrans{\abortType} \inactType$\ \ \rulelabel{TS-Abt}
	\\
	\\
%	\multicolumn{3}{@{}l@{}}{	
%	$
%	{\typeT_1 \typeTrans{\tau} \typeT_1'}
%	\Rightarrow	
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	\quad $\rulelabel{TS-Tau}$
%	$	
%	}\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\!\outType{S}\!} \typeT_1'
%	\, ,\,
%	 \typeT_2 \typeTrans{\!\!\inpType{S}\!} \typeT_2'}	
%	\Rightarrow		
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	\ \ $\rulelabel{TS-Com}$
%	$	
%	}\\
%	\\
	\multicolumn{3}{@{}l@{}}{
	$
	{\typeT_1 \typeTrans{\selTypeLabel{l}} \typeT_1'
	\, , \,
	 \typeT_2 \typeTrans{\branchTypeLabel{l}} \typeT_2'}
	\Rightarrow 
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
	\ \ $\rulelabel{TS-Lab}$
	$	
	}
%	\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\commitType} \typeT_1' \, , \, \checkpointType{\typeU}_2 \neq \typeT_2}
%	\Rightarrow	
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%	\ \ \ $\rulelabel{TS-Cmt$_1$}$
%	$	
%	}\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\commitType} \typeT_1' \, ,\, \checkpointType{\typeU}_2 = \typeT_2}
%	\Rightarrow
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	\ \ \ $\rulelabel{TS-Cmt$_2$}$
%	$	
%	}\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\rollType} \typeT_1'}
%	\Rightarrow
%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeU_2}}
%	\quad $\rulelabel{TS-Rll$_1$}$
%	$	
%	}\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\abortType} \typeT_1'}
%	\Rightarrow
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT}{\typeT} \confcomp \conf{\typeT'}{\typeT'}}
%	\quad $\rulelabel{TS-Abt$_1$}$
%	$	
%	}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Semantics of types and type configurations (omitted rules)}
	\label{fig:typeSemantics_ext_omitted}
	%\vspace*{-.5cm}
\end{figure}




The omitted rules defining the error semantics are given 
in Fig.~\ref{tab:error_red_omitted}.
%
The semantics of \cherry\ is extended by the additional rules, 
where \rulelabel{E-Cmt$_1$} and \rulelabel{E-Cmt$_2$} replace \rulelabel{F-Cmt},
and \rulelabel{E-Rll$_1$} replaces  \rulelabel{B-Rll},
and $\checkpointType{\ }$ is used in the checkpoints of the other rules.
%
The definition of these rules relies  on the notion of \emph{barb} predicates, whose straightforward 
definition is: 
$P\Barb{\mu}$ holds if there exists $P'$ such that $P \Rightarrow P'$ and 
$P'$ can perform an action $\mu$, 
where $\mu$ stands for $k?$, $k!$ ,$k\triangleleft l$ or $k\triangleright l$
(i.e., input, output, select and branching action along session channel $k$);
$\Rightarrow$ is the reflexive and transitive closure of $\auxrel{\ite}$.
\begin{figure*}[!h]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
%	$
%	\infer[$\!\rulelabel{E-Com1}$]{
%	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred
%	\comError
%	}
%	{
%	P_1 \auxrel{\send{{k}}{v}} P_1'
%	\qquad
%	\neg P_2 \BarbInp{k}
%	}
%	$	
%	\qquad
%	$
%	\infer[$\!\rulelabel{E-Com2}$]{
%	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\comError
%	}
%	{
%	P_1 \auxrel{\receive{{k}}{x}} P_1'
%	\qquad
%	\neg P_2 \BarbOut{k}
%	}
%	$	
%		\\[.3cm]	
	$
	\infer[$\!\rulelabel{E-Lab$_1$}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\select{{k}}{l}} P_1'
	\qquad
	\neg P_2\BarbBranching{k}{l}
	}
	$			
	\qquad\
	$
	\infer[$\!\rulelabel{E-Lab$_2$}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\branching{k}l} P_1'
	\qquad
	\neg P_2\BarbSelect{k}{l}
	}
	$
		\\[.3cm]	
	$
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\imposed{P_2}} P_2
	}
	{\hspace*{.8cm}
	P_1 \auxrel{\commitLab} P_1'
	\qquad 
	\checkpointType{Q_2} \neq P_2
	\hspace*{.8cm}
	$\rulelabel{E-Cmt$_1$}$
	}
	$	
	\qquad
	$
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	}
	{\hspace*{.8cm}
	P_1 \auxrel{\commitLab} P_1'
	\qquad 
	\checkpointType{Q_2} = P_2
	\hspace*{.8cm}
	$\rulelabel{E-Cmt$_2$}$
	}
	$	
		\\[.3cm]	
	%\hspace*{-1.5cm}
	$
	\infer{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\bwred
	\logged{\ce{\genSession}}{Q_1} Q_1
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} Q_2
	}
	{	\hspace*{2.1cm}
	P_1 \auxrel{\rollLab} P_1'
		\hspace*{1.9cm}
	$\rulelabel{E-Rll$_1$}$
	}
	$	
	\qquad	
%	$
%	\infer{
%	\logged{\ce{\genSession}}{\imposed{Q_1}} P_1 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\rollError
%	}
%	{\hspace*{1.4cm}
%	P_1 \auxrel{\rollLab} P_1'
%	\hspace*{1.2cm}
%	$\,\rulelabel{E-Rll$_2$}$
%	}
%	$	
	$
	\infer[$\!\rulelabel{E-Com$_2$}$]{
	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\comError
	}
	{
	P_1 \auxrel{\receive{{k}}{x}} P_1'
	\qquad
	\neg P_2 \BarbOut{k}
	}
	$	
	\\[.1cm]
	\hline
	\end{tabular}	
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: error reductions  (omitted rules)}
	\label{tab:error_red_omitted}
	%\vspace*{-.5cm}
\end{figure*}



\newpage
%%%%%%%%%%%%%%%%%%%% MULTIPARTY
The omitted syntax of multiparty \cherry\ and of multiparty session types 
are in Fig.~\ref{fig:syntax_cherry_pi_multi_omitted} and~\ref{fig:typeSyntax_cherry_multi_omitted},
respectively.
\begin{figure}[!h]
\small
	\begin{tabular}{@{}r@{ }c@{\ \ }l@{\ \ \ }l@{}}
	$C$ & ::= & $\cdots$   \ $\mid$ \
	                   $\mrequestAct{a}{\role{p}}{x}{P}$ \ $\mid$ \ $\macceptAct{a}{\role{p}}{x}{P}$
	                   & \textbf{Collaborations}
	\\[.2cm]
	$P$ & ::= &  $\cdots$  \ $\mid$ \
                                        $\msendAct{\sessId}{\role{p}}{e}{P}$ 
		         $\mid$ \ $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ 	
		         $\mid$ \ $\mselectAct{\sessId}{\role{p}}{l}{P}$ 
		         $\mid$ \ $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
			& \textbf{Processes}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}	
	\caption{Multiparty \cherry\ runtime syntax (the omitted parts are as in Fig.~\ref{fig:syntax_cherry_pi_ext}).}
%	\vspace*{-.5cm}	
	\label{fig:syntax_cherry_pi_multi_omitted}
\end{figure}
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
	$\typeT$ & ::= &  &  \ldots \  $\mid$  \
	$\moutType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
	$\minpType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	 \   $\mid$ \ 
	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$
	\quad \textbf{Session types}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.5cm}	
	\caption{Multiparty \Cherry\ type syntax 
	(the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry}).
	}
	\label{fig:typeSyntax_cherry_multi_omitted}
	%\vspace*{-.5cm}
\end{figure}

Finally, the omitted rules of the multiparty type configurations semantics are reported in 
Fig.~\ref{fig:typeSemantics_ext_multi_omitted}.
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}l@{\qquad}l@{}}
	$\moutType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Snd}	
	&
	$\minpType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\minpType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Rcv}  
	\\[.3cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
	\, ,\,
	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\ \qquad \quad
	\typered
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i'} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j'}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\end{array}
	$
	\
	 $i,j\in I$
	\quad
	\rulelabel{M-TS-Com}
	}
	\\[.6cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\commitLab} \typeT_i'
	 }	
	 \quad
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\ \qquad \quad	
	\typered
	\minitConf{\typeT^I}
	\conf{\typeT_i'}{\typeT_i'} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h}
	\end{array}
	$
	 $i\in I$
	 \ , \
	 $
	 \checkpointType{\typeU}_h' \! =\!\! 
	 \left\{
	 \begin{array}{ll}
	 \checkpointType{\typeU}_h & \textrm{if}\ \checkpointType{\typeU}_h = \typeT_h \\[-.1cm]
	 \imposed{\typeT_h} & \textrm{otherwise}
	 \end{array}
	 \right.
	 $
	\quad
	\rulelabel{M-TS-Cmt}
	}
	\\[.6cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\rollLab} \typeT_i'
	 }	
	 \quad
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\typered
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeU_i}  
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeU_h}
	\end{array}
	$
	 $i\in I$	 
	\quad
	\rulelabel{M-TS-Rll}
	}
	\\[.5cm]	
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\abortLab} \typeT_i'
	 }	
	 \ \
	\Rightarrow
	%\\		
	\ \
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\typered
	\minitConf{\typeT^I}
	\prod_{k\in I}\conf{\typeT^k}{\typeT^k}
	\end{array}
	$
	 $i\in I$	 
	\ \
	\rulelabel{M-TS-Abt}
	}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Semantics of multiparty type configurations 
	(excerpt of rules, where $I=\{1,\ldots,n\}$).}
	\label{fig:typeSemantics_ext_multi_omitted}
	\vspace*{-.5cm}
\end{figure}

==> tex/binary_calculus_LONG.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex
\section{The \cherry\ calculus}\label{sec:cherry}

In this section, we introduce \cherry, 
%(\underline{che}ckpoint-based \underline{r}ollback \underline{r}ecover\underline{y} binary session \underline{pi}-calculus), 
a calculus (extending that in~\cite{YoshidaV07}) devised for studying 
sessions equipped with our checkpoint-based rollback recovery mechanism.

\myparagraph{Syntax}
The syntax of the \cherry\ calculus relies on the following base sets: 
\emph{shared channels} (ranged over by $a$), used to initiate sessions;
\emph{session channels} (ranged over by $s$), consisting of pairs of \emph{endpoints} 
(ranged over by $s$, $\ce{s}$) used by the two parties to interact within an established session;
\emph{labels} (ranged over by $l$), used to select and offer branching choices;
\emph{values} (ranged over by $v$), including booleans, integers and strings
(whose \emph{sorts}, ranged over by $S$, are $\boolType$, $\intType$ and $\strType$, respectively), 
which are exchanged within a session; 
\emph{variables} (ranged over by $x$, $y$, $z$), storing values and session endpoints;
 \emph{process variables} (ranged over by $X$), used for recursion. 
%Letter $\genSession$ denotes \emph{generic session endpoints}, i.e. they can be either of 
%the form $s$ or $\ce{s}$; 
%letter $\sessId$ denotes \emph{session identifiers}, i.e. session endpoints and variables together.
%%letter $c$ denotes \emph{channels}, i.e. session channels and shared channels together. 


\Cherry\ specifications, called \emph{collaborations} and ranged over by $C$, 
are given by the grammar in Fig.~\ref{fig:syntax_cherry_pi}. 
%
The key ingredient of the calculus is the set of actions for controlling the session rollback. 
Actions $\commit$, $\roll$ and $\abort$ are used, respectively, to commit a session 
(producing a checkpoint for each session participant), 
to trigger the session rollback (restoring the last committed checkpoints) 
or to abort the whole session. We discuss below the other constructs of the calculus, 
which are those typically used for session-based programming \cite{HondaVK98}.  

A \cherry\ collaboration is a collection of \emph{session initiators}, i.e. terms ready to initiate sessions 
by synchronising on shared channels.
A synchronisation of two initiators $\requestAct{a}{x}{P}$ and $\acceptAct{a}{y}{Q}$
causes the generation of a fresh session channel, whose endpoints replace 
variables $x$ and $y$ in order to be used by the triggered processes $P$ and $Q$, 
respectively, for later communications. No subordinate sessions can be initiated within a running session.

\begin{figure}[t]
\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ \ }l@{}}
	\\[-.7cm]	
	$C$ & ::= & & \textbf{Collaborations} \\
	&             & $\requestAct{a}{x}{P}$ \ $\mid$ \ $ \acceptAct{a}{x}{P}$ 
	                   \ $\mid$ \
	                   $C_1 \!\mid\! C_2$ 
	                   & \ request, accept, parallel
	\\[.1cm]
	$P$ & ::= & & \textbf{Processes} \\
	&             & $\sendAct{x}{e}{P}$ 
		        \ $\mid$ \ $\receiveAct{x}{y:S}{P}$ 
		        \ $\mid$ \ $\selectAct{x}{l}{P}$ 
		        \ $\mid$ \ $ \branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ 
			& \ output, input, selection, branching
	\\
	& $\mid$ & $\ifthenelseAct{e}{P_1}{P_2}$ 
	                   \ $\mid$ \ $X$ 
	                   \ $\mid$ \ $\recAct{X}{P}$
	                   \ $\mid$ \ $\inact$
	                   & \ choice, recursion, inact 
	\\
	& $\mid$ &  $\commitAct{P}$
	\ $\mid$ \ $\roll$
	\ $\mid$ \ $\abort$  
        & \ commit, roll, abort                   
	\\[.1cm]	
	$e$ & ::= &\ \  $v$ \ $\mid$ \ $+(e_1,e_2)$ \ $\mid$ \ $\wedge(e_1,e_2)$ \ $\mid$ \ \ldots  
	& \textbf{Expressions} 
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{\Cherry\ syntax.}
	\label{fig:syntax_cherry_pi}
\vspace{-6mm}
\end{figure}

When a session is started, each participant executes a \emph{process}. Processes are built up from the  process $\inact$, which does nothing, and from basic actions by means of 
action prefix $\_\,.\,\_\,$,
conditional choice $\ifthenelseAct{e}{\_}{\_}$, 
and recursion $\recAct{X}{\_}$.
Actions $\send{x}{e}$ and \mbox{$\receive{y}{z:S}$}  denote output and input 
via session endpoints replacing $x$ and $y$, respectively. 
These communication primitives realise the standard synchronous 
message passing, where messages result from the evaluation of \emph{expressions},
which are defined by means of standard operators on boolean, integer and string values.
Variables that are arguments of input actions are (statically) typed by sorts. 
%Statically typing the variables occurring as arguments of session initiating actions is instead not necessary, as they are always 
%replaced by session endpoints. 
There is no need for statically typing the variables occurring as arguments of session initiating actions, as they are always 
replaced by session endpoints. 
Notice that in \cherry\ the exchanged values cannot be endpoints, 
%as session delegation (i.e., channel-passing) is disallowed in the single session setting. 
meaning that session delegation (i.e., channel-passing) is not considered. 
%
Actions $\select{x}{l}$ and $\branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ denote selection and branching (where $l_1$, \ldots, $l_n$ are pairwise distinct). 
%They mime method invocation in object-based programming.
%
%Finally, actions $\commit$, $\roll$ and $\abort$  are used, respectively, to irreversibly commit a session (producing a checkpoint for each session participant), 
%to trigger the session rollback (restoring the last committed checkpoints) 
%or to abort the whole session.
\vspace*{-.1cm}

\begin{example}\label{example_syntax}
Let us consider the VOD example informally introduced in \S~\ref{sec:motivating_example}.
The scenario described in Fig.~\ref{fig:scenario}(a) with commit actions placed as in 
Fig.~\ref{fig:scenario}(b) is rendered in \cherry\ as
$
C_{\texttt{US}} \ = \ \requestPrefix{login}{x}.\ P_\texttt{U} \ \mid\ \acceptPrefix{login}{y}.\ P_\texttt{S}
$
where:\\[1mm]
$
\begin{array}{r@{\ \ }c@{ \ \ }l}
P_\texttt{U} & = & 
\sendAct{x}{v_{\textit{\textsf{req}}}}{\,}
\receiveAct{x}{x_{\textsf{\textit{price}}}:\intType}{\,}
\commitAct{\,}
\receiveAct{x}{x_{\textit{\textsf{meta}}}:\strType}{\,}
\ifPi\
(f_{\textit{\textsf{eval}}}(x_{\textit{\textsf{price}}},x_{\textit{\textsf{meta}}}))
\\
&&
\quad
\thenPi\ \selectAct{{x}}{l_{\textit{\textsf{HD}}}}{\,}
\receiveAct{x}{x_{\textit{\textsf{testHD}}}:\strType}{\,}
(\ifPi\ (f_{\textit{\textsf{HD}}}(x_{\textit{\textsf{testHD}}}))\ \thenPi\ \receiveAct{x}{x_{\textit{\textsf{videoHD}}}:\strType}{\inact}\ \elsePi\ \roll)
\\
&&
\quad
\elsePi\ \selectAct{{x}}{l_{\textit{\textsf{SD}}}}{\,}
\receiveAct{x}{x_{\textit{\textsf{testSD}}}:\strType}{\,}\
(\ifPi\ (f_{\textit{\textsf{SD}}}(x_{\textit{\textsf{testSD}}}))\ \thenPi\ \receiveAct{x}{x_{\textit{\textsf{videoSD}}}:\strType}{\inact}\ \elsePi\ \abort)
\end{array}
$\\[1mm]
\noindent
$
\begin{array}{r@{\ \ }c@{ \ \ }l}
P_\texttt{S} & = & 
\receiveAct{y}{y_{\textit{\textsf{req}}}:\strType}{\,}
\sendAct{y}{f_{\textit{\textsf{price}}}(y_{\textit{\textsf{req}}})}{\,}
\sendAct{y}{f_{\textit{\textsf{meta}}}(y_{\textit{\textsf{req}}})}{\,}
\\
&&
\branchAct{y}{\
\branch{l_{\textit{\textsf{HD}}}\!}{\!\commitAct{\,}
\sendAct{y}{f_{\textit{\textsf{testHD}}}(y_{\textit{\textsf{req}}})}{\,}
\sendAct{y}{f_{\textit{\textsf{videoHD}}}(y_{\textit{\textsf{req}}})}{\,}
\inact}
\ \branchSep \\
&&
\qquad\ \
\branch{l_{\textit{\textsf{SD}}}\!}{\!\commitAct{\,}
\sendAct{y}{f_{\textit{\textsf{testSD}}}(y_{\textit{\textsf{req}}})}{\,}
\sendAct{y}{f_{\textit{\textsf{videoSD}}}(y_{\textit{\textsf{req}}})}{\,}
\inact}\
}
\end{array}
$
\\[1mm]
Note that expressions used for decisions and computations are abstracted by 
%means of unspecified 
functions $f_{\textit{\textsf{n}}}(\cdot)$.

Considering the placement of commit actions depicted in Fig.~\ref{fig:scenario}(c), 
the \cherry\ specification of the service's process becomes:\\[1mm]
$
\begin{array}{l}
\receiveAct{y}{y_{\textit{\textsf{req}}}:\strType}{\,}
\sendAct{y}{f_{\textit{\textsf{price}}}(y_{\textit{\textsf{req}}})}{\,}
\commitAct{\,}
\sendAct{y}{f_{\textit{\textsf{meta}}}(y_{\textit{\textsf{req}}})}{\,}
\\
\branchAct{y}{\
\branch{l_{\textit{\textsf{HD}}}\!}{\!
\sendAct{y}{f_{\textit{\textsf{testHD}}}(y_{\textit{\textsf{req}}})}{\,}
\sendAct{y}{f_{\textit{\textsf{videoHD}}}(y_{\textit{\textsf{req}}})}{\,}
\inact}
\ \branchSep \
\branch{l_{\textit{\textsf{SD}}}\!}{\!
\sendAct{y}{f_{\textit{\textsf{testSD}}}(y_{\textit{\textsf{req}}})}{\,}
\sendAct{y}{f_{\textit{\textsf{videoSD}}}(y_{\textit{\textsf{req}}})}{\,}
\inact}\
}
\end{array}
$

Finally, considering the placement of commit actions depicted in Fig.~\ref{fig:scenario}(d), 
the \cherry\ specification of the user's process becomes:\\[1mm]
$
\begin{array}{l}
\sendAct{x}{v_{\textit{\textsf{req}}}}{\,}
\receiveAct{x}{x_{\textsf{\textit{price}}}:\intType}{\,}
\receiveAct{x}{x_{\textit{\textsf{meta}}}:\strType}{\,}
\commitAct{\,}
\ifPi\ (f_{\textit{\textsf{eval}}}(x_{\textit{\textsf{price}}},x_{\textit{\textsf{meta}}}))\
\thenPi\ \ldots
\end{array}
$
\end{example}



\vspace*{-.1cm}	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myparagraph{Semantics}
The operational semantics of \cherry\ is defined for \emph{runtime} terms, generated by the extended syntax of the calculus in Fig.~\ref{fig:syntax_cherry_pi_ext} (where the new constructs are highlighted by a grey 
background).
%
We use $\genSession$ to denote \emph{generic session endpoints}
($s$ or $\ce{s}$); and
$\sessId$ to denote \emph{session identifiers}, i.e. session endpoints and variables together.
%and $c$ to denote \emph{channels}, i.e. session channels and shared channels together. 
%As a matter of terminology, we 
We refer as \emph{initial collaborations} to those runtime terms that 
can be also generated by the grammar in Fig.~\ref{fig:syntax_cherry_pi}. 


At collaboration level, two constructs are introduced:
\mbox{$\singleSession{s}{C_1}\ C_2$ } represents a \emph{session} along the channel $s$ 
with associated starting checkpoint $C_1$ (corresponding to the collaboration that has initialised the session)
and code $C_2$; construct \mbox{$\logged{\genSession}{P_1}P_2$} represents a \emph{log}
%\todo{{\scriptsize FT: ho tolto la $k$ dal log, perch\'e non mi sembrava necessario associare un endpoint al
%logged process. Infatti  i logged processes $\logged{}{\ce{s}:Q_1} P_1 \mid  \logged{}{s :Q_2} P_2$  possono stare solo dentro lo scope di $\singleSession{s}{P}$, che non \`e estendibile. Quindi considerando solo reachable processes, non posso mai accoppiare logged processes di sessioni diverse, come ad esempio $\logged{}{\ce{s}:Q_1} P_1 \mid  \logged{}{s' :Q_2} P_2$. Che dici?}}
%identified by the session endpoint $\genSession$, 
storing the checkpoint $P_1$ associated to the code $P_2$.
%
At process level, the only difference is that session identifiers $\sessId$ are used as first argument of communicating actions.  

\begin{figure}[t]
\small
	\begin{tabular}{@{}r@{ }c@{\!\!\!\!\!\! }l@{\ }l@{}}
	\\[-.7cm]	
	$C$ & ::= & & \textbf{Collaborations} \\
	&             & $\requestAct{a}{x}{P}$ \ $\mid$ \ $ \acceptAct{a}{x}{P}$ 
	                   \ $\mid$ \
	                   $C_1 \!\mid\! C_2$ 
	                   \ $\mid$ \
	                   \graybox{$\singleSession{s}{C_1}\ C_2$}
	                   \ $\mid$ \ \graybox{$\logged{\genSession}{P_1}P_2$}    	                   
	                   & \ request, accept, parallel, session, log
	\\[.1cm]
	$P$ & ::= & & \textbf{Processes} \\
	&             & $\sendAct{\gb{\sessId\!}}{e}{P}$
		         $\mid$ \ $\receiveAct{\gb{\sessId\!}}{y:S}{P}$	
		         $\mid$ \ $\selectAct{\gb{\sessId\!}\!}{l}{P}$ 
		         $\mid$ \ $\branchAct{\gb{\sessId\!}\!}{\branch{l_1\!\!}{\!\!P_1} 
		                          \branchSep\! \ldots\! \branchSep
                                          \branch{l_n\!\!}{\!\!P_n}}
                                        \mid \cdots$
			& \ output, input, selection, branching
%	\\
% 	& $\mid$ &  $\commitAct{P}$
% 	\ $\mid$ \ $\roll$
% 	\ $\mid$ \ $\abort$  
%         & \ commit, roll, abort                   
%	\\[.2cm]	
%	$e$ & ::= & $v$ \ $\mid$ \ $+(e_1,e_2)$ \ $\mid$ \ $\wedge(e_1,e_2)$ \ $\mid$ \ \ldots  
%	& \textbf{Expressions} 
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}	
	\caption{\Cherry\ runtime syntax (
The rest of processes $P$ and 
expressions $e$ are as in Fig.~\ref{fig:syntax_cherry_pi}).}
	\vspace*{-.1cm}	
	\label{fig:syntax_cherry_pi_ext}
\end{figure}

%\begin{figure}[t]
%\centering
%\small
%	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ \ }l@{}}
%	$C$ & ::= & & \textbf{Collaborations} \\
%	&             & $\requestAct{a}{x}{P}$ \ $\mid$ \ $ \acceptAct{a}{x}{P}$ 
%	                   \ $\mid$ \
%	                   $C_1 \!\mid\! C_2$ 
%	                   & \ request, accept, parallel
%	                   \\
%	& $\mid$ & \graybox{$\singleSession{s}{C_1}\ C_2$}	        
%	\ $\mid$ \ \graybox{$\logged{\genSession}{P_1}P_2$}    
%	& \ single session, log\\        
%	\\[.2cm]
%	$P$ & ::= & & \textbf{Processes} \\
%	&             & $\sendAct{\gb{\sessId}}{e}{P}$ \ $\mid$ \ $\receiveAct{\gb{\sessId}}{y:S}{P}$ 
%		 	%\ $\mid$ \ $P_1 \!\mid\! P_2$
%		        \ $\mid$ \ $\inact$
%			& \ output, input, inact %, parallel
%	\\
%	& $\mid$ & $\selectAct{\gb{\sessId}}{l}{P}$ \ $\mid$ \ $ \branchAct{\gb{\sessId}}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ 
%	                     & \ selection, branching \\
%	& $\mid$ & %$ \res{c}\, P$ \ $\mid$ \ 
%			  $\ifthenelseAct{e}{P_1}{P_2}$ 
%	                   \ $\mid$ \
%	                   $X$ \ $\mid$ \ $\recAct{X}{P}$ 
%	                   & \ choice, recursion
%	\\
%	& $\mid$ &  $\commitAct{P}$
%	\ $\mid$ \ $\roll$
%	\ $\mid$ \ $\abort$  
%        & \ commit, roll, abort                   
%%	\\[.2cm]	
%%	$e$ & ::= & & \textbf{Expressions} \\
%%	&             & $v$ 
%%	                   \ $\mid$ \
%%	                   $\text{op}(e_1,\ldots,e_n)$ 
%%	                   & \ value, expression operator
%%	\\[.2cm]
%%		$S$ & ::= &  & \textbf{Sorts}\\
%%	&             & $\boolType$ \quad $\mid$ \quad $\intType$ \quad $\mid$ \quad $\strType$ & \ boolean, integer, string
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.2cm}	
%	\caption{\Cherry\ runtime syntax (Expressions $e$ and Sorts $S$ are as in Figure~\ref{fig:syntax_cherry_pi})}
%	\label{fig:syntax_cherry_pi_ext}
%\end{figure}

We extend the standard notion of binders to take into account the operator
\mbox{$\singleSession{s}{C_1}\ C_2$}, which
binds session endpoints $s$ and $\ce{s}$ in $C_2$
(in this respect, it acts similarly to operator $\res s P$ of \pic, but its scope cannot be extended 
in order to avoid involving processes that do not belong to the session in the rollback effect).
%Bindings are defined as follows: 
%$\requestAct{a}{x}{P}$, 
%$ \acceptAct{a}{x}{P}$ 
%and 
%\mbox{$\receiveAct{\sessId}{x:S}{P}$ }
%bind variable $x$ in $P$; 
%\mbox{$\singleSession{s}{C_1}\ C_2$}
%binds session endpoints $s$ and $\ce{s}$ in $C_2$
%(in this respect, it acts similarly to operator $\res s P$ of \pic, but its scope cannot be extended 
%in order to avoid involving processes that do not belong to the session in the rollback effect);
%$\recAct{X}{P}$ binds process variable $X$ in $P$. 
The derived notions of bound and free names (where \emph{names} stand for variables, process variables and session endpoints), alpha-equivalence, and substitution are standard
%For $P$ a process, $fv(P)$ denotes the set of free variables, $fc(P)$ denotes the set of free shared channels, and $fse(P)$ the set of free session endpoints. 
and we assume that bound names are pairwise distinct. 
%This condition is not restrictive and can always be fulfilled by possibly using alpha-conversion.
The semantics of the calculus is defined for \emph{closed} terms, i.e. terms without free 
variables and process variables. 

Not all processes allowed by the extended syntax corresponds to meaningful
collaborations. In a general term the processes stored in logs 
may not be consistent with the computation that has taken place.
%
%We address these issues by only considering a class of well-formed processes, called 
%\emph{reachable} processes. 
%In the definition of this class of processes, 
%to ensure the use of single sessions only, as in \cite{HYCJACM15} we resort to 
%the notion of \emph{simple} process. 
%\begin{definition}[Simple binary process]\label{def:simple}
%A process is \emph{simple} if (i)~it is generated by the grammar in Figure~\ref{fig:syntax_pi} and
%(ii)~it is typable with a type derivation using prefix rules
%where the session typings in the premise and the conclusion are restricted to at most a 
%singleton\footnote{Using the standard typing system for the binary session \pic\ 
%\iftr
%(Figure~\ref{fig:typingSysytem} in Appendix~\ref{app:background}), 
%\else
%(see \cite[Figure~13]{RC_TR}), 
%\fi
%point (ii) boils down to:  $\typing$ of rules 
%\rulelabel{Req}, 
%\rulelabel{Acc},
%\rulelabel{Send},
%\rulelabel{Rcv},
%\rulelabel{Sel}
%and \rulelabel{Br} are empty; 
%neither \rulelabel{Thr} nor \rulelabel{Cat} is used;
%$\typing\comp \typing'$ in \rulelabel{Conc} contains at most a singleton; 
%and $\typing$ of the remaining rules contain at most a singleton.}. 
%\end{definition}
%The point (i) of the above definition states that a simple process has no log, while 
%point (ii) states that each prefixed subterm in a simple process uses only a single session. 
%Notably, in a simple process, delegation and subordinate sessions 
%(i.e., new sessions initialised within the single session) are disallowed.
%
%Now, 
%Therefore, to ensure history consistency, as in~\cite{CristescuKV13} we only consider \emph{reachable} 
%collaborations, i.e. runtime collaborations obtained by means of forward reductions  from 
%static ones. 
%%\todo{FT: non serve piu' la nozione di simple process; infatti adesso si garantisce che le sessioni sono
%%single attraverso la definizione della sintassi con categorie sintattiche separate per collaborations e processes.}
%
%\begin{definition}[Reachable collaborations]\label{def:reachable}
%The set of \emph{reachable} collaborations is the closure under relation $\fwred$ (see below)  
%of the set of collaborations generated by the grammar in Figure~\ref{fig:syntax_cherry_pi}. 
%\end{definition}
%
We get rid of such malformed terms, as we
will only consider those runtime terms, called  \emph{reachable} collaborations, 
obtained by means of reductions from initial collaborations.
% generated by the grammar in Figure~\ref{fig:syntax_cherry_pi}).

%
%Therefore, to ensure history consistency, as in~\cite{CristescuKV13} we only consider \emph{reachable} 
%collaborations, i.e. runtime collaborations obtained by means of forward reductions  from 
%static ones. 
%%\todo{FT: non serve piu' la nozione di simple process; infatti adesso si garantisce che le sessioni sono
%%single attraverso la definizione della sintassi con categorie sintattiche separate per collaborations e processes.}
%
%\begin{definition}[Reachable collaborations]\label{def:reachable}
%The set of \emph{reachable} collaborations is the closure under relation $\fwred$ (see below)  
%of the set of collaborations generated by the grammar in Figure~\ref{fig:syntax_cherry_pi}. 
%\end{definition}


%In the extended calculus,  
In \cherry\ processes can perform, besides usual 
\emph{forward computations}, also  \emph{backward computations} 
that restore the last committed checkpoints, thus undoing the effect of 
forward computations. 
%
The operational semantics is given in terms of a structural congruence and 
a reduction relation. 

The \emph{structural congruence}, written $\congr$, is standard:
the parallel operator is associative and commutative; 
recursion $\recAct{X}{P}$ can be unfolded (i.e., replaced by $P[\recAct{X}{P}/X]$, 
where notation $P[Q/X]$ denotes replacement of free occurrences of $X$ in $P$ by process $Q$);
finally, alpha-equivalent processes, i.e. processes only differing in the identity of bound names,
are equated. 

The \emph{reduction} relation, written $\fwbwred$, 
is given as the union of the corresponding \emph{forward reduction} relation $\fwred$ and \emph{backward reduction} relations $\bwred$.
%%
%The semantics is only defined for closed, reachable terms, 
%where now the definition of \emph{closed} term extends to session endpoints, 
%in the sense that all occurrences of an endpoint $\genSession$
%have to be bound by a log term $\logged{\genSession}{\cdot}\cdot$. 
%%This latter requirement is needed for ensuring that
%%every running session in the considered process can be reverted; 
%%for example, in the reachable process $(\send{\ce{s}}{1}\mid\receive{s}{x} \mid Q)$
%%there is a running session $s$ that cannot be reverted because no computation history 
%%information (i.e., no log) is available for it. 
%
%We resort to the auxiliary function $\expreval{\cdot}{\,}$ 
%for evaluating closed expressions: 
%$\expreval{e}{v}$ says that expression $e$ evaluates to value $v$. 
%Notationally, for $P$ a process, $\freev{P}$ denotes the set of free variables in $P$, 
%and $\freese{P}$ the set of free session endpoints. 
The definition of the forward reduction relation $\fwred$ over closed %reachable 
collaborations relies on an auxiliary labelled relation $\auxrel{\actionLab}$ over processes that specifies %\emph{commitments}, i.e. 
the actions that processes can initially perform and the continuation process obtained after each such action. 
The notation of the above relations is summarised in Fig.~\ref{fig:relations}.
%
\begin{figure*}[t]
	\small
	\begin{tabular}{l@{\ \ }l@{\qquad}l}
	$\fwred$ & Forward reduction over collaborations
	&
	$\fwbwred =\! (\fwred \cup \bwred)$  Reduction over collaborations
	\\%[.1cm]
	$\bwred$ & Backward reduction over collaborations
        &
        $\auxrel{\actionLab}$  Auxiliary relation labelled by actions over processes
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{\cherry\ reduction relations}
	\label{fig:relations}
	\vspace*{-.7cm}	
\end{figure*}
%
Given a reduction relation $\mathcal{R}$, we will indicate with  $\mathcal{R}^{+}$ and  
$\mathcal{R}^{*}$ respectively the \textit{transitive} and the \textit{reflexive-transitive} closure of $\mathcal{R}$.
%
The operational rules defining the auxiliary labelled relation are reported in Fig.~\ref{fig:semantics_cherry_pi_aux} (omitted rules are in Appendix~\ref{app:omitted}), 
where action label $\actionLab$ stands for either 
$\send{k}{v}$,
$\receive{k}{x}$,
$\select{k}{l}$,
$\branching{k}l$, 
$\commitLab$,
$\rollLab$,
$\abortLab$,
or $\ite$.
%
The meaning of these rules is straightforward, as they just produce as labels the actions currently 
enabled in the process. In doing that, expressions of sending actions and conditional choices are 
evaluated (the auxiliary function $\expreval{e}{v}$ says that closed expression $e$ evaluates to 
value $v$). 
%Notably, since we are considering the single session setting, connecting actions, 
%i.e. request and accept, are dealt with as the inaction, that is no rule is provided for them.

\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{l@{\ \ }l@{\qquad\quad}l@{\ \ }l@{\ }l}
	\\[-.7cm]
	$\sendAct{k}{e}{P} \auxrel{\send{k}{v}} P$
	\quad $\expreval{e}{v}$ 
	& \rulelabel{P-Snd}
	&
	$\receiveAct{k}{x:S}{P} \auxrel{\receive{k}{x}} P$
	& \rulelabel{P-Rec}
	\\[.3cm]
	$\selectAct{{k}}{l}{P} \auxrel{\select{k}{l}} P$
	& \rulelabel{P-Sel}
	&
	$\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}
	\auxrel{\branching{k}l_i} P_i$
	\quad ($1 \leq i \leq n$) 
	& \rulelabel{P-Brn}
	\\[.3cm]
		$
	\infer{P_1 \ \auxrel{\actionLab}\ P_2}
	{P_1 \congr P_1'\ \auxrel{\actionLab}\ P_2' \congr P_2}
	$
	& \raisebox{.4cm}{\rulelabel{P-Str}}
	&
	\raisebox{.4cm}{
	\begin{tabular}{l}
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_1$
	\quad ($\expreval{e}{\ctrue}$) 
	\\[.3cm]
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_2$ 
	\quad ($\expreval{e}{\cfalse}$) 
	\end{tabular}
	}
	&
	\raisebox{.4cm}{
	\begin{tabular}{@{\!}l}
	\rulelabel{P-IfT} 
	\\[.3cm]
	\rulelabel{P-IfF}
	\end{tabular}}
	\\[.2cm]
	\multicolumn{4}{l}{
	$\commitAct{P} \auxrel{\commitLab} P$ 
	\ \ \rulelabel{P-Cmt}
	\qquad\qquad\quad
	$\roll \auxrel{\rollLab} \inact$ 
	\ \ \rulelabel{P-Rll}
	\qquad\qquad\quad
	$\abort \auxrel{\abortLab} \inact$ 
	\ \  \rulelabel{P-Abt}}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: auxiliary labelled relation}
	\label{fig:semantics_cherry_pi_aux}
	\vspace*{-.1cm}	
\end{figure*}
The operational rules defining the reduction relation $\fwbwred$
are reported in Fig.~\ref{fig:semantics_cherry_pi}. 
We comment on salient points.
%
Once a session is created, its initiating collaboration is stored in the 
session construct (rule \rulelabel{F-Con}).
%Conditional choices taken outside sessions are not revertible, 
%as they are not subject to checkpointing  (rules \rulelabel{F-IfT} and \rulelabel{F-IfF}).
Communication, branching selection and internal conditional choices proceed as usual, without affecting 
logs (rules \rulelabel{F-Com}, \rulelabel{F-Lab} and \rulelabel{F-If}).  
A commit action updates the checkpoint of a session, by replacing the processes stored in the logs of the two involved parties (rule \rulelabel{F-Cmt}). 
Conversely, a rollback action restores the processes in the two logs (rule \rulelabel{B-Rll}). 
The abort action, instead, restores the collaboration stored in the session 
construct formed by the two initiators that have started the session (rule \rulelabel{B-Abt}).
The other rules simply extend the standard parallel, 
restriction, structural congruence rules to forward and backward relations. 

%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{l@{\hspace*{-.4cm}}l@{\qquad }l}
%%	$C$
%%	$\ \fwred\ $
%%	$\singleSession{s}{C}\ 
%%	(\logged{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}$ 
%%        & $C=(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})$ & \rulelabel{F-Con}
%%        \\
%%        \qquad\qquad\qquad\quad
%%        $\mid\ 
%%	\logged{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )$ 
%%	\\[.4cm]	
%	$\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2}$
%	$\ \fwred\ $
%	$\singleSession{s}{(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})}$ 
%        &  & \rulelabel{F-Con}
%        \\
%        \qquad\qquad\qquad\qquad\qquad\ \ 
%        $(\logged{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}
%        \mid\ 
%	\logged{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )$ 
%	\\[.4cm]	
%%	$\ifthenelseAct{e}{P_1}{P_2}$
%%	$\ \fwred\ $
%%	$P_1$
%%	& $\expreval{e}{\ctrue}$ & \rulelabel{F-IfT}
%%	\\[.2cm]
%%	$\ifthenelseAct{e}{P_1}{P_2}$
%%	$\ \fwred\ $
%%	$P_2$
%%	& $\expreval{e}{\cfalse}$ & \rulelabel{F-IfF}
%%	\\[.3cm]	
%%	$\logged{\ce{\genSession}}{Q_1} \sendAct{\ce{\genSession}}{e}{P_1} 
%%	\ \mid \ 
%%	\logged{\genSession}{Q_2} \receiveAct{\genSession}{x}{P_2}$
%%	$\ \fwred\ $
%%	$\logged{\ce{\genSession}}{Q_1} P_1 
%%	\ \mid \ 
%%	\logged{\genSession}{Q_2} P_2\subst{v}{x}$
%%	\quad $\expreval{e}{v}$
%%	&  & \rulelabel{F-Com}
%%	\\[.2cm]
%	$
%	\infer[$\,\rulelabel{F-Com}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{Q_1} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{\ce{k}}{v}} P_1'
%	\qquad
%	P_2 \auxrel{\receive{k}{x}} P_2'	
%	}
%	$	
%       &  & 
%		\\[.3cm]
%	$
%	\infer[$\,\rulelabel{F-Lab}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{Q_1} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2'
%	}
%	{
%	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
%	\qquad
%	P_2 \auxrel{\branching{k}l} P_2'	
%	}
%	$	
%       &  & 
%		\\[.3cm]		
%	$
%	\infer[$\,\rulelabel{F-Cmt}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{P_2} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	}
%	$	
%       &  & 
%		\\[.3cm]					
%	\end{tabular}
%	\begin{tabular}{l}
%		$
%	\infer[$\,\rulelabel{F-If}$]{
%	\logged{\genSession}{Q} P
%	\ \fwred\ 
%	\logged{\genSession}{Q} P' 
%	}
%	{
%	P \auxrel{\ite} P'
%	}
%	$	
%\qquad\qquad\qquad\qquad
%	$
%	\infer[$\,\rulelabel{F-Par}$]{C_1 \!\mid\! C_2 \ \fwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \fwred\ C_1'}
%	$	
%	\\[.4cm]	
%%	$
%%	\infer[$\,\rulelabel{F-Res1}$]{\res{c}P \ \fwred\ \res{c}P'}
%%	{P \ \fwred\ P'}
%%	$
%	$
%	\infer[$\,\rulelabel{F-Str}$]{C_1 \ \fwred\ C_2}
%	{C_1 \congr C_1'\ \fwred\ C_2' \congr C_2}
%	$
%\qquad\qquad\qquad
%	$
%	\infer[$\,\rulelabel{F-Res}$]{\singleSession{s}{C_1}\,C_2 \ \fwred\ \singleSession{s}{C_1}\,C_2'}
%	{C_2 \ \fwred\ C_2'}
%	$
%	\\[.4cm]	
%	\end{tabular}
%	%%%% BACKWARD RULES
%	\begin{tabular}{l}
%	$
%	\infer[$\,\rulelabel{B-Rll}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \bwred\ 
%	\logged{\ce{\genSession}}{Q_1} Q_1
%	\ \mid \ 
%	\logged{\genSession}{Q_2} Q_2
%	}
%	{
%	P_1 \auxrel{\rollLab} P_1'
%	}
%	$	
%		\\[.4cm]				
%	$
%	\infer[$\,\rulelabel{B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2)
%	\ \bwred\ C
%	}
%	{
%	P_1 \auxrel{\abortLab} P_1'
%	}
%	$	
%	\\[.3cm]
%	\end{tabular}	
%	\begin{tabular}{c@{\qquad\qquad\qquad}c}		
%		$
%	\infer[$\,\rulelabel{B-Par}$]{C_1 \!\mid\! C_2 \ \bwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \bwred\ C_1'}
%	$	
%	&
%%	$
%%	\infer[$\,\rulelabel{B-Res1}$]{\res{c}P \ \bwred\ \res{c}P'}
%%	{P \ \bwred\ P'}
%%	$
%	$
%	\infer[$\,\rulelabel{B-Str}$]{C_1 \ \bwred\ C_2}
%	{C_1 \congr C_1'\ \bwred\ C_2' \congr C_2}
%	$
%	\\[.4cm]	
%	$
%	\infer[$\,\rulelabel{B-Res}$]{\singleSession{s}{C_1}C_2 \ \bwred\ \singleSession{s}{C_1}C_2'}
%	{C_2 \ \bwred\ C_2'}
%	$
%	&
%	\\[.1cm]
%	\hline
%	\end{tabular}	
%	\vspace*{-.2cm}	
%	\caption{\Cherry\ semantics: forward and backward reduction relations }
%	\label{fig:semantics_cherry_pi}
%\end{figure*}
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{@{}l@{}}
%	$\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2}$
%	$\ \fwred\ $
%	$\singleSession{s}{(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})}$ 
%	\hspace*{2.8cm}
%        \rulelabel{F-Con}
%        \\
%        \qquad\qquad\qquad\qquad\qquad\ \ 
%        $(\logged{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}
%        \ \mid\ 
%	\logged{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )$ 
$\requestAct{a}{x_1}{P_1} \!\mid\! \acceptAct{a}{x_2}{P_2}$
	$\!\fwred\!$
	$\singleSession{s\!}{\!(\requestAct{a}{x_1}{P_1} \!\mid\! \acceptAct{a}{x_2}{P_2})} 
        (\loggedShort{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}
        \!\mid\! 
	\loggedShort{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )\ $         \rulelabel{F-Con}
	\\[.4cm]	
	$
	\infer{
	\loggedShort{\ce{\genSession}}{Q_1} P_1 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2
	\ \fwred\ 
	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
	}
	{
	\hspace*{.9cm}
	P_1 \auxrel{\send{\ce{k}}{v}} P_1'
	\qquad
	P_2 \auxrel{\receive{k}{x}} P_2'	
	\hspace*{.7cm}
	$\rulelabel{F-Com}$
	}
	$	
       	\qquad\ \
	$
	\infer{
	\loggedShort{\ce{\genSession}}{Q_1} P_1 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2
	\ \fwred\ 
	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2'
	}
	{
	\hspace*{.7cm}
	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
	\qquad
	P_2 \auxrel{\branching{k}l} P_2'	
	\hspace*{.6cm}
	$\rulelabel{F-Lab}$
	}
	$
	\\[.4cm]		
	$
	\infer[$\rulelabel{F-Cmt}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \fwred\ 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\ \mid \ 
	\logged{\genSession}{P_2} P_2
	}
	{
	P_1 \auxrel{\commitLab} P_1'
	}
	$	
	\quad\
        $
	\infer[$\rulelabel{F-Res}$]{\singleSession{s}{C_1}\,C_2 \ \fwred\ \singleSession{s}{C_1}\,C_2'}
	{C_2 \ \fwred\ C_2'}
	$
        \\[.5cm]
	$
	\infer[$\rulelabel{F-Par}$]{C_1 \!\mid\! C_2 \ \fwred\ C_1' \!\mid\! C_2}
	{C_1 \ \fwred\ C_1'}
	$	
       \qquad\ \	
	$
	\infer[$\rulelabel{F-If}$]{
	\logged{\genSession}{Q} P
	\ \fwred\ 
	\logged{\genSession}{Q} P' 
	}
	{
	P \auxrel{\ite} P'
	}
	$	
	\qquad\quad
	$
	\infer[$\rulelabel{F-Str}$]{C_1 \ \fwred\ C_2}
	{C_1 \congr C_1'\ \fwred\ C_2' \congr C_2}
	$
	\\[.4cm]	
	$
	\infer{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \bwred\ 
	\logged{\ce{\genSession}}{Q_1} Q_1
	\ \mid \ 
	\logged{\genSession}{Q_2} Q_2
	}
	{\hspace*{2.9cm}
	P_1 \auxrel{\rollLab} P_1'
	\hspace*{1.8cm}
	$\rulelabel{B-Rll}$
	}
	$	
	\qquad\quad\
	$
	\infer{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2)
	\ \bwred\ C
	}
	{
	\hspace*{1.6cm}
	P_1 \auxrel{\abortLab} P_1'
	\hspace*{1.3cm}
	$\rulelabel{B-Abt}$
	}
	$	
	\\[.4cm]				
	$
	\infer{\singleSession{s}{C_1}C_2 \ \bwred\ \singleSession{s}{C_1}C_2'}
	{\hspace{.6cm}
	C_2 \ \bwred\ C_2'
	\hspace{.6cm}
	$\rulelabel{B-Res}$}
	$
	\qquad\ \
	$
	\infer[$\!\!\rulelabel{B-Par}$]{C_1 \!\mid\! C_2 \ \bwred\ C_1' \!\mid\! C_2}
	{C_1 \ \bwred\ C_1'}
	$
	\qquad
	$
	\infer[$\!\!\rulelabel{B-Str}$]{C_1 \ \bwred\ C_2}
	{C_1 \congr C_1'\, \bwred\, C_2' \congr C_2}
	$
	\\[.1cm]
	\hline
	\end{tabular}	
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: forward and backward reduction relations }
	\label{fig:semantics_cherry_pi}
	\vspace*{-.5cm}	
\end{figure*}

\begin{example}\label{example_semantics}
Consider the first \cherry\ specification of the VOD scenario given in Ex.~\ref{example_syntax}.
%
In the initial state $C_{\texttt{US}}$ of the collaboration, \texttt{U} and \texttt{S} can synchronise in order to 
initialise the session, thus evolving to:
\\[1mm]
$
C_{\texttt{US}}^1 \ = \ 	\singleSession{s}{C_{\texttt{US}}}\ 
	(\logged{\ce{s}}{P_\texttt{U}\subst{\ce{s}}{x} } P_\texttt{U}\subst{\ce{s}}{x} \ \mid\ 
  	 \logged{s}{P_\texttt{S}\subst{s}{y}}	P_\texttt{S}\subst{s}{y} )
$
 
Let us consider now a possible run of the session. After three reduction steps, \texttt{U} executes the commit action, obtaining the following 
runtime term:\\[1mm]
$
\begin{array}{r@{\ \ }c@{\ \ }l}
C_{\texttt{US}}^2 & = &	\singleSession{s}{C_{\texttt{US}}}\ (\logged{}{P_\texttt{U}'} P_\texttt{U}' \
\mid\ \logged{}{P_\texttt{S}'} P_\texttt{S}' )
\end{array}
$\\[1mm]
$
\begin{array}{@{\quad}r@{\ \ }c@{\ \ }l}
P_\texttt{U}' & = & 
\receiveAct{\ce{s}}{x_{\textit{\textsf{meta}}}:\strType}{\,}
\ifPi\ (f_{\textit{\textsf{eval}}}(v_{\textit{\textsf{price}}},x_{\textit{\textsf{meta}}}))\ \thenPi\ \ldots
\qquad
P_\texttt{S}' \ = \ 
\sendAct{s}{f_{\textit{\textsf{meta}}}(v_{\textit{\textsf{req}}})}{\,}
\branchAct{y}{\ \ldots \ }
\end{array}
$\\[1mm]
After four further reduction steps, \texttt{U} chooses the {\small\textsf{HD}} video quality and \texttt{S} commits as well; the resulting runtime 
collaboration is as follows: 
\\[1mm]
$
\begin{array}{r@{\ \ }c@{\ \ }l}
C_{\texttt{US}}^3 & = & 	\singleSession{s}{C_{\texttt{US}}}\ (\logged{}{P_\texttt{U}''} P_\texttt{U}'' \ \mid\ \logged{}{P_\texttt{S}''} P_\texttt{S}'' )
\end{array}
$\\[1mm]
$
\begin{array}{r@{\ \ }c@{\ \ }l}
P_\texttt{U}'' & = & 
\receiveAct{\ce{s}}{x_{\textit{\textsf{testHD}}}:\strType}{\,}
\ifPi\ (f_{\textit{\textsf{HD}}}(x_{\textit{\textsf{testHD}}}))\ \thenPi\ \receiveAct{\ce{s}}{x_{\textit{\textsf{videoHD}}}:\strType}{\inact}\ \elsePi\ \roll
\end{array}
$\\[1mm]
$\begin{array}{r@{\ \ }c@{\ \ }l}
P_\texttt{S}'' & = & 
\sendAct{s}{f_{\textit{\textsf{testHD}}}(v_{\textit{\textsf{req}}})}{\,}
\sendAct{s}{f_{\textit{\textsf{videoHD}}}(v_{\textit{\textsf{req}}})}{\,}
\inact
\end{array}
$\\[1mm]
In the next reductions, \texttt{U} evaluates the test video and decides to revert the session execution:
\\[1mm]
$
C_{\texttt{US}}^4 \ = \ 	\singleSession{s}{C_{\texttt{US}}}\ (\logged{}{P_\texttt{U}''} \roll \ \mid\ \logged{}{P_\texttt{S}''} 
\sendAct{s}{f_{\textit{\textsf{videoHD}}}(v_{\textit{\textsf{req}}})}{\,}\inact )
$\\[1mm]
The execution of the roll action restores the checkpoints $P_\texttt{U}''$ and $P_\texttt{S}''$, that is 
\mbox{$C_{\texttt{US}}^4 \ \bwred\ C_{\texttt{US}}^3$}. Therefore, 
after the rollback, \texttt{U} is not able to change 
the video quality as her own commit point would have permitted; in fact, it holds
\mbox{$C_{\texttt{US}}^4 \ \bwred\!\!\!\!\!\!\!/\ \ \ \ C_{\texttt{US}}^2$}.
\end{example}


==> tex/binary_properties_LONG.tex <==
% !TEX root = ../rev_sessions@concur.tex
\myparagraph{Soundness properties}
The second group of properties concerns soundness guarantees. 
%In particular, they state that 
%neither \emph{rollback errors} nor \emph{communication errors} 
%occur on rollback safe collaborations (Theorems~\ref{th:roll_soundness} and~\ref{th:com_soundness},
%respectively). 
The definition of these properties requires to formally characterise the errors that 
may occur on the execution of an unsound collaboration. We rely on error reduction 
(as in \cite{ChenDSY17}) rather than on the usual static characterisation of errors
(as, e.g., in \cite{YoshidaV07}), since rollback errors cannot be easily detected statically. 
In particular, we extend the syntax of \cherry\ collaborations
with the $\rollError$ and $\comError$ terms, denoting %respectively 
collaborations in rollback and communication error states:
\\[1mm]
$
\begin{array}{@{}r@{ \ }c@{\ }l@{}}
C & ::= &
\requestAct{a}{x}{P}
\, \mid\,
\acceptAct{a}{x}{P}
\, \mid\,
C_1 \!\mid\! C_2
\, \mid\,
\singleSession{s}{C_1}\ C_2	        
\, \mid
\graybox{$\logged{\genSession}{\checkpointType{P_1}}P_2$}    
\mid
\graybox{$\rollError$}
\mid
\graybox{$\comError$}
\end{array}
$\\[1mm]
where $\checkpointType{P}$ denotes either a checkpoint $P$ committed by the party 
or a checkpoint $\imposed{P}$ imposed by the other party of the session. 
%
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
	$
	\infer[$\!\rulelabel{E-Com1}$]{
	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\send{{k}}{v}} P_1'
	\qquad
	\neg P_2 \BarbInp{k}
	}
	$	
	\qquad
	$
	\infer[$\!\rulelabel{E-Com2}$]{
	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\comError
	}
	{
	P_1 \auxrel{\receive{{k}}{x}} P_1'
	\qquad
	\neg P_2 \BarbOut{k}
	}
	$	
		\\[.3cm]	
	$
	\infer[$\!\rulelabel{E-Lab1}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\select{{k}}{l}} P_1'
	\qquad
	\neg P_2\BarbBranching{k}{l}
	}
	$			
	\qquad\
	$
	\infer[$\!\rulelabel{E-Lab2}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\branching{k}l} P_1'
	\qquad
	\neg P_2\BarbSelect{k}{l}
	}
	$
		\\[.3cm]	
	$
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\imposed{P_2}} P_2
	}
	{\hspace*{.8cm}
	P_1 \auxrel{\commitLab} P_1'
	\qquad 
	\checkpointType{Q_2} \neq P_2
	\hspace*{.8cm}
	$\rulelabel{E-Cmt$_1$}$
	}
	$	
	\qquad
	$
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	}
	{\hspace*{.8cm}
	P_1 \auxrel{\commitLab} P_1'
	\qquad 
	\checkpointType{Q_2} = P_2
	\hspace*{.8cm}
	$\rulelabel{E-Cmt$_2$}$
	}
	$	
		\\[.3cm]	
	\hspace*{-1.5cm}
	$
	\infer{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\bwred
	\logged{\ce{\genSession}}{Q_1} Q_1
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} Q_2
	}
	{	\hspace*{2.1cm}
	P_1 \auxrel{\rollLab} P_1'
		\hspace*{1.9cm}
	$\rulelabel{E-Rll$_1$}$
	}
	$	
	\qquad	
	$
	\infer{
	\logged{\ce{\genSession}}{\imposed{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\rollError
	}
	{\hspace*{1.4cm}
	P_1 \auxrel{\rollLab} P_1'
	\hspace*{1.2cm}
	$\,\rulelabel{E-Rll$_2$}$
	}
	$	
%		
%	$
%	\infer[$\,\rulelabel{F-Lab}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{Q_1} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2'
%	}
%	{
%	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
%	\qquad
%	P_2 \auxrel{\branching{k}l} P_2'	
%	}
%	$	
%       &  & 
%		\\[.3cm]		
%	$
%	\infer[$\,\rulelabel{F-Cmt}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{P_2} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	}
%	$	
%       &  & 
%		\\[.3cm]					
%	\end{tabular}
%	\begin{tabular}{l}
%		$
%	\infer[$\,\rulelabel{F-If}$]{
%	\logged{\genSession}{Q} P
%	\ \fwred\ 
%	\logged{\genSession}{Q} P' 
%	}
%	{
%	P \auxrel{\ite} P'
%	}
%	$	
%\qquad\qquad\qquad\qquad
%	$
%	\infer[$\,\rulelabel{F-Par}$]{C_1 \!\mid\! C_2 \ \fwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \fwred\ C_1'}
%	$	
%	\\[.4cm]	
%	$
%	\infer[$\,\rulelabel{F-Str}$]{C_1 \ \fwred\ C_2}
%	{C_1 \congr C_1'\ \fwred\ C_2' \congr C_2}
%	$
%\qquad\qquad\qquad
%	$
%	\infer[$\,\rulelabel{F-Res}$]{\singleSession{s}{C_1}\,C_2 \ \fwred\ \singleSession{s}{C_1}\,C_2'}
%	{C_2 \ \fwred\ C_2'}
%	$
%	\\[.4cm]	
%	\end{tabular}
%	%%%% BACKWARD RULES
%	\begin{tabular}{l}
%	$
%	\infer[$\,\rulelabel{B-Rll}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \bwred\ 
%	\logged{\ce{\genSession}}{Q_1} Q_1
%	\ \mid \ 
%	\logged{\genSession}{Q_2} Q_2
%	}
%	{
%	P_1 \auxrel{\rollLab} P_1'
%	}
%	$	
%		\\[.4cm]				
%	$
%	\infer[$\,\rulelabel{B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2)
%	\ \bwred\ C
%	}
%	{
%	P_1 \auxrel{\abortLab} P_1'
%	}
%	$	
%	\\[.3cm]
%	\end{tabular}	
%	\begin{tabular}{c@{\qquad\qquad\qquad}c}		
%		$
%	\infer[$\,\rulelabel{B-Par}$]{C_1 \!\mid\! C_2 \ \bwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \bwred\ C_1'}
%	$	
%	&
%	$
%	\infer[$\,\rulelabel{B-Str}$]{C_1 \ \bwred\ C_2}
%	{C_1 \congr C_1'\ \bwred\ C_2' \congr C_2}
%	$
%	\\[.4cm]	
%	$
%	\infer[$\,\rulelabel{B-Res}$]{\singleSession{s}{C_1}C_2 \ \bwred\ \singleSession{s}{C_1}C_2'}
%	{C_2 \ \bwred\ C_2'}
%	$
%	&
	\\[.1cm]
	\hline
	\end{tabular}	
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: error reductions  (symmetric rules are omitted)}
	\label{tab:error_red}
	\vspace*{-.5cm}
\end{figure*}
%
The semantics of \cherry\ is extended as well by the (error reduction) rules in  Fig.~\ref{tab:error_red}, 
where \rulelabel{E-Cmt$_1$} and \rulelabel{E-Cmt$_2$} replace \rulelabel{F-Cmt},
and \rulelabel{E-Rll$_1$} replaces  \rulelabel{B-Rll},
and $\checkpointType{\ }$ is used in the checkpoints of the other rules.
The error semantics does not affect the normal behaviour of \cherry\ specifications, 
but it is crucial for stating our soundness theorems. 
%
Its definition is based on the notion of \emph{barb} predicates, whose straightforward 
definition is: 
\vspace*{-.2cm}
\begin{itemize}
\item $P\barbInp{k}$ if $P$ can perform an input action along session channel $k$;
\item $P\barbOut{k}$ if $P$ can perform an output action along session channel $k$;
\item $P\barbSelect{k}{l}$ if $P$ can perform a select action on label $l$ along session channel $k$;
\item $P\barbBranching{k}{l}$ if $P$ can perform a branching action on label $l$ along session channel $k$;
\item $P\Barb{\mu}$ if there exists $P'$ such that $P \Rightarrow P'$ and $P'\barb{\mu}$, 
where $\mu$ stands for $k?$, $k!$,$k\triangleleft l$ or $k\triangleright l$, and $\Rightarrow$ 
is the reflexive and transitive closure of $\auxrel{\ite}$.
\end{itemize}
The meaning of the error semantics rules is as follows.
A \emph{communication error} takes place in a collaboration when 
a session participant is willing to perform an output but the other participant is not ready to 
perform the corresponding input (\rulelabel{E-Com1}) or viceversa 
(\rulelabel{E-Com2}), or 
one participant is willing to perform a selection but the corresponding branching is not available 
on the other side (\rulelabel{E-Lab1}) or viceversa (\rulelabel{E-Lab2}).
Instead, a \emph{rollback error} takes place in a collaboration when a participant is willing 
to perform a rollback action but its checkpoint has been imposed by the other participant
(\rulelabel{E-Rll$_2$}). To enable this error check, the rules for commit and rollback 
have been modified in order to keep track of imposed overwriting of checkpoints (see, in particular, 
rule \rulelabel{E-Cmt$_1$}). 
This information is not relevant for the runtime execution of processes, 
but it is necessary for characterising 
%essential for conveniently characterise 
the rollback errors that our 
type-based approach prevents. 
%This motivates the use of error reduction rather than of the 
%usual static characterisation of errors, as e.g. in \cite{YoshidaV07}, because rollback errors cannot be easily detected statically.



Besides defining the error semantics, we also need to define erroneous collaborations,
based on the following notion of context:
$
\collContext \ ::=  \ [\cdot] \,\, \mid\,\,  \collContext \!\mid\! C \,\, \mid\,\,  \singleSession{s}{C}\ \collContext
$.
%\begin{definition}[Erroneous collaborations]
%A collaboration $C$ is \emph{communication (resp. rollback) erroneous} if 
%$C = \collContext[\comError]$ (resp. $C = \collContext[\rollError]$).
%\end{definition}
Thus, a collaboration is \emph{communication (resp. rollback) erroneous} if 
it has the form $\collContext[\comError]$ (resp. $\collContext[\rollError]$).


%Finally, we are able to state the two soundness results. 
%\begin{theorem}[Communication soundness]
%\label{th:com_soundness}
%A rollback safe collaboration never reduces to a communication erroneous collaboration.
%\end{theorem}
%\begin{proof} 
%\emph{(Sketch)} todo
%\end{proof}
%
%\begin{theorem}[Rollback soundness]
%\label{th:roll_soundness}
%A rollback safe collaboration never reduces to a rollback erroneous collaboration.
%\end{theorem}
%\begin{proof} 
%\emph{(Sketch)} todo
%\end{proof}

The key soundness results follow: a rollback safe collaboration never 
reduces to either a rollback erroneous collaboration (Theorem~\ref{th:roll_soundness}) or a
communication erroneous collaboration (Theorem~\ref{th:com_soundness}). 
\begin{theorem}[Rollback soundness]
\label{th:roll_soundness}
If $C$ is a rollback safe collaboration, then $C\ {\fwbwred\!\!\!\!\!\!/\ }^*\ \collContext[\rollError]$.
\end{theorem}
%\begin{proof} 
%\emph{(Sketch)} The proof proceed by contradiction (see Appendix~\ref{soundness_proofs}). 
%\end{proof}

\begin{theorem}[Communication soundness]
\label{th:com_soundness}
If $C$ is a rollback safe collaboration, then $C\ {\fwbwred\!\!\!\!\!\!/\ }^*\ \collContext[\comError]$.
\end{theorem}
%\begin{proof} 
%\emph{(Sketch)} The proof proceed by contradiction (see Appendix~\ref{soundness_proofs}). 
%\end{proof}

We conclude with a property concerning the progress of \cherry\ sessions: 
given a rollback safe collaboration that can initiate a session, 
each collaboration reachable from it either is able to progress on the session 
with a forward/backward reduction step or has correctly reached the end of 
the session. This result straightforwardly follows from 
Theorems~\ref{th:roll_soundness} and~\ref{th:com_soundness}, and from
the fact that we consider binary sessions without delegation and subordinate sessions. 
\begin{theorem}[Session progress]
\label{th:deadlock_freedom}
Let $C=(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})$ be a rollback safe collaboration.
If $C \fwbwred^* C'$ then either $\exists\, C''$ such that $C' \fwbwred C''$ or 
$C' \congr 
\singleSession{s}{C}
(\logged{{\genSession}}{\checkpointType{Q_1}} \inact 
\ \mid \ 
\logged{\genSession}{\checkpointType{Q_2}} \inact)$
for some $\checkpointType{Q_1}$ and $\checkpointType{Q_2}$.
\end{theorem}
%\begin{proof} 
%\emph{(Sketch)} todo
%\end{proof}







%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{l}
%	$
%	\receiveAct{k}{y:S}{P}\barbInp{k}
%	$	
%	\\[.3cm]
%
%	\hline
%	\end{tabular}	
%	\vspace*{-.2cm}	
%	\caption{\Cherry\ semantics: barbs }
%	\label{tab:barbs}
%\end{figure*}


%$\sendAct{x}{e}{P}$
%$\receiveAct{x}{y:S}{P}$ 
%$\inact$
%$\selectAct{x}{l}{P}$
%$\branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ 
%$\ifthenelseAct{e}{P_1}{P_2}$ 
%$X$ 
%$\recAct{X}{P}$ 
%$\commitAct{P}$
%$\roll$
%$\abort$  




==> tex/binary_type_system_LONG.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex
\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{c}
	$
	\infer[$\rulelabel{T-Req}$]{\requestAct{a}{x}{P} \hasType \{\ce{a}:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$		
	\qquad
	$
	\infer[$\rulelabel{T-Acc}$]{\acceptAct{a}{x}{P} \hasType \{a:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$
	\qquad
	$
	\infer[$\rulelabel{T-Par}$]{C_1\mid C_2 \hasType \sessions_1 \cup \sessions_2}
	{C_1 \hasType \sessions_1 & C_2 \hasType \sessions_2}
	$
        \\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}
	\caption{Typing system for \cherry\ collaborations}
	\vspace*{-.6cm}	
	\label{fig:typingSystem_coll}
\end{figure}
	


	
	
\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{@{}r@{\qquad\qquad}r@{}}
		$
	\infer[$\rulelabel{T-Send}$]{\basis;\sorting \judge \sendAct{x}{e}{P} \hasType x:\outType{S}.\typeT}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
	$		
	&
	$
	\infer[$\rulelabel{T-Rcv}$]{\basis;\sorting \judge \receiveAct{x}{y:S}{P} \hasType x:\inpType{S}.\typeT}
	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
	$	
	\\[.4cm]	
        $\basis;\sorting \judge \inact \hasType x:\inactType$\ \ \rulelabel{T-Inact}		
        &
	$
	\infer[$\rulelabel{T-Sel}$]{\basis;\sorting \judge \selectAct{x}{l}{P} \hasType 
	x:\selType{l}.\typeT}
	{\basis;\sorting  \judge P \hasType x:\typeT}
	$        
	\end{tabular}
	\begin{tabular}{@{}c@{}}
	\\[.2cm]			
	$
	\infer[$\rulelabel{T-Br}$]{\basis;\sorting \judge \branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType 
	x:\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}}
	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
	$
	\\[.6cm]		
	$
	\infer[$\rulelabel{T-If}$]{\basis;\sorting \judge \ifthenelseAct{e}{P_1}{P_2} \hasType 
	x:\typeT_1 \choiceType \typeT_2}
	{\sorting  \judge e \hasType \boolType &&
	\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \basis;\sorting  \judge P_2 \hasType x:\typeT_2}
	$
	\\[.4cm]	
	$\basis\comp X:t;\sorting \judge X \!\hasType\! t$\ \rulelabel{T-Pvar}			
	\quad
	\infer[$\rulelabel{T-Rec}$]{\basis;\sorting \judge \recAct{X}{P} \hasType \recAct{t}{\typeT}}
	{\basis\comp X:t;\sorting  \judge P \hasType \typeT}	
	\quad
	$
	\infer{\basis;\sorting \judge \commitAct{P}  \hasType 
	x:\commitType.\typeT}
	{\ \ 
	\basis;\sorting  \judge P \hasType x:\typeT 
	\quad\ $\rulelabel{T-Cmt}$}
	$
	\\[.4cm]
	$\basis;\sorting \judge \roll \hasType x:\rollType$\ \ \rulelabel{T-Rll}	
	\quad
      %  \hspace*{2.5cm}
	$\basis;\sorting \judge \abort \hasType x:\abortType$\ \ 
	\rulelabel{T-Abt}		
	\quad
	$\sorting\comp x:S \judge x \hasType S$\ \ \rulelabel{T-Var}\\	
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Typing System for \cherry\ processes}
	\label{fig:typingSystem_proc}
\end{figure}


\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{tt}}$}
	\qquad
	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{ff}}$}
	\\[.4cm]	
	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{T-Int}	
	\qquad\qquad
	$\sorting \judge\!\!``a" \hasType \strType$\ \ \rulelabel{T-Str}	
	\qquad\qquad
	$\sorting\comp x:S \judge x \hasType S$\ \ \rulelabel{T-Var}	
	\\[.4cm]
	$
	\infer[$\rulelabel{T-Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
	{\sorting \judge e_1 \hasType \intType & & \sorting \judge e_2 \hasType \intType}
	\qquad
	\infer[$\rulelabel{T-And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
	{\sorting \judge e_1 \hasType \boolType & & \sorting \judge e_2 \hasType \boolType}
	$		
        \\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}
	\caption{Typing system for \cherry\ expressions (excerpt of
          rules)}
	\vspace*{-.5cm}
	\label{fig:typingSystem_exp}
\end{figure}



==> tex/binary_types_LONG.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex
\section{Rollback safety}
\label{sec:rollback_safety}

The operational semantics of \cherry\ provides a description of the functioning of the 
primitives for programming  checkpoint-based rollback recovery in a session-based language. 
However, as shown in the Ex.~\ref{example_semantics}, it does not guarantee high-level 
properties about the safe execution of the rollback. 
%
%As mentioned in Section~\ref{sec:intro}, in our approach a party executing a 
%rollback action expects that it is restored the last checkpoint she has committed, not one committed 
%by the other session party. The undesired situation is instead allowed by the semantics, as illustrated by the following example. 
%\begin{example}\label{example}
%Let us consider a client/server scenario where the server ($S$) can offer to the user ($U$) a service with two different quality levels, namely high ($H$) and low ($L$). This is rendered in \cherry\ as the collaboration:
%$$
%\requestPrefix{serv\_req}{x}.\ P_U \ \mid\ \acceptPrefix{serv\_req}{y}.\ P_S
%$$
%where:
%$$
%\begin{array}{rcl}
%P_U & = & \commitAct{}\ \ifPi\ (e)\ \thenPi\ \selectAct{{x}}{l_H}{\sendAct{x}{v}{}}
%\ifPi\ (e')\ \thenPi\ \receiveAct{x}{w}{Q_H}\ \elsePi\ \roll\\
%&& \qquad\qquad\qquad\quad\, 
%\elsePi\ \selectAct{{x}}{l_L}{\sendAct{x}{v}{}}
%\ifPi\ (e'')\ \thenPi\ \receiveAct{x}{w}{Q_L}\ \elsePi\ \roll
%\\
%\\
%P_S & = & 
%\branchAct{y}{
%\branch{l_H\!}{\!\commitAct{\receiveAct{y}{z}{\sendAct{y}{e_H(z)}{P_H}}}} 
%\ \branchSep \
%\branch{l_L\!}{\!\commitAct{\receiveAct{y}{z}{\sendAct{y}{e_L(z)}{P_L}}}}}
%\end{array}
%$$
%After the client selection, the server commits. After sending the service request data (value $v$), 
%the client decides whether proceedings on the session or rolling back to the beginning of the session 
%to possibly change the service quality. However, when the client activate the rollback, she is not able 
%to go back to the beginning of the session, because the rollback effect is blocked by the 
%server's commit as shown in Figure~\ref{fig:scenario}(b).
%\qed
%%\begin{figure}[t]
%%\centering
%%\includegraphics[scale=.4]{img/scenario}
%%\vspace*{-.4cm}
%%\caption{Undesired rollback recovery scenario}
%%\label{fig:scenario}
%%\end{figure}
%\end{example}
%
To prevent such undesired rollbacks, we propose the use of a \emph{compliance checking}, to be performed at design time before actually executing the system. This check is not done on the full system specification, but only at the level of session types. 

\myparagraph{Session types and typing}
%SESSION TYPES
%{\color{red}
%To type \cherry\ collaborations, we have revised and extended the standard binary session types for \pic\ 
%%\cite{HondaVK98,YoshidaV07}. 
%\cite{YoshidaV07}. 
%A key difference with respect to the standard type discipline is the relaxation of the duality requirement. Indeed, the type of two session participants are not required to be dual, but they will be compared with respect to a compliance relation, which takes into account the effects of commit and rollback actions. Such relaxation also involves the requirements concerning selection and branching types, and those concerning the branches of the conditional choice construct. 
%%
%In fact, the aim of our type system is not to check duality, but just to infer the types of collaboration participants, which will be then checked together according to the compliance relation. 
%}
The syntax of the \cherry\ \emph{session types} is defined in Fig.~\ref{fig:typeSyntax_cherry}. 
\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\quad}l@{}}
%	$S$ & ::= &  & \textbf{Sorts}\\
%	&             & $\boolType$ \quad $\mid$ \quad $\intType$ \quad $\mid$ \quad $\strType$ 
%	& \ boolean, integer, string
	$S$ & ::= & \ \ $\boolType$ \quad $\mid$ \quad $\intType$ \quad $\mid$ \quad $\strType$ & \textbf{Sorts}
	\\[.1cm]	
	$\typeT$ & ::= &  &  \textbf{Session types}\\
	&             & 
	$\outType{S}.\typeT$ \ \ $\mid$ \ \
	$\inpType{S}.\typeT$ \ \ $\mid$ \ \
	$\selType{l}.\typeT$ 	 \ \  $\mid$ \ \ 
	$\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$
	& \ output, input, selection, branching
	\\[.05cm]
	& $\mid$ &  
	$\typeT_1 \choiceType \typeT_2$ \ \ $\mid$ \ \ 
	$t$ \ \ $\mid$ \ \ $\recType{t}.\typeT$ \ \ $\mid$ \ \ 
	$\inactType$ \ \ $\mid$ \ \
	$\commitType.\typeT$ \ \ $\mid$ \ \ 
	$\rollType$ \ \ $\mid$ \ \ 
	$\abortType$
	& \ choice, recursion, end, commit, roll, abort
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{\Cherry\ type syntax %(Sorts $S$ are as in Figure~\ref{fig:syntax_cherry_pi})
	}
	\label{fig:typeSyntax_cherry}
	\vspace*{-.2cm}
\end{figure}
The type $\outType{S}.\typeT$ represents the behaviour of first outputting a value of sort $S$, 
then performing the actions prescribed by type $\typeT$. The type $\inpType{S}.\typeT$ is the dual one, where a value is received instead of sent. 
Type $\inactType$ represents inaction. %, acting as the unit of sequential composition.
Type $\selType{l}.\typeT$ represents the behaviour that selects the label $l$ and then behaves as $\typeT$. 
Type $\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$ describes a branching 
behaviour: it waits with $n$ options, and behaves as type $\typeT_i$ if the $i$-th label is selected 
(external choice).
Type $\typeT_1 \choiceType \typeT_2$ behaves as either $\typeT_1$ or 
$\typeT_2$ (internal choice).
Type $\recType{t}.\typeT$ represents a recursive behaviour that starts 
by doing $\typeT$ and, when variable $t$ is encountered, recurs to $\typeT$ again. 
%
Type $\commitType.\typeT$ represents a commit action followed by the actions prescribed by type 
$\typeT$. 
Finally, types $\rollType$ and $\abortType$ represent rollback and abort actions, respectively. 

%\emph{Typing judgements} are of the form $\basis;\sorting \judge C \hasType \typing;\sessions$,
%where $\basis$, $\sorting$ and $\typing$, called \emph{basis}, \emph{sorting} and \emph{typing}
%respectively,  are finite partial maps 
%from process variables to typings,
%from variables to sorts, 
%from variables to types, respectively, 
%while $\sessions$, called \emph{type associations}, is a set of session type 
%associations of the form $\reqOrApp{a}:\typeT$, where $\reqOrApp{a}$
%stands for either $\ce{a}$ or $a$.
%%
%Intuitively,  the judgement $\basis;\sorting \judge C \hasType \typing;\sessions$ 
%stands for ``under the environment $\basis;\sorting$, collaboration $C$ has typing $\typing$''. 
%The axioms and rules defining the typing system are standard 
%Figure~\ref{fig:typingSysytem}
The \cherry\ type system does not perform compliance checks, but 
it just aims at inferring the types of collaboration participants, which will be then checked together 
according to the compliance relation. 
\emph{Typing judgements} are of the form $C \hasType \sessions$,
where $\sessions$, called \emph{type associations}, is a set of session type 
associations of the form $\reqOrApp{a}:\typeT$, where $\reqOrApp{a}$
stands for either $\ce{a}$ or $a$.
%
Intuitively,  the judgement $C \hasType \sessions$ indicates that from 
the collaboration $C$ the type associations in $\sessions$ are inferred. 
%
The definition of the type system for these judgments relies on auxiliary 
typing judgements for processes, of the form $\basis;\sorting \judge P \hasType \typing$,
where $\basis$, $\sorting$ and $\typing$, called \emph{basis}, \emph{sorting} and \emph{typing}
respectively,  are finite partial maps 
from process variables to type variables,
from variables to sorts, 
from variables to types, respectively.
The update of basis and sorting are denoted, respectively, 
by $\basis\comp X:t$ and $\sorting\comp y:S$, where 
$X \notin dom(\basis)$, $t \notin cod(\basis)$ and $y \notin dom(\sorting)$.
%
Intuitively,  the judgement $\basis;\sorting \judge P \hasType \typing$ 
stands for ``under the environment $\basis;\sorting$, process $P$ has typing $\typing$''. 
%
In its own turn, the typing of processes relies on auxiliary (standard) judgments for
expressions, of the form $\sorting \judge e \hasType S$.
%
The axioms and rules defining the typing system for \cherry\ collaborations, processes and expressions 
are given in Fig.~\ref{fig:typingSystem_coll} and~\ref{fig:typingSystem_proc} %and~\ref{fig:typingSystem_exp}, 
respectively. {\color{blue} We omit typing rules for expressions, which are standard.}
%
The type system is defined only for initial collaborations, i.e. for terms generated by the grammar in Fig.~\ref{fig:syntax_cherry_pi}. Other runtime collaborations are not considered here, as no check will be performed at runtime.
%
We comment on salient points. Typing rules at collaboration level simply collect the type associations 
of session initiators in the collaboration. Rules at process level instead determine the session 
type corresponding to each process, by mapping each process operator to the corresponding type operator. 
Data and expression used in communication actions are abstracted as
sorts and
a conditional choice is rendered as an internal non-deterministic choice. 


\input{./tex/binary_type_system}

\myparagraph{Compliance checking}
To check compliance between pairs of session parties, we consider
\emph{type configurations} of the form 
$
\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeT}_1}{\typeT_2} \confcomp \conf{\checkpointType{\typeT}_3}{\typeT_4}
$,  
consisting in a pair $(\typeT,\typeT')$ of session types, corresponding to the types of the parties at the initiation of the session, and in the parallel composition of two pairs $\conf{\checkpointType{\typeT}_c}{\typeT}$, where $\typeT$ is the session type of a party and $\checkpointType{\typeT}_c$ is the type of the party's checkpoint. We use $\checkpointType{\typeT}$ to denote either a type $\typeT$, representing a checkpoint committed by the party, or $\imposed{\typeT}$, representing a checkpoint imposed by the other party of the session. 
%
The semantics of type configurations, necessary for the definition of the compliance relation, is given in Fig.~\ref{fig:typeSemantics_ext}, where label $\typeLab$ stands for either 
$\outType{S}$,
$\inpType{S}$,
$\selTypeLabel{l}$,
$\branchTypeLabel{l}$,
$\tau$,
$\commitType$,
$\rollType$,
or $\abortType$.
{\color{blue} Given a label $\typeLab = \outType{S}$ (resp.$\typeLab = \selTypeLabel{l}$) we indicate  
with $\overline\typeLab = \inpType{S}$ (resp. $\overline\typeLab = \branchTypeLabel{l}$) and vice versa.
 }
%
The only relevant rules are those for commit, roll and abort synchronisations. 
In case of a commit action, the checkpoints of both parties are updated, but the one 
of the passive party (i.e., the party that has not performed the commit action) 
is marked as `imposed' (rule \rulelabel{TS-Cmt$_1$}). 
However, if the passive party did not perform any action from its 
current checkpoint, this checkpoint is not overwritten by the active party (rule \rulelabel{TS-Cmt$_2$}),
as discussed in \S~\ref{sec:motivation} (Fig.~\ref{fig:scenario}(c)). 
In case of a roll action (rule \rulelabel{TS-Rll$_1$}), the reduction step is performed 
only if the active party (i.e., the party that has performed the rollback 
action) has a non-imposed checkpoint; % and the passive party has an imposed checkpoint;
in all other situations the configuration cannot proceed with the rollback.
Finally, in case of abort (rule \rulelabel{TS-Abt$_1$}), the configuration goes back to the initial state; this 
allows the type computation to proceed, in order to not affect the compliance check
between the two parties. 

\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{@{}r@{\hspace*{-.7cm}}r@{\hspace*{-.7cm}}r@{}}
	$\outType{S}.\typeT \typeTrans{\outType{S}} \typeT$\ \ \rulelabel{TS-Snd}	
	&
	$\inpType{S}.\typeT \typeTrans{\inpType{S}} \typeT$\ \ \rulelabel{TS-Rcv}  
	&
	$\selType{l}.\typeT \typeTrans{\selTypeLabel{l}} \typeT$\ \ \rulelabel{TS-Sel}
	\\[.3cm]
	\multicolumn{2}{l}{
	\qquad
	\raisebox{.6cm}{$
	\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}
	\typeTrans{\branchTypeLabel{l_i}} \typeT_i$ \quad $(1 \leq i \leq n)$\ \ \ \ \rulelabel{TS-Br}
	\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!	}
	}
	&
	$
	\infer[$\rulelabel{TS-rec}$]
	{\recType{t}.\typeT \typeTrans{\typeLab} \typeT'}
	{\typeT\subst{\recType{t}.\typeT}{t} \typeTrans{\typeLab} \typeT'}
	$
\\[-.3cm]
	$
	\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_1$\ \ \rulelabel{TS-If$_1$}
	&
	$\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_2$\ \ \rulelabel{TS-If$_2$}
	&
		\\[.3cm]
	$\commitType.\typeT \typeTrans{\commitType} \typeT$\ \ \rulelabel{TS-Cmt}
	&
	$\rollType \typeTrans{\rollType} \inactType$\ \ \rulelabel{TS-Rll}
	&
	$\abortType \typeTrans{\abortType} \inactType$\ \ \rulelabel{TS-Abt}
	\\
	\\
%	\multicolumn{3}{l}{
%	$
%	\infer[$ \rulelabel{TS-Tau}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	{\typeT_1 \typeTrans{\tau} \typeT_1'}
%	$	
%	}\\
%	\\
%	\multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Com}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	{\typeT_1 \typeTrans{\outType{S}} \typeT_1'
%	\qquad\qquad
%	 \typeT_2 \typeTrans{\inpType{S}} \typeT_2'}
%	$	
%	}\\
%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Lab}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	{\typeT_1 \typeTrans{\selTypeLabel{l}} \typeT_1'
%	\qquad\qquad
%	 \typeT_2 \typeTrans{\branchTypeLabel{l}} \typeT_2'}
%	$	
%	}\\
%	\\
%%        \multicolumn{3}{l}{
%%	$
%%	\infer[$\rulelabel{TS-}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%%	{\typeT_1 \typeTrans{\commitType} \typeT_1'}
%%	$	
%%	}\\
%%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Cmt$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%	{\typeT_1 \typeTrans{\commitType} \typeT_1' \qquad\qquad \checkpointType{\typeU}_2 \neq \typeT_2}
%	$	
%	}\\
%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Cmt$_2$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	{\typeT_1 \typeTrans{\commitType} \typeT_1' \qquad\qquad \checkpointType{\typeU}_2 = \typeT_2}
%	$	
%	}\\
%	\\
%%        \multicolumn{3}{l}{
%%	$
%%	\infer[$\rulelabel{TS-}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\imposed{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\imposed{\typeU_2}}{\typeU_2}}
%%	{\typeT_1 \typeTrans{\rollType} \typeT_1'}
%%	$	
%%	}\\
%%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Rll$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeU_2}}
%	{\typeT_1 \typeTrans{\rollType} \typeT_1'}
%	$	
%	}\\
%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-Abt$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT}{\typeT} \confcomp \conf{\typeT'}{\typeT'}}
%	{\typeT_1 \typeTrans{\abortType} \typeT_1'}
%	$	
%	}
	\multicolumn{3}{@{}l@{}}{	
	$
	{\typeT_1 \typeTrans{\tau} \typeT_1'}
	\Rightarrow	
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
	\quad $\rulelabel{TS-Tau}$
	$	
	}\\
	\\
	\multicolumn{3}{@{}l@{}}{
	{\color{blue}
	$
	{\typeT_1 \typeTrans{\typeLab} \typeT_1'
	\, ,\,
	 \typeT_2 \typeTrans{\overline{\typeLab}} \typeT_2'}	
	\Rightarrow		
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
	\ \ $\rulelabel{TS-Synch}$
	$
	}	
	}\\
	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\!\outType{S}\!} \typeT_1'
%	\, ,\,
%	 \typeT_2 \typeTrans{\!\!\inpType{S}\!} \typeT_2'}	
%	\Rightarrow		
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	\ \ $\rulelabel{TS-Com}$
%	$	
%	}\\
%	\\
%	\multicolumn{3}{@{}l@{}}{
%	$
%	{\typeT_1 \typeTrans{\selTypeLabel{l}} \typeT_1'
%	\, , \,
%	 \typeT_2 \typeTrans{\branchTypeLabel{l}} \typeT_2'}
%	\Rightarrow 
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	\ \ $\rulelabel{TS-Lab}$
%	$	
%	}\\
%	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%	{\typeT_1 \typeTrans{\commitType} \typeT_1'}
%	$	
%	}\\
%	\\
	\multicolumn{3}{@{}l@{}}{
	$
	{\typeT_1 \typeTrans{\commitType} \typeT_1' \, , \, \checkpointType{\typeU}_2 \neq \typeT_2}
	\Rightarrow	
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
	\ \ \ $\rulelabel{TS-Cmt$_1$}$
	$	
	}\\
	\\
	\multicolumn{3}{@{}l@{}}{
	$
	{\typeT_1 \typeTrans{\commitType} \typeT_1' \, ,\, \checkpointType{\typeU}_2 = \typeT_2}
	\Rightarrow
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
	\ \ \ $\rulelabel{TS-Cmt$_2$}$
	$	
	}\\
	\\
%        \multicolumn{3}{l}{
%	$
%	\infer[$\rulelabel{TS-}$]
%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\imposed{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\imposed{\typeU_2}}{\typeU_2}}
%	{\typeT_1 \typeTrans{\rollType} \typeT_1'}
%	$	
%	}\\
%	\\
	\multicolumn{3}{@{}l@{}}{
	$
	{\typeT_1 \typeTrans{\rollType} \typeT_1'}
	\Rightarrow
	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeU_2}}
	\quad $\rulelabel{TS-Rll$_1$}$
	$	
	}\\
	\\
	\multicolumn{3}{@{}l@{}}{
	$
	{\typeT_1 \typeTrans{\abortType} \typeT_1'}
	\Rightarrow
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\typeT}{\typeT} \confcomp \conf{\typeT'}{\typeT'}}
	\quad $\rulelabel{TS-Abt$_1$}$
	$	
	}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Semantics of types and type configurations (symmetric rules for configurations are omitted)}
	\label{fig:typeSemantics_ext}
	\vspace*{-.5cm}
\end{figure}

We define the compliance relation, inspired by the relation in
\cite{BarbaneraDLd16}, and prove its decidability. 
\begin{defi}[Compliance]\label{def:compliance}
Two types $\typeT_1$ and $\typeT_2$ are \emph{compliant}, written 
$\typeT_1 \compliant \typeT_2$, if  
$\initConf{\typeT_1}{\typeT_2}\conf{\typeT_1}{\typeT_1} \compliant \conf{\typeT_2}{\typeT_2}$.
Relation $\compliant$ on configurations is defined as follows:
$\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU_1}}{\typeT_1} \compliant \conf{\checkpointType{\typeU_2}}{\typeT_2}$
%whenever 
%$\initConf{\typeT'}{\typeT''}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\typeU_2}{\typeT_2}
%\typered^*$
%$\initConf{\typeT'}{\typeT''}\conf{\typeU_1'}{\typeT_1'} \confcomp \conf{\typeU_2'}{\typeT_2'}
%\typered\!\!\!\!\!\!\!\!/$
%implies $\typeT_1'=\typeT_2'=\inactType$.
holds if for any $\typeU_1'$, $\typeT_1'$, $\typeU_2'$, $\typeT_2'$ such that
$\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU_1}}{\typeT_1} \confcomp \conf{\checkpointType{\typeU_2}}{\typeT_2}
\typered^*$
$\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU_1'}}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU_2'}}{\typeT_2'}
\typered\!\!\!\!\!\!\!\!/\ \ \  $
we have that $\typeT_1'=\typeT_2'=\inactType$.
\end{defi}

%The result below states that compliance checking is decidable. 
\begin{thm}\label{th:decidability}
Let $\typeT_1$ and $\typeT_2$ be two session types, checking if $\typeT_1 \compliant \typeT_2$ holds
is decidable.
\end{thm}
%Compliance is decidable. In fact, it boils down to check if the leaves of the 
%labelled transition system (LTS) produced by the semantics of the considered type configuration correspond to $\inactType$ types. 
%The decidability of this check depends on the finiteness of the LTS, which is ensured 
%by the fact that we have no static operators (i.e., parallel and restriction) within recursion. 
%%The complexity cost of the compliance check depends on the size of the LTS, given 
%%by the product of the sizes of the two composed types.  


The above compliance relation is used to define the notion of \emph{rollback safety}.
\begin{defi}[Rollback safety]\label{def:rollback_safety}
Let $C$ be an initial collaboration, then $C$ is \emph{rollback safe} if $C \hasType \sessions$
and for all pairs $\ce{a}:\typeT_1$ and $a:\typeT_2$ in $\sessions$ we have 
$\typeT_1 \compliant \typeT_2$.
\end{defi}


\begin{exa}
Given a collaboration $C=\requestAct{a}{x}{P} \mid \acceptAct{a}{y}{Q} \mid \acceptAct{a}{z}{R}$
such that $C \hasType \{\ce{a}:\typeT_1,a:\typeT_2,a:\typeT_3\}$, then 
$C$ is rollback safe if $\typeT_1 \compliant \typeT_2$ and $\typeT_1 \compliant \typeT_3$. 
\end{exa}


\begin{exa}
Let us consider again the VOD example. 
As expected, the first \cherry\ collaboration defined in Ex.~\ref{example_syntax}, corresponding to the 
scenario described in Fig.~\ref{fig:scenario}(b), is not rollback safe, because 
the types of the two parties are not compliant. 
Indeed, the session types $\typeT_\texttt{U}$ and $\typeT_\texttt{S}$ associated by the type system to the user and 
the service processes, respectively, are as follows:
$$
\begin{array}{r@{\ \ }c@{\ \ }l}
\typeT_\texttt{U} & = & 
\outType{\strType}.\,
\inpType{\intType}.\,
\commitType.\,
\inpType{\strType}.\,
(\, \selType{l_{\textit{\textsf{HD}}}}.\, \inpType{\strType}.\, (\, \inpType{\strType}.\,\inactType  \ \choiceType\ \rollType\,)\\
&&\qquad\qquad\qquad\qquad \qquad\qquad
\choiceType \ 
\selType{l_{\textit{\textsf{SD}}}}.\, \inpType{\strType}.\, (\, \inpType{\strType}.\,\inactType \ \choiceType\ \abortType\,)\,)
\\[.2cm]
\typeT_\texttt{S} & = & 
\inpType{\strType}.\,
\outType{\intType}.\,
\outType{\strType}.\,
\branchType{\branch{l_{\textit{\textsf{HD}}}}{\commitType.\, \outType{\strType}.\,\outType{\strType}.\,\inactType}
\ ,\ 
\branch{l_{\textit{\textsf{SD}}}}{\commitType.\, \outType{\strType}.\,\outType{\strType}.\,\inactType}}
\end{array}
$$
Thus, the resulting initial configuration is 
$\initConf{\typeT_\texttt{U}}{\typeT_\texttt{S}}\conf{\typeT_\texttt{U}}{\typeT_\texttt{U}} \confcomp \conf{\typeT_\texttt{S}}{\typeT_\texttt{S}}$, 
which can evolve to the configuration 
$
\initConf{\typeT_\texttt{U}}{\typeT_\texttt{S}}\conf{\imposed{\typeT}}{\rollType} \confcomp \conf{\typeU}{\outType{\strType}.\inactType}
$,
with 
%$\typeT = \inpType{\strType}.\,
%(\, \selType{l_{\textit{\textsf{HD}}}}.\, \ldots \ \choiceType \ \selType{l_{\textit{\textsf{SD}}}}.\, \ldots\,)$
$\typeT = \inpType{\strType}.\, (\inpType{\strType}.\,\inactType  \ \choiceType\ \rollType)$
and 
$\typeU = \outType{\strType}.\,\outType{\strType}.\,\inactType$.
This configuration cannot evolve and is not in a final state (in fact, types 
$\rollType$ and $\outType{\strType}.\inactType$ are different from $\inactType$),
meaning that ${\typeT_\texttt{U}}$ and ${\typeT_\texttt{S}}$ are not compliant.

In the scenario described in Fig.~\ref{fig:scenario}(c), instead, the type of the server 
process is as follows:
$$
\begin{array}{r@{\ \ }c@{\ \ }l}
\typeT_\texttt{S}' & = & 
\inpType{\strType}.\,
\outType{\intType}.\,
\commitType.\,
\outType{\strType}.\,
\branchType{\branch{l_{\textit{\textsf{HD}}}}{\outType{\strType}.\,\outType{\strType}.\,\inactType}
\ ,\ 
\branch{l_{\textit{\textsf{SD}}}}{\outType{\strType}.\,\outType{\strType}.\,\inactType}}
\end{array}
$$
and we have $\typeT_\texttt{U} \compliant \typeT_\texttt{S}'$. 
The types of the processes depicted in Fig.~\ref{fig:scenario}(d) are:
$$
\begin{array}{r@{\ \ }c@{\ \ }l}
\typeT_\texttt{U}' & = & 
\outType{\strType}.\,
\inpType{\intType}.\,
\inpType{\strType}.\,
\commitType.\,
(\, \selType{l_{\textit{\textsf{HD}}}}.\, \ldots\ \choiceType \ 
\selType{l_{\textit{\textsf{SD}}}}.\, \ldots\,)
\\[.2cm]
\typeT_\texttt{S}'' & = & 
\inpType{\strType}.\,
\outType{\intType}.\,
\outType{\strType}.\,
\commitType.\,
\branchType{\branch{l_{\textit{\textsf{HD}}}}{\outType{\strType}.\,\outType{\strType}.\,\inactType}
\ ,\ 
\branch{l_{\textit{\textsf{SD}}}}{\outType{\strType}.\,\outType{\strType}.\,\inactType}}
\end{array}
$$
but we have $\typeT_\texttt{U}' \compliant\!\!\!\!/\ \ \typeT_\texttt{S}''$. 
Indeed, the corresponding initial configuration can evolve to the configuration 
$
\initConf{\typeT_\texttt{U}'}{\typeT_\texttt{S}''}\conf{\imposed{\selType{l_{\textit{\textsf{HD}}}}.\, \ldots}}{\rollType} 
\confcomp \conf{\branchType{\branch{l_{\textit{\textsf{HD}}}}{\ldots}, 
\branch{l_{\textit{\textsf{SD}}}}{\ldots}}}{\outType{\strType}.\inactType}
$, 
which again is deadlocked and not in a final state.
\end{exa}



==> tex/case_study.tex <==
% !TEX root = ../rev_sessions@concur.tex
\section{\Cherry\ at Work on an Online Loan Service}
\label{sec:case_study}

\todo[inline]{This section should be updated with a new case study from the reversibility literature or by connecting this to a real use case}

To shed light on the effectiveness of \cherry\ and the related notion of rollback safety, we consider 
a more realistic case study regarding an online service offering loans. 
The interactions with this service are organized in three phases: 
(1) negotiation of the loan rate, 
(2) definition of the duration, 
(3) payment of the monthly instalments.

Let us consider a scenario involving a client and a couple of loan services:
$$
\requestPrefix{loan}{x}.\ P_C 
\ \mid\ \acceptPrefix{loan}{y}.\ P_{S1} \ \mid\ \acceptPrefix{loan}{z}.\ P_{S2} 
$$
For more conveniently coding the processes, we will make use of 
variables that can be repeatedly assigned, denoted by $\varFont{x}$,
and the assignment primitive $\assign{\varFont{x}}{e}$,
which are offered by any common programming language. 

The \cherry\ process of the client is as follows :
$$
\begin{array}{r@{\ \ }c@{ \ \ }l}
P_C & = & 
\sendAct{x}{``loan\_req"}{\,}
\commitAct{\,}
\receiveAct{x}{x_{rate}:\intType}{\,}
\\
&&
\ifPi\ (x_{rate}\geq th_{unaccRate})
\\
&&
\quad\ \ 
\thenPi\ \abort\\
&&
\quad\ \ 
\elsePi\ \ifPi\ (th_{accRate}<x_{rate}<th_{unaccRate})
\\
&&
\quad\ \ \quad\ \
\thenPi\ 
\ifPi\ (eval(x_{rate}))\
\thenPi\ \abort\ \elsePi\ \roll
\\ 
&&
\quad\ \ \quad\ \
\elsePi\ \sendAct{x}{``accept"}{\,}
P_C^2\\
\\
P_C^2 & = & 
\assign{\varFont{d}}{getDuration()}.\,
\sendAct{x}{\varFont{d}}{\,}
\receiveAct{x}{x_{instalment}:\intType}{\,}
\\
&&
\ifPi\ (x_{instalment}>th_{maxAmount})\ 
\thenPi\ \roll\ \elsePi\ P_C^3\\
\\
P_C^3 & = & 
\recAct{X}{\,}
\ifPi\ (\varFont{d}\,==\,0)\ \thenPi\ \inact\ 
\\
&&
\qquad
\elsePi\ \sendAct{x}{payment(x_{instalment})}{\,}
\assign{\varFont{d}}{\varFont{d}-1}.\,
X
\end{array}
$$
The process is structured in three subprocesses, one for each service phase. 
In the first phase the client sends the data for the loan request and commits. 
Then, she receives a rate and compares it with given thresholds. If the proposed rate is 
unacceptable, the client immediately aborts the session, and possibly starts a new session 
with another service provider. If the rate is considered negotiable, the client 
performs a more detailed evaluation of the rate (by means of the $eval()$ function) 
and decides whether to 
abort (because, e.g., after some interactions the loan service does not offer a better rate) 
or to rollback to the committed point and evaluates another rate. Finally, if the rate is 
under the acceptable threshold, the client accepts it and passes to the second phase ($P_C^2$).
In this phase, the client send a loan duration, expressed in number of months, and gets
the corresponding monthly instalment amount. If the amount is too high, she rollbacks to 
the committed checkpoint, otherwise she passes to the third phase ($P_C^3$).
This consists of a loop where each iteration step corresponds to the payment
of a monthly instalment. 

Let us consider now the behaviour of the first service provider:
$$
\begin{array}{r@{\ \ }c@{ \ \ }l}
P_{S1} & = & 
\receiveAct{y}{y_{req}:\strType}{\,}
\assign{\varFont{r}}{rate(y_{req})}.\,
\sendAct{y}{\varFont{r}}{\,}
\receiveAct{y}{y_{duration}:\intType}{\,}
\assign{\varFont{d}}{y_{duration}}.\,\\
&&
\receiveAct{y}{y_{accept}:\strType}{\,}
\commitAct{\,}
\sendAct{y}{instalment(\varFont{r},\varFont{d})}{\,}
\\
&&
\recAct{Y}{\,}
\ifPi\ (\varFont{d}\,==\,0)\ \thenPi\ \inact\ 
\elsePi\ \receiveAct{y}{x_{payment}:\strType)}{\,}
\assign{\varFont{d}}{\varFont{d}-1}.\,
Y
\end{array}
$$
The interesting aspect here is that when the proposed rate is accepted, the service considers it fixed 
and hence commits the session. 
Now, if the client would perform a rollback after the evaluation of the monthly instalment amount, 
she would be able only to change the loan duration, but not to renegotiate the rate.
Indeed the client checkpoint has been overwritten by the service's commit action. 
This situation, undesirable for the client, is detected by our compliance check, which 
indeed identifies the collaboration as rollback unsafe. 

Finally, let the process $P_{S2}$ of the second service provider be like $P_{S1}$
but without the commit action. In this case, the service is compliant with the client 
and they can then safely interact. 








==> tex/conclusions_LONG.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex
\section{Conclusion and related work}
\label{sec:conclusion}
\vspace*{-.2cm}
%\todo[inline]{to add comparison with [24] and [TY16:RC]}
%
%\todo[inline]{be careful in comparison with uncontrolled approaches: in some works
%rollback is partially controlled, but it is implicit and the provided mechanisms are not 
%flexible as ours and hence reversibility results less programmable.
% }
% \todo[inline]{clarify why we allow to put commit in any place wrt approaches that 
% consider only choices as checkpoints: we are interested in commiting, hence 
% making irreversible, a given state of the session, hence the performed interactions
% (e.g., after a payment I would like to commit the session) }
% 
% \todo[inline]{to add a comparison to work on compensation by Hoare (POPL2005)}

This paper proposes rollback recovery primitives for session-based programming, which permit 
checkpointing session participants, rolling back to the last committed checkpoints, or
completely aborting a session.   
%
These primitives come together with session typing, enabling a design time compliance 
check that statically ensures 
checkpoint persistency properties (Lemma~\ref{lemma:safe_roll} and 
Theorem~\ref{lemma:undoability}) and session soundness 
(Theorems~\ref{th:roll_soundness} and \ref{th:com_soundness}), 
which differ from the properties of the existing (fully) reversible calculi. 
%
We have first illustrated our rollback recovery approach in the binary sessions setting, 
and then we have shown how it smoothly extends to the multiparty case.

\input{tex/rw}

%\paragraph*{Future work}

As future work, 
%we intend to deeply investigate on decidability of compliance. 
%We argue indeed that our compliance checking 
% is decidable. In fact, it boils down to check if the leaves of the 
%labelled transition system (LTS) produced by the semantics of the considered type configuration correspond to $\inactType$ types. 
%The decidability of this check depends on the finiteness of the LTS, which is ensured 
%by the fact that we have no static operators (i.e., parallel and restriction) within recursion. 
we plan to extend our approach to deal 
% multiparty sessions \cite{HYCJACM15}.
%To demonstrate the essence of our recovery mechanism, we have studied 
%it in the context of binary session types. Our results are extendable to multiparty session types 
%in which the parties that have created a session can only continue to interact along that 
%session. Hence our recovery framework can assure the same session progress property (Corollary~\ref{th:deadlock_freedom}) in sessions with more than two participants.
%
%Instead, dealing 
with sessions where parties can interleave interactions 
performed along different sessions. % could be more challenging.  
This requires to deal with subordinate sessions, which may affect enclosing sessions
by performing, e.g., commit actions that make some interaction of the enclosing sessions 
irreversible, similarly to \textit{nested transactions}~\cite{Weikum92conceptsand}.
To tackle this issue it would be necessary to extend the notion of compliance 
relation  to take into account possible partial commits (in case of nested sub-sessions) that
could be undone at the top level if a rollback is performed.
  

==> tex/host_calculus2.tex <==
% !TEX root = ../reversible_sessions@rc.tex
\section{Background on session-based $\pi$-calculi}
\label{sec:host_calculus}

\todo[inline]{This is a background session to be used in the initial phase the work 
as reference for the considered versions of \pic\ (notation, syntax, semantics, etc.). 
Later, to save space, we could omit it and incorporate the necessary notions in the 
other sections.}

In this section, we give the basic definitions concerning two variants of the \pic, 
enriched with primitives for managing binary and multiparty sessions, respectively.

\medskip

\noindent
\textbf{Binary session calculus.}
The syntax of the binary session \pic\ \cite{YoshidaV07} relies on the following base sets: 
\emph{variables} (ranged over by $x$), storing values;
\emph{shared channels} (ranged over by $a$), used to initiate sessions;
\emph{session channels} (ranged over by $s$), consisting on pairs of \emph{endpoints} 
(ranged over by $s$, $\ce{s}$) used by the two parties to exchange values within an established session;
\emph{labels} (ranged over by $l$), used to select and offer branching choices;
and  \emph{process variables} (ranged over by $X$), used for recursion. 
Letter $u$ denotes \emph{shared identifiers}, i.e. shared channels and variables together; 
letter $\genSession$ denotes \emph{generic session endpoints}, i.e. they can be either of 
the form $s$ or $\ce{s}$; 
letter $\sessId$ denotes \emph{session identifiers}, i.e. session endpoints and variables together;
letter $c$ denotes \emph{channels}, i.e. session channels and shared channels together. 
\emph{Values}, including booleans, integers, shared channels
and session endpoints, are ranged over by $v$.

\emph{Processes} (ranged over by $P$) and 
\emph{expressions} (ranged over by $e$ and defined by means of 
a generic expression operator $\text{op}$ representing standard operators on boolean and integer values) are 
given by the grammar in Figure~\ref{fig:syntax_pi}. 
\begin{figure}[t]
\centering
\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ \ }l@{}}
	$P$ & ::= & & \textbf{Processes} \\
	&             & $\requestAct{u}{x}{P}$ \ $\mid$ \ $ \acceptAct{u}{x}{P}$ 
	                   \ $\mid$ \
	                   $\sendAct{\sessId}{e}{P}$ \ $\mid$ \ $\receiveAct{\sessId}{x}{P}$ & \ request, accept ,output, input\\
	& $\mid$ & $\selectAct{\sessId}{l}{P}$ \ $\mid$ \ $ \branchAct{\sessId}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$ 
	                   \ $\mid$ \
	                   $\inact$ \ $\mid$ \ $P_1 \!\mid\! P_2$ & \ selection, branching, inact, parallel\\
	& $\mid$ & $ \res{c}\, P$ \ $\mid$ \ $\ifthenelseAct{e}{P_1}{P_2}$ 
	                   \ $\mid$ \
	                   $X$ \ $\mid$ \ $\recAct{X}{P}$ & \ choice, restriction, recursion
	\\[.2cm]
	$e$ & ::= & \ \ $v$ \ $\mid$ \ $\text{op}(e_1,\ldots,e_n)$  & \textbf{Expressions}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Binary session calculus: syntax}
	\label{fig:syntax_pi}
\end{figure}

The operational semantics of the calculus is given in terms of a structural congruence and of a reduction relation, 
and is only defined for \emph{closed} terms, i.e. terms without free variables. 
The \emph{structural congruence}, written $\congr$, is standard 
\iftr
(cf. Figure~\ref{fig:congruence_pic} in Appendix).
\else
(see \cite{RC_TR}).
\fi
The \emph{reduction relation}, written $\red$, is the smallest relation on 
closed processes generated by the rules in Figure~\ref{fig:reduction_pic}.
We resort to the auxiliary function $\expreval{\cdot}{\,}$ 
for evaluating closed expressions: 
$\expreval{e}{v}$ says that expression $e$ evaluates to value $v$. 
Notationally, for $P$ a process, $\freev{P}$ denotes the set of free variables in $P$, 
and $\freese{P}$ the set of free session endpoints. 
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{l@{\qquad}l@{\qquad }l}
	$\requestAct{a}{x_1}{P_1}\ \mid \ \acceptAct{a}{x_2}{P_2}$
	$\ \red\ $
	$\res{s}(P_1\subst{\ce{s}}{x_1} \mid P_2\subst{s}{x_2})$ 
	& $s,\ce{s} \notin \freese{P_1,P_2}$ & \rulelabel{Con}
	\\[.2cm]
	$\sendAct{\ce{k}}{e}{P_1} \ \mid \ \receiveAct{k}{x}{P_2}$
	$\ \red\ $
	$P_1 \mid P_2\subst{v}{x}$
	& $\expreval{e}{v}$ & \rulelabel{Com}
	\\[.2cm]
	$\selectAct{\ce{k}}{l_i}{P} \ \mid \ \branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
	$\ \red\ $
	$P \mid P_i$
	& $1 \leq i \leq n$ & \rulelabel{Lab}
	\\[.2cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \red\ $
	$P_1$
	& $\expreval{e}{\ctrue}$ & \rulelabel{If1}
	\\[.2cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \red\ $
	$P_2$
	& $\expreval{e}{\cfalse}$ & \rulelabel{If2}
	\\[.1cm]
	\end{tabular}
	\begin{tabular}{c}
	$
	\infer[$\,\rulelabel{Par}$]{P_1 \!\mid\! P_2 \ \red\ P_1' \!\mid\! P_2}
	{P_1 \ \red\ P_1'}
	$	
	\qquad
	$
	\infer[$\,\rulelabel{Res}$]{\res{c}P \ \red\ \res{c}P'}
	{P \ \red\ P'}
	$
	\qquad
	$
	\infer[$\,\rulelabel{Str}$]{P_1 \ \red\ P_2}
	{P_1 \congr P_1'\ \red\ P_2' \congr P_2}
	$
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Binary session calculus: reduction relation}
	\label{fig:reduction_pic}
\end{figure*}
We comment on salient points. 
A new session is established when two parallel processes synchronise 
via a shared channel $a$; this results on the generation of a fresh (private) session 
channel whose endpoints are assigned to the two session parties (rule \rulelabel{Con}).
Along a session, the two parties can exchange values (for data- and channel-passing, 
rule \rulelabel{Com}) and labels (for branching selection, rule \rulelabel{Lab}). 
The other rules are standard and state that: 
conditional choice evolves according to the evaluation of the expression argument 
(rules \rulelabel{If1} and \rulelabel{If2});
if a part of a larger process evolves, the whole process evolves accordingly 
(rules \rulelabel{Par} and \rulelabel{Res});
and structural congruent processes have the same reductions (rule \rulelabel{Str}). 

\label{sec:typingPic}

The syntax of \emph{sorts} (ranged over by $S$) and \emph{types} (ranged over by $\alpha$, 
$\beta$) used in the \emph{binary session type discipline} is defined in Figure~\ref{fig:typeSyntax}.
\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ }l@{}}
	$S$ & ::= &  & \textbf{Sorts}\\
	&             & $\boolType$ \quad $\mid$ \quad $\intType$ \quad $\mid$ \quad $\sharedChanType{\alpha}$ & \ boolean, integer, shared channel
	\\[.2cm]
	$\alpha$ & ::= &  &  \textbf{Types}\\
	&             & $\outType{S}.\alpha$ \quad $\mid$ \quad $\thrType{\beta}.\alpha$ \quad $\mid$ \quad $\inpType{S}.\alpha$  
	\quad $\mid$ \quad $\catType{\beta}.\alpha$ & \ output, input\\
	& $\mid$ & $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ 
	\ \  $\mid$ \ \ $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$
	& \ selection, branching\\			
	& $\mid$ & $\inactType$ \quad $\mid$ \quad $t$ \quad $\mid$ \quad $\recType{t}.\alpha$ & \ end, recursion
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Binary session calculus: sorts and types}
	\label{fig:typeSyntax}
	\vspace*{-.2cm}
\end{figure}
The type $\outType{S}.\alpha$ represents the behaviour of first outputting a value of sort $S$, 
then performing the actions prescribed by type $\alpha$; 
type $\thrType{\beta}.\alpha$ represents a similar behaviour, which starts with session output 
(\emph{delegation}) instead; 
types $\inpType{S}.\alpha$ and $\catType{\beta}.\alpha$ are the dual ones, 
receiving values instead of sending. 
Type $\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ represents the behaviour 
which would select one of $l_i$ and then behaves as $\alpha_i$, according to the selected $l_i$ 
(internal choice). 
Type $\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}$ describes a branching 
behaviour: it waits with $n$ options, and behave as type $\alpha_i$ if the $i$-th action is selected 
(external choice).
Type $\inactType$ represents inaction, acting as the unit of sequential composition.
Type $\recType{t}.\alpha$ denotes a recursive behaviour, representing the behaviour that starts 
by doing $\alpha$ and, when variable $t$ is encountered, recurs to $\alpha$ again. 

\emph{Typing judgements} are of the form $\basis;\sorting \judge P \hasType \typing$,
where $\basis$, $\sorting$ and $\typing$, called \emph{basis}, \emph{sorting} and \emph{typing}
respectively,  are finite partial maps from shared identifiers to sorts, 
from session identifiers to types, and from process variables to typings, respectively
Intuitively,  the judgement $\basis;\sorting \judge P \hasType \typing$ 
stands for ``under the environment $\basis;\sorting$, process $P$ has typing $\typing$''. 
The axioms and rules defining the typing system are standard 
\iftr
(cf. Figure~\ref{fig:typingSysytem} in Appendix).
\else
(see \cite{RC_TR}).
\fi
 
%\begin{example}[Buyer-Seller protocol]\label{ex:BS}
%We show how the protocol in Figure~\ref{fig:examples}.(a) is rendered in the variant of \pic\
%with binary sessions. 
%The behaviour of Buyer is described by the following process:
%$$
%\small
%\begin{array}{@{}r@{\ }c@{\ }l}
%Buyer & \triangleq & 
%\requestAct{a}{x}{\,}
%\sendAct{x}{``\mathit{The\ Divine\ Comedy}"}{\,}
%\receiveAct{x}{x_{quote}}{}\\
%&& 
%\ifPi\ \, x_{quote} \leq 20\ \
%\thenPi\ \,
%\selectAct{x}{l_{ok}}{\,} 
%\sendAct{x}{addr()}{\,}
%\receiveAct{x}{x_{date}}{\,P}
%\ \ \elsePi\ \
%\selectAct{x}{l_{quit}}{\,\inact} 
%\end{array}
%$$
%This Buyer is interested in buying the Divine Comedy and is willing to pay not more than $20$ euros.  
%The Seller participant instead is rendered as follows:
%$$
%\small
%\begin{array}{@{}r@{\ }c@{\ }l}
%Seller & \triangleq & 
%\acceptAct{a}{z}{\,}
%\receiveAct{z}{z_{title}}{\,}
%\sendAct{z}{quote(z_{title})}{\,}
%\branchAct{z}{\branch{l_{ok}\!\!}{\!\!
%\receiveAct{z}{z_{addr}}{\,}
%\sendAct{z}{date()}{Q\, }
%} \branchSep 
%\branch{l_{quit}\!\!}{\!\!\inact}}
%\\
%\end{array}
%$$
%Note that  $\mathit{addr()}$, $\mathit{quote()}$ and $\mathit{date()}$ are used to get a buyer address,
%a quote for a given book, and the delivery date, respectively.
%The overall specification is $Buyer \mid Seller$. 
%\end{example}



==> tex/host_calculus_multi.tex <==
% !TEX root = ../reversible_sessions@rc.tex
\smallskip

\noindent
\textbf{Multiparty session calculus.}
The base sets for the synchronous multiparty session calculus \cite{KouzapasY14} are the same
of the binary case, except for \emph{session endpoints}, which now are denoted by 
$s\mendpoint{\role{p}}$, with $\role{p}$,$\role{q}$ ranging over \emph{roles} 
(represented as natural numbers). Thus, \emph{session identifiers} $\sessId$ 
now range over session endpoints $s\mendpoint{\role{p}}$ or variables $x$.

The syntax of the calculus is defined by the grammar in Figure~\ref{fig:syntax_multipi},
where expressions $e$ are defined as in the binary case (with values that extends to 
multiparty session endpoints). 
\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\,}l@{\ }l@{}}
	$P$ & ::= &  & \textbf{Processes}\\
	&             & $\mrequestAct{u}{\role{p}}{x}{P}$ \ \ $\mid$ \ \ $\macceptAct{u}{\role{p}}{x}{P}$ 
	                   \ \ $\mid$ \ \
	                   $\msendAct{\sessId}{\role{p}}{e}{P}$ \ \ $\mid$ \ \ $\mreceiveAct{\sessId}{\role{p}}{x}{P}$ 
	               & \ request, accept, output, input\\
	& $\mid$ & $\mselectAct{\sessId}{\role{p}}{l}{P}$ \ \ $\mid$ \ \ 
	                  $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1} \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
	                  \ \ $\mid$ \ \ $\inact$ \ \ $\mid$ \ \ $P_1 \!\mid\! P_2$
	                  & \ selection, branching, inact, par.\\
	& $\mid$ &  $\ifthenelseAct{e}{P}{Q}$ \ \ $\mid$ \ \ $\res{c}\, P$
	                    \ \ $\mid$ \ \ 
	                   $X$ \ \ $\mid$ \ \  $\recAct{X}{P}$ 
	& \ choice, restriction, recursion
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Multiparty session calculus: syntax}
	\label{fig:syntax_multipi}
\end{figure}
Primitive $\mrequestAct{u}{\role{p}}{x}{P}$ initiates a new session through 
identifier $u$ on the other multiple participants, each one of the form 
$\macceptAct{u}{\role{q}}{x}{P_{\role{q}}}$ where $1 \leq \role{q} \leq \role{p}-1$. 
Variable $x$ will be substituted with the session endpoint used for the interactions
inside the established session. 
Primitive $\msendAct{\sessId}{\role{p}}{e}{P}$ denotes the intention of sending a value to 
role $\role{p}$; similarly, process $\mreceiveAct{\sessId}{\role{p}}{x}{P}$ denotes the intention 
of receiving a value from role $\role{p}$. Selection and branching behave in a similar way. 

As usual the operational semantics is given in terms of a structural congruence and of a 
reduction relation. 
The rules defining the structural congruence are the same ones used for the binary calculus%
\iftr
~(Figure~\ref{fig:congruence_pic} in Appendix~\ref{app:background}), 
\else , 
\fi
where the rule for the scope extension of session channels takes into account the new form 
of session endpoints. 
The \emph{reduction relation} $\red$, instead, is the smallest relation on 
closed processes generated by the rules \rulelabel{If1}, \rulelabel{If2},
\rulelabel{Par}, \rulelabel{res} and \rulelabel{Str} in Figure~\ref{fig:reduction_pic},
and the additional rules in Figure~\ref{fig:reduction_pic_multi}.
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{@{}l@{\hspace*{-1.3cm} }r@{\quad}r@{}}
	$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i=\{1,..,n-1\}}\macceptAct{a}{i}{x}{P_i}$ 
	$\ \ \red\ \ $
	&
	$s \notin \freese{P_i}$ with $i=\{1,..,n\}$
	&
	\rulelabel{M-Con}
	\\
	\qquad 	
	$\res{s}(P_n\subst{s\mendpoint{n}}{x} \mid \prod_{i=\{1,..,n-1\}}P_i\subst{s\mendpoint{i}}{x})$ 	
	\\[.3cm]
	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P}
	\, \mid \, \mreceiveAct{s\mendpoint{\role{q}}}{\role{p}}{x}{Q}$
	$\ \ \red\ \ $
	$P \mid Q\subst{v}{x}$
	& $\expreval{e}{v}$ & \rulelabel{M-Com}
	\\[.3cm]
	$\mselectAct{s\mendpoint{\role{p}}}{\role{q}}{l_i}{P}
	\, \mid \, \mbranchAct{s\mendpoint{\role{q}}}{\role{p}}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}}$
	$\ \ \red\ \ $
	$P \mid P_i$
	& $1 \leq i \leq n$ & \rulelabel{M-Lab}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Multiparty session calculus: reduction relation (excerpt of rules)}
	\label{fig:reduction_pic_multi}	
\end{figure*}
We comment on salient points.
Rule \rulelabel{M-Con} synchronously initiates a session by requiring all session 
endpoints be present for a synchronous reduction, where each role $\role{p}$ 
creates a session endpoint $s\mendpoint{\role{p}}$ on a fresh session channel $s$. 
The participant with the maximum role ($\mrequestAct{a}{n}{x}{P_n}$) is 
responsible for requesting a session initiation. Rule \rulelabel{M-Com} defines how 
a party with role $\role{p}$ sends a value to the receiving party with role $\role{q}$. 
Selection and branching are defined in a similar way (rule \rulelabel{M-Lab}). 

The type discipline of this synchronous multiparty session calculus is simpler 
than the asynchronous one in \cite{HYCJACM15}, but it is much more elaborate than the binary 
case, as it considers global and local types. Therefore, due to lack of space, we 
relegate the definitions of types, as well as the rules of the corresponding type system,
to 
\iftr
Appendix~\ref{app:background}, 
\else
the companion technical report \cite{RC_TR}
\fi
and refer the interested reader to \cite{KouzapasY14} for a detailed account.

%\begin{example}[Two-Buyers-Seller protocol]\label{ex_BBS}
%We show how the protocol in Figure~\ref{fig:examples}.(b) is rendered in the variant of \pic\
%with the multiparty sessions. 
%The behaviour of Buyer1 and Buyer2 are described by the following processes:
%$$
%\small
%\begin{array}{r@{\ }c@{\ }l}
%Buyer1 & \triangleq & 
%\mrequestAct{a}{3}{x}{\,}
%\msendAct{x}{1}{``\mathit{The\ Divine\ Comedy}"}{\,}
%\mreceiveAct{x}{1}{x_{quote}}{\,}
%\msendAct{x}{2}{split(x_{quote})}{\,P_1}
%\\[.2cm]
%Buyer2 & \triangleq & 
%\macceptAct{a}{2}{y}{\,}
%\mreceiveAct{y}{1}{y_{quote}}{\,}
%\mreceiveAct{y}{3}{y_{contrib}}{\,}
%\ifPi\ \ y_{quote}-y_{contrib} \leq 10 \\
%& & 
%\thenPi\ \
%\mselectAct{y}{1}{l_{ok}}{\,} 
%\msendAct{y}{1}{addr()}{\,}
%\mreceiveAct{y}{1}{y_{date}}{\,P_2}
%\ \
%\elsePi\ \
%\mselectAct{y}{1}{l_{quit}}{\,\inact} 
%\end{array}
%$$
%Now, Buyer1 divides the quote by means of the $split()$ function. 
%The Seller process is similar to the binary case, but for the form of session 
%endpoints:
%$$
%\small
%\begin{array}{@{}r@{\ }c@{\ }l@{}}
%Seller & \triangleq & 
%\macceptAct{a}{1}{z}{\,}
%\mreceiveAct{z}{3}{z_{title}}{\,}
%\msendAct{z}{2}{quote(z_{title})}{\,}
%\msendAct{z}{3}{\mathit{lastQuote}(z_{title})}{\,}\\
%&& 
%\mbranchAct{z}{2}{\branch{l_{ok}\!\!}{\!
%\mreceiveAct{z}{2}{z_{addr}}{\,}
%\msendAct{z}{2}{date()}{P_3\, }
%} \branchSep\, 
%\branch{l_{quit}\!\!}{\!\inact}}
%\\
%\end{array}
%$$
%where $\mathit{lastQuote}()$ simply returns the last quote computed for a 
%given book. 
%\end{example}
%
%


==> tex/multiparty.tex <==
% !TEX root = ../rev_sessions@coord19.tex
\section{Extension to multiparty sessions}
\label{sec:multiparty}

We discuss in this section how to extend \cherry, its type discipline,
the compliance checking and the related results, to multiparty 
sessions \cite{KouzapasY14}.

The base sets for the multiparty syntax of \cherry\  are the same
of the binary case, except for \emph{session endpoints}, which now are denoted by 
$s\mendpoint{\role{p}}$, with $\role{p}$,$\role{q}$ ranging over \emph{roles} 
(represented as natural numbers). 
Thus, \emph{session identifiers} $\sessId$ 
now range over session endpoints $s\mendpoint{\role{p}}$ or variables $x$.
%
%The runtime syntax of multiparty \cherry\ is defined by the grammar in 
%Fig.~\ref{fig:syntax_cherry_pi_multi}, where expressions $e$ are defined as in the binary case (with values that extends to 
%multiparty session endpoints). 
% %
%\begin{figure}[t]
%\small
%	\begin{tabular}{@{}r@{ }c@{\ }l@{\ \ }l@{}}
%	$C$ & ::= & $\cdots$    $\mid$ 
%	                   $\mrequestAct{a}{\role{p}}{x}{P}$  $\mid$  $\macceptAct{a}{\role{p}}{x}{P}$
%	                   & \!\!\!\!\!\!\!\!\!\textbf{Collaborations}
%	\\[.3cm]
%	$P$ & ::= &  $\cdots$  $\mid$ 
%                                        $\msendAct{\sessId}{\role{p}}{e}{P}$ 
%		         $\mid$  $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ 	
%		         $\mid$  $\mselectAct{\sessId}{\role{p}}{l}{P}$ 
%		         $\mid$  $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
%		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
%			& \ \ \ \textbf{Processes}
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.4cm}	
%	\caption{Multiparty \cherry\ runtime syntax (the omitted parts are as in Fig.~\ref{fig:syntax_cherry_pi_ext}).}
%	%\vspace*{.2cm}	
%	\label{fig:syntax_cherry_pi_multi}
%\end{figure}
%
Primitive $\mrequestAct{a}{\role{p}}{x}{P}$ initiates a new session through 
identifier $a$ on the other multiple participants, each one of the form 
$\macceptAct{a}{\role{q}}{x}{P_{\role{q}}}$ where $1 \leq \role{q} \leq \role{p}-1$. 
Variable $x$ will be substituted with the session endpoint used for the interactions
inside the established session. 
Primitive $\msendAct{\sessId}{\role{p}}{e}{P}$ denotes the intention of sending a value to 
role $\role{p}$; similarly, process $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ denotes the intention 
of receiving a value from role $\role{p}$. Selection and branching are extended in a similar way. 


%As usual the operational semantics is given in terms of a structural congruence 
%and of a reduction relation. 
%The rules defining the structural congruence are standard, while 
%%the same ones used for the binary calculus,
%%where the rule for the scope extension of session channels takes into account the new form 
%%of session endpoints. 
%%The reduction relation, instead, is the smallest relation on 
%%closed collaborations generated by the rules (an excerpt of which are) reported 
%%in Figure~\ref{fig:reduction_pic_multi}.
%the forward and backward reduction relations are given by the rules 
%in Fig.~\ref{fig:reduction_pic_multi}.
%%
%\begin{figure*}[t]
%	\centering
%	\small
%        \begin{tabular}{@{ }c@{}}
%	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
%	\auxrel{\!\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}\!} \!P$
%	\ ($\expreval{e}{v}$)
%	 \rulelabel{M-P-Snd}
%	\qquad
%	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y\!:\!S}{P}
%	 \auxrel{\!\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}\!\!} \!P$
%	\rulelabel{M-P-Rcv}
%	\\[.5cm]
%	\end{tabular}	
%	\\
%	\begin{tabular}{@{}l@{}}
%		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
%	$\ \ \fwred\ \ $
%	\\[.1cm]
%	\quad 	
%	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$
%	\qquad\quad\qquad\qquad\qquad\ \
%	$I\!=\!\{1,..,n\!-\!1\}$\quad
%	\rulelabel{M-F-Con}	
%	\\[.1cm] 	
%	\quad 	
%        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
%        \!\mid\! 
%        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
%	\\[.5cm]
%	\end{tabular}
%	\begin{tabular}{@{}c@{}}	
%	$
%	\infer[$\rulelabel{M-F-Com}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P_1'
%	& & 
%	P_2 \auxrel{\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}} P_2'	
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-F-Cmt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \fwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{P'} P' 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
%	}
%	{
%	P \auxrel{\commitLab} P'
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-B-Rll}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} Q 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
%	}
%	{
%	P \auxrel{\rollLab} P'
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	C}
%	{
%	P \auxrel{\abortLab} P'
%	}
%	$
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.4cm}	
%	\caption{Multiparty \cherry\ semantics: forward and backward reductions (excerpt of rules).}
%	\label{fig:reduction_pic_multi}
%	\vspace*{.7cm}	
%\end{figure*}
%%
%%The forward and backward reduction relations are given by the rules 
%%in Fig.~\ref{fig:reduction_pic_multi}(upper part).
%%
%We comment on salient points.
%Rule \rulelabel{M-F-Con} synchronously initiates a session by requiring all session 
%endpoints be present for a forward reduction, where each role $\role{p}$ 
%creates a session endpoint $s\mendpoint{\role{p}}$ on a fresh session channel $s$. 
%The participant with the maximum role %($\mrequestAct{a}{n}{x}{P_n}$) 
%is responsible for requesting a session initiation. Rule \rulelabel{M-F-Com} defines how 
%a party with role $\role{p}$ synchronously sends a value to the receiving party with role $\role{q}$. 
%Rules \rulelabel{M-F-Cmt}, \rulelabel{M-B-Rll} and \rulelabel{M-B-Abt} are similar to 
%those of the binary case, and affect all participants within the considered session. 
%
%%The syntax of session types extends to multiparty as shown in Fig.~\ref{fig:typeSyntax_cherry_multi}. 
%%%
%%\begin{figure}[t]
%%	\centering
%%	\small
%%	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
%%	$\typeT\!$ & ::= &  &\!\!  \ldots   $\mid$  
%%	$\moutType{\role{p}}{\role{q}}{S}.\typeT$  $\,\mid\,$ 
%%	$\minpType{\role{p}}{\role{q}}{S}.\typeT$   $\,\mid\,$ 
%%	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	$\,\mid\,$  
%%	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}$
%%	\ \ \textbf{Types}
%%	\\[.1cm]
%%	\hline
%%	\end{tabular}
%%	\vspace*{-.6cm}	
%%	\caption{Multiparty \Cherry\ type syntax 
%%	(the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry}).
%%	}
%%	\label{fig:typeSyntax_cherry_multi}
%%	%\vspace*{.5cm}
%%\end{figure}
%%
%The session types for output ($\moutType{\role{p}}{\role{q}}{S}.\typeT$)
%and input ($\minpType{\role{p}}{\role{q}}{S}.\typeT$) are extended with information 
%about the interacting roles; selection and branching types are similarly extended. 
%In the type inference, when one of such role is unknown, it is used
%a placeholder $\_$ to be filled with a given role; $\typeT\cdot\role{p}$ denotes the type obtained 
%from $\typeT$ by filling all its placeholders with the role $\role{p}$.
%%
%%The \cherry\ type system extends accordingly; as an example we 
%%report below the rules for output and input:
%%$$
%%{\small
%%	\infer{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
%%	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
%%	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
%%\qquad\quad
%%	\infer{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
%%	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
%%	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
%%}
%%$$
%The \cherry\ type system extends accordingly, as shown in Fig.~\ref{fig:typingSystem_multi}.
%
%\input{tex/multiparty_type_system}
%
%
%
%The semantics of type configurations is defined only for filled types.
%%
%Semantic rules in Fig.~\ref{fig:typeSemantics_ext_multi}
%are the natural extension of those for the binary case.
%Rule \rulelabel{M-TS-Com} shows that communication affects only 
%the two interacting parties, without modifying any checkpoint.
%Rule \rulelabel{M-TS-Cmt} sets the checkpoint of the committing party and 
%sets an imposed checkpoint for each other party that has performed at least 
%an action from its current checkpoint. 
%Rule \rulelabel{M-TS-Rll} rolls all parties back to their checkpoints,
%provided that the checkpoint of the party requesting the rollback  is not imposed. 
%Rule \rulelabel{M-TS-Abt} brings all parties back to the initial configuration. 
%
% 
%\begin{figure}[t]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{\qquad\quad}l@{}}
%	$\moutType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Snd}	
%	& 
%	$\minpType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\minpType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Rcv}  
%	\\[.5cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[$\rulelabel{M-TS-Com}$]
%	{\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\conf{\checkpointType{\typeU}_j}{\typeT_j}
%	\confcomp 	
%	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\\[.1cm] 
%	\quad
%	\typered
%	\ \
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i'} 
%	\confcomp 
%	\conf{\checkpointType{\typeU}_j}{\typeT_j'}
%	\confcomp 	
%	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\end{array}}
%	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
%	& &
%	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
%	$
%	}
%	\\[.8cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[\ \	
%	 \checkpointType{\typeU}_h' \! =\!\! 
%	 \left\{
%	 \begin{array}{ll}
%	 \checkpointType{\typeU}_h & \textrm{if}\ \checkpointType{\typeU}_h = \typeT_h \\
%	 \imposed{\typeT_h} & \textrm{otherwise}
%	 \end{array}
%	 \right.
%	\ \
%	$\rulelabel{M-TS-Cmt}$
%	]	
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\\
%	\quad
%	\typered
%	\ \
%	\minitConf{\typeT^I}
%	\conf{\typeT_i'}{\typeT_i'} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h}
%	\end{array}
%	}
%	{\typeT_i \typeTrans{\commitLab} \typeT_i'}	
%	$
%	}
%	\\[.8cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\typeU_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\
%	\typered
%	\
%	\minitConf{\typeT^I}
%	\conf{\typeU_i}{\typeU_i}  
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeU_h}
%	\end{array}
%	}
%	{\hspace*{4cm}
%	\typeT_i \typeTrans{\rollLab} \typeT_i' 
%	\hspace*{4cm}
%	$\rulelabel{M-TS-Rll}$
%	}	
%	$
%	}
%	\\[.8cm]	
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[$\rulelabel{M-TS-Abt}$]
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\
%	\typered
%	\
%	\minitConf{\typeT^I}
%	\prod_{k\in I}\conf{\typeT^k}{\typeT^k}
%	\end{array}
%	}
%	{\typeT_i \typeTrans{\abortLab} \typeT_i' }	
%	$	
%	}
%	\\[.4cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.3cm}	
%	\caption{Multiparty \cherry\ type semantics (excerpt of rules, 
%	where $I=\{1,\ldots,n\}$, $i,j\in I$, and $\typeT^{I}$ denotes $\typeT^1,\ldots,\typeT^n$).}
%	\label{fig:typeSemantics_ext_multi}
%	%\vspace*{-.2cm}
%\end{figure}

\begin{figure*}[t]
	\hspace{-.3cm}
	\small
	\begin{tabular}{@{}l@{}}
	%
	\begin{tabular}{l@{\ \ }l@{\qquad\ }l@{\ \ }l@{\ }l}
	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
	\auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P$
	\ $\expreval{e}{v}$ 
	& \rulelabel{M-P-Snd}
	&
	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y:S}{P}
	 \auxrel{\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}} P$
	& \rulelabel{M-P-Rec}
	\\[.2cm]
	\end{tabular}	
	\\
	\begin{tabular}{@{}l@{}}
		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
	$\ \ \fwred\ \ $
	\qquad\qquad\qquad\quad\qquad\qquad\ \
	$I=\{1,..,n-1\}$\quad
	\rulelabel{M-F-Con}	
		\\[.1cm]
	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n} \mid  \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$ 
        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
        \!\mid\! 
        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
	\\[.3cm]	
	$
	\infer{
	\loggedShort{\ce{\genSession}}{Q_1} P_1 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2
	\fwred
	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
	}
	{
	P_1 \auxrel{\!\!\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}\!\!} P_1'
	\quad
	P_2 \auxrel{\!\!\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}\!\!} P_2'	
	\hspace*{.3cm}
	$\rulelabel{M-F-Com}$
	}
	$
	\quad\ \ 
	$
	\infer{
	\singleSession{s}{C}(
	\loggedShort{\ce{\genSession}}{Q} P 
	 \mid 
	\prod_{i\in I}\loggedShort{\genSession}{Q_i} P_i)
	\bwred 
	C}
	{\hspace*{1.3cm}
	P \auxrel{\abortLab} P'
	\hspace*{1cm}
	$\rulelabel{M-B-Abt}$
	}
	$	
	\\[.2cm]
	$
	\infer[$\rulelabel{M-F-Cmt}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \fwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{P'} P' 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
	}
	{
	P \auxrel{\commitLab} P'
	}
	$
	\\[.2cm]
	$
	\infer[$\rulelabel{M-B-Rll}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \bwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} Q 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
	}
	{
	P \auxrel{\rollLab} P'
	}
	$
	\\[.3cm]
	\end{tabular}
	%
	\\
	\hline
	\hspace{6cm}\textsc{Typing Rules }
	\\[.2cm]
	%
	\begin{tabular}{@{}c@{}}
	$
	\infer{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
\qquad\quad
	\infer{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
	$
	\end{tabular}
	%
	\\[.5cm]
	\hline
	\hspace{6cm}\textsc{Typing Semantics}
	\\[.0cm]
	%	
	\begin{tabular}{@{}c@{}}
		$
	\begin{array}{l}
	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
	\, ,\,
	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
	\Rightarrow
	\		
	\minitConf{\typeT^I}\!
	\conf{\checkpointType{\typeU}_i\!}{\!\typeT_i} 
	\!\confcomp\! 
	\conf{\checkpointType{\typeU}_j\!}{\!\typeT_j}
	\!\confcomp\! 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h\!}{\!\typeT_h}
	\\
	\hspace*{5.1cm}
	\typered\minitConf{\typeT^I}\!
	\conf{\checkpointType{\typeU}_i\!}{\!\typeT_i'} 
	\!\confcomp\! 
	\conf{\checkpointType{\typeU}_j\!}{\!\typeT_j'}
	\!\confcomp\! 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h\!}{\!\typeT_h}
	\end{array}
	$
	\end{tabular}
	\\[.4cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Multiparty \cherry: operational semantics, typing system, type semantics (excerpt of rules).}
	\label{fig:reduction_pic_multi}
	\vspace*{-.5cm}	
\end{figure*}

%As usual the operational semantics is given in terms of a structural congruence and of a 
%reduction relation. 
%The rules defining the structural congruence are the same ones used for the binary calculus,
%where the rule for the scope extension of session channels takes into account the new form 
%of session endpoints. 
%The reduction relation, instead, is the smallest relation on 
%closed collaborations generated by the rules (an excerpt of which are) reported 
%in Figure~\ref{fig:reduction_pic_multi}.
The forward and backward reduction relations are given by the rules 
in Fig.~\ref{fig:reduction_pic_multi}(upper part).
%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{l@{\ \ }l@{\qquad\qquad\ }l@{\ \ }l@{\ }l}
%	\\[-.9cm]
%	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
%	\auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P$
%	\quad $\expreval{e}{v}$ 
%	& \rulelabel{M-P-Snd}
%	&
%	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y:S}{P}
%	 \auxrel{\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}} P$
%	& \rulelabel{M-P-Rec}
%	\\[.2cm]
%	\end{tabular}	
%	%
%	\begin{tabular}{@{}l@{}}
%		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
%	$\ \ \fwred\ \ $
%	\qquad\qquad\qquad\quad\qquad\qquad\qquad\qquad
%	$I=\{1,..,n-1\}$\quad
%	\rulelabel{M-F-Con}	
%		\\[.1cm]
%	\qquad 	
%	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$ 
%        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
%        \!\mid\! 
%        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
%	\\[.3cm]	
%	$
%	\infer{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P_1'
%	\quad
%	P_2 \auxrel{\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}} P_2'	
%	\hspace*{.3cm}
%	$\rulelabel{M-F-Com}$
%	}
%	$
%	\qquad
%	$
%	\infer{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	C}
%	{\hspace*{1.7cm}
%	P \auxrel{\abortLab} P'
%	\hspace*{1.5cm}
%	$\rulelabel{M-B-Abt}$
%	}
%	$	
%	\\[.2cm]
%	$
%	\infer[$\rulelabel{M-F-Cmt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \fwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{P'} P' 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
%	}
%	{
%	P \auxrel{\commitLab} P'
%	}
%	$
%	\\[.2cm]
%	$
%	\infer[$\rulelabel{M-B-Rll}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} Q 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
%	}
%	{
%	P \auxrel{\rollLab} P'
%	}
%	$
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.3cm}	
%	\caption{Multiparty \cherry\ semantics: forward and backward reduction relations (excerpt of rules).}
%	\label{fig:reduction_pic_multi}
%	%\vspace*{-.2cm}	
%\end{figure*}
We comment on salient points.
Rule \rulelabel{M-F-Con} synchronously initiates a session by requiring all session 
endpoints be present for a forward reduction, where each role $\role{p}$ 
creates a session endpoint $s\mendpoint{\role{p}}$ on a fresh session channel $s$. 
The participant with the maximum role %($\mrequestAct{a}{n}{x}{P_n}$) 
is responsible for requesting a session initiation. Rule \rulelabel{M-F-Com} defines how 
a party with role $\role{p}$ synchronously sends a value to the receiving party with role $\role{q}$. 
Rules \rulelabel{M-B-Abt}, \rulelabel{M-F-Cmt} and \rulelabel{M-B-Rll} are similar to 
those of the binary case, and affect all participants within the considered session. 

%The syntax of session types extends to multiparty as shown in Fig.~\ref{fig:typeSyntax_cherry_multi}. 
%\begin{figure}[t]
%	\centering
%	\small
%	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
%	$\typeT$ & ::= &  &  \ldots \  $\mid$  \
%	$\moutType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
%	$\minpType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
%	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	 \   $\mid$ \ 
%	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$
%	\quad \textbf{Session types}
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.5cm}	
%	\caption{Multiparty \Cherry\ type syntax 
%	(the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry}).
%	}
%	\label{fig:typeSyntax_cherry_multi}
%	\vspace*{-.5cm}
%\end{figure}
The session types for output ($\moutType{\role{p}}{\role{q}}{S}.\typeT$)
and input ($\minpType{\role{p}}{\role{q}}{S}.\typeT$) are extended with information 
about the interacting roles; selection and branching types are similarly extended. 
In the type inference, when one of such role is unknown, it is used
a placeholder $\_$ to be filled with a given role; $\typeT\cdot\role{p}$ denotes the type obtained 
from $\typeT$ by filling all its placeholders with the role $\role{p}$.
%
The \cherry\ type system extends accordingly; as an example we report in Fig.~\ref{fig:reduction_pic_multi}(central part) the rules for output and input.
%${\small
%\qquad
%	\infer{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
%	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
%	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
%\qquad\qquad
%	\infer{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
%	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
%	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
%}$\\[.2mm]
%The semantics of type configurations 
%is defined only for filled types. 
%Notation $\typeT^I$, with 
%$I={\{1,\ldots,n\}}$, denotes $\typeT^1,\ldots,\typeT^n$.
%
%Rules in Fig.~\ref{fig:typeSemantics_ext_multi}
%(where $I=\{1,\ldots,n\}$, $i,j\in I$, and 
%$\typeT^{I}$ denotes $\typeT^1,\ldots,\typeT^n$)
%are the natural extension of those for the binary case.
%Rule \rulelabel{M-TS-Com} shows that 
%communication 	affects only the two interacting parties, without modifying any checkpoint.
%Rule \rulelabel{M-TS-Cmt} sets the checkpoint of the committing party and sets an imposed 
%checkpoint for each other party that has performed at least an action from 
%its current checkpoint. Rule \rulelabel{M-TS-Rll} rolls all parties back to their checkpoints,
%provided that the checkpoint of the party requesting the rollback  is not imposed. 
%Rule \rulelabel{M-TS-Abt} brings all parties back to the initial configuration. 
%
The semantics of type configurations is defined only for filled types;
the semantic rules are the natural extension of those for the binary case.
In particular, the rule for commit sets the checkpoint of the committing party and 
sets an imposed checkpoint for each other party that has performed at least an action from 
its current checkpoint; the rule for rollback rolls all parties back to their checkpoints,
provided that the checkpoint of the party requesting the rollback  is not imposed; 
and rule for abort brings all parties back to the initial configuration. 
%
As an example, we report in Fig.~\ref{fig:reduction_pic_multi}(lower part)
the rule for communication, where $I=\{1,\ldots,n\}$, $i,j\in I$, and 
$\typeT^{I}$ denotes $\typeT^1,\ldots,\typeT^n$.
The rule shows that communication affects only 
the two interacting parties, without modifying any checkpoint. 


%%%%%%%%%% ROLLBACK SAFETY
%Our notion of 
\emph{Rollback safety}, and the related compliance relation, extended 
to multiparty sessions is as follows. Notice that types $\typeT_i$ in 
Def.~\ref{def:rollback_safety_multi} contain placeholders, while in 
Def.~\ref{def:compliance_multi} all types are filled. 

\begin{definition}[Multiparty Rollback safety]\label{def:rollback_safety_multi}
Let $C$ be an initial collaboration, then $C$ is \emph{rollback safe} 
(shortened \emph{\rollSafe}) if $C \hasType \sessions$
and for each $n$-tuple $\ce{a}\mendpoint{\role{n}}:\typeT_n,\ldots,a\mendpoint{\role{1}}:\typeT_1$
in $\sessions$ we have $\compliant(\typeT_n\cdot\role{n},\ldots,\typeT_1\cdot\role{1})$.
\end{definition}


\begin{definition}[Compliance for Multiparty Sessions]\label{def:compliance_multi}
Types $\typeT_1,\ldots,\typeT_n$ are \emph{compliant}, written 
\mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$}, if  
\mbox{$\compliant(\minitConf{\typeT_1,\ldots,\typeT_n}
\conf{\typeT_1}{\typeT_1},\ldots, \conf{\typeT_n}{\typeT_n})$}.
Relation $\compliant$ on type configurations is defined as follows:
$\compliant(\minitConf{\typeT^1,\ldots,\typeT^n}\conf{\checkpointType{\typeU_1}}{\typeT_1},
\ldots,\conf{\checkpointType{\typeU_n}}{\typeT_n})$
holds if for any $\checkpointType{\typeU}_1'$, $\typeT_1'$, \ldots, $\checkpointType{\typeU}_n'$, $\typeT_n'$ such that
$\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
\typered^*
\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h'}
\typered\!\!\!\!\!\!\!\!/\ \ \  $
we have that $\typeT_1'=\ldots=\typeT_n'=\inactType$.
\end{definition}


%
\noindent All notions 
%and concepts 
of our rollback recovery approach smoothly 
extend to the multiparty case. As consequence, all properties in Sec.~\ref{sec:properties}
still hold in the extended setting; their proofs are in Appendix~\ref{proofs:multiparty}.
% indeed would follow the same structure and only 
%differ for the technicalities concerning the extended definitions. 
We report the key theorem concerning session progress.

\begin{theorem}[Multiparty session progress]
\label{th:deadlock_freedom_multi}
Let $C$ be a \rollSafe\ collaboration of the form 
$(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in \{1,..,n-1\}}\macceptAct{a}{i}{x}{P_i})$.
If $C \fwbwred^* C'$ then either $C' \fwbwred C''$ for some $C''$ or 
$C' \congr \singleSession{s}{C}$ 
$\prod_{i\in \{1,..,n\}}
\logged{{\genSession}}{\checkpointType{Q_i}} \inact\, 
$ for some $\checkpointType{Q_1}, \ldots,\checkpointType{Q_n}$.
\end{theorem}



==> tex/multiparty_LONG.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex
\section{Extension to multiparty sessions}
\label{sec:multiparty}

We discuss in this section how to extend \cherry, its type discipline,
the compliance checking and the related results, to multiparty 
sessions \cite{KouzapasY14}.

The base sets for the multiparty syntax of \cherry\  are the same
of the binary case, except for \emph{session endpoints}, which now are denoted by 
$s\mendpoint{\role{p}}$, with $\role{p}$,$\role{q}$ ranging over \emph{roles} 
(represented as natural numbers). 
Thus, \emph{session identifiers} $\sessId$ 
now range over session endpoints $s\mendpoint{\role{p}}$ or variables $x$.
%
The runtime syntax of multiparty \cherry\ is defined by the grammar in 
Figure~\ref{fig:syntax_cherry_pi_multi}, where expressions $e$ are defined as in the binary case. 
%(with values that extends to 
%multiparty session endpoints). 
 %
\begin{figure}[t]
\small
	\begin{tabular}{@{}r@{ }c@{\ \ }l@{\ \ \ }l@{}}
	$C$ & ::= & $\cdots$   \ $\mid$ \
	                   $\mrequestAct{a}{\role{p}}{x}{P}$ \ $\mid$ \ $\macceptAct{a}{\role{p}}{x}{P}$
	                   & \textbf{Collaborations}
	\\[.2cm]
	$P$ & ::= &  $\cdots$  \ $\mid$ \
                                        $\msendAct{\sessId}{\role{p}}{e}{P}$ 
		         $\mid$ \ $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ 	
		         $\mid$ \ $\mselectAct{\sessId}{\role{p}}{l}{P}$ 
		         $\mid$ \ $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
			& \textbf{Processes}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.2cm}	
	\caption{Multiparty \cherry\ runtime syntax (the omitted parts are as in Fig.~\ref{fig:syntax_cherry_pi_ext}).}
	\vspace*{-.5cm}	
	\label{fig:syntax_cherry_pi_multi}
\end{figure}
%
Primitive $\mrequestAct{a}{\role{p}}{x}{P}$ initiates a new session through 
identifier $a$ on the other multiple participants, each one of the form 
$\macceptAct{a}{\role{q}}{x}{P_{\role{q}}}$ where $1 \leq \role{q} \leq \role{p}-1$. 
Variable $x$ will be substituted with the session endpoint used for the interactions
inside the established session. 
Primitive $\msendAct{\sessId}{\role{p}}{e}{P}$ denotes the intention of sending a value to 
role $\role{p}$; similarly, process $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ denotes the intention 
of receiving a value from role $\role{p}$. Selection and branching behave in a similar way. 

%As usual the operational semantics is given in terms of a structural congruence and of a 
%reduction relation. 
%The rules defining the structural congruence are the same ones used for the binary calculus,
%where the rule for the scope extension of session channels takes into account the new form 
%of session endpoints. 
%The reduction relation, instead, is the smallest relation on 
%closed collaborations generated by the rules (an excerpt of which are) reported 
%in Figure~\ref{fig:reduction_pic_multi}.
The forward and backward reduction relations are given by the (excerpt of) rules 
in Figure~\ref{fig:reduction_pic_multi}.
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{l@{\ \ }l@{\qquad\qquad\ }l@{\ \ }l@{\ }l}
	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
	\auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P$
	\quad $\expreval{e}{v}$ 
	& \rulelabel{M-P-Snd}
	&
	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y:S}{P}
	 \auxrel{\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}} P$
	& \rulelabel{M-P-Rec}
	\\[.3cm]
	\end{tabular}	
	%
	\begin{tabular}{@{}l@{}}
		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
	$\ \ \fwred\ \ $
	\qquad\qquad\qquad\quad\qquad\qquad\qquad\qquad
	$I=\{1,..,n-1\}$\quad
	\rulelabel{M-F-Con}	
		\\[.1cm]
	\qquad 	
	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$ 
        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
        \!\mid\! 
        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
	\\[.4cm]	
	$
	\infer{
	\loggedShort{\ce{\genSession}}{Q_1} P_1 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2
	\ \fwred\ 
	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
	}
	{
	P_1 \auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P_1'
	\quad
	P_2 \auxrel{\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}} P_2'	
	\hspace*{.3cm}
	$\rulelabel{M-F-Com}$
	}
	$
	\qquad
	$
	\infer{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \bwred\ 
	C}
	{\hspace*{1.7cm}
	P \auxrel{\abortLab} P'
	\hspace*{1.5cm}
	$\rulelabel{M-B-Abt}$
	}
	$	
	\\[.2cm]
	$
	\infer[$\rulelabel{M-F-Cmt}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \fwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{P'} P' 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
	}
	{
	P \auxrel{\commitLab} P'
	}
	$
	\\[.2cm]
	$
	\infer[$\rulelabel{M-B-Rll}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \bwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} Q 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
	}
	{
	P \auxrel{\rollLab} P'
	}
	$
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Multiparty \cherry\ semantics: forward and backward reduction relations (excerpt of rules).}
	\label{fig:reduction_pic_multi}
	%\vspace*{-.5cm}	
\end{figure*}
We comment on salient points.
Rule \rulelabel{M-F-Con} synchronously initiates a session by requiring all session 
endpoints be present for a forward reduction, where each role $\role{p}$ 
creates a session endpoint $s\mendpoint{\role{p}}$ on a fresh session channel $s$. 
The participant with the maximum role %($\mrequestAct{a}{n}{x}{P_n}$) 
is responsible for requesting a session initiation. Rule \rulelabel{M-F-Com} defines how 
a party with role $\role{p}$ synchronously sends a value to the receiving party with role $\role{q}$. 
Rules \rulelabel{M-B-Abt}, \rulelabel{M-F-Cmt} and \rulelabel{M-B-Rll} are similar to 
those of the binary case, and affect all participants within the considered session. 

The syntax of session types extends to multiparty as shown in Fig.~\ref{fig:typeSyntax_cherry_multi}. 
\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
	$\typeT$ & ::= &  &  \ldots \  $\mid$  \
	$\moutType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
	$\minpType{\role{p}}{\role{q}}{S}.\typeT$ \  $\mid$ \ 
	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	 \   $\mid$ \ 
	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$
	\quad \textbf{Session types}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.5cm}	
	\caption{Multiparty \Cherry\ type syntax 
	(the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry}).
	}
	\label{fig:typeSyntax_cherry_multi}
	\vspace*{-.5cm}
\end{figure}
The types for output, input, selection and branching are extended with information 
about the interacting roles. In the type inference, when one of such role is unknown, it is used
a placeholder $\_$ to be filled with a given role; $\typeT\cdot\role{p}$ denotes the type obtained 
from $\typeT$ by filling all its placeholders with the role $\role{p}$.
%
The \cherry\ type system extends accordingly; as an example we report below the rules for 
output and input:
$$
	\infer{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
\qquad\qquad
	\infer{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
$$
The semantics of types and type configurations is defined only for filled types; we report 
in Fig.~\ref{fig:typeSemantics_ext_multi} an excerpt of rules. Notation $\typeT^I$, with 
$I={\{1,\ldots,n\}}$, denotes $\typeT^1,\ldots,\typeT^n$.
%
These rules are the natural extension of those for the binary case. 
Rules \rulelabel{M-TS-Snd}, \rulelabel{M-TS-Rcv} and \rulelabel{M-TS-Com} show that 
communication 	affects only the two interacting parties, without modifying any checkpoint.
Rule \rulelabel{M-TS-Cmt} sets the checkpoint of the committing party and sets an imposed 
checkpoint for each other session party that has performed at least an action from 
its current checkpoint. Rule \rulelabel{M-TS-Rll} rolls all parties back to their checkpoints,
provided that the checkpoint of the party requesting the rollback  is not imposed. 
Rule \rulelabel{M-TS-Abt} brings all parties back the initial configuration. 


Our notion of \emph{rollback safety}, and the related compliance relation, extend 
to multiparty sessions as follows. Notice that types $\typeT_i$ in 
Def.~\ref{def:rollback_safety_multi} contain placeholders, while in 
Def.~\ref{def:compliance_multi} all types are filled. 
 

\begin{definition}[Multiparty Rollback safety]\label{def:rollback_safety_multi}
Let $C$ be an initial collaboration, then $C$ is \emph{rollback safe} if $C \hasType \sessions$
and for each $n$-tuple $\ce{a}\mendpoint{\role{n}}:\typeT_n,\ldots,a\mendpoint{\role{1}}:\typeT_1$
in $\sessions$ we have $\compliant(\typeT_n\cdot\role{n},\ldots,\typeT_1\cdot\role{1})$.
\end{definition}


\begin{definition}[Compliance for Multiparty Sessions]\label{def:compliance_multi}
Types $\typeT_1,\ldots,\typeT_n$ are \emph{compliant}, written 
\mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$}, if  
\mbox{$\compliant(\minitConf{\typeT_1,\ldots,\typeT_n}
\conf{\typeT_1}{\typeT_1},\ldots, \conf{\typeT_n}{\typeT_n})$}.
Relation $\compliant$ on configurations is defined as follows:
$\compliant(\minitConf{\typeT^1,\ldots,\typeT^n}\conf{\checkpointType{\typeU_1}}{\typeT_1},
\ldots,\conf{\checkpointType{\typeU_n}}{\typeT_n})$
holds if for any $\checkpointType{\typeU}_1'$, $\typeT_1'$, \ldots, $\checkpointType{\typeU}_n'$, $\typeT_n'$ such that
$\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
\typered^*
\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h'}
\typered\!\!\!\!\!\!\!\!/\ \ \  $
we have that $\typeT_1'=\ldots=\typeT_n'=\inactType$.
\end{definition}
%
All notions and concepts of our rollback recovery approach smoothly 
extend to the multiparty case. As consequence, all properties in \S~\ref{sec:properties}
still hold in the extended setting; their proofs indeed would follow the same structure and only 
differ for the technicalities concerning the extended definitions. 

\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{@{}l@{\qquad}l@{}}
%	$\moutType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Snd}	
%	&
%	$\minpType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\minpType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Rcv}  
%	\\[.3cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
	\, ,\,
	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\ \qquad \quad
	\typered
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i'} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j'}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\end{array}
	$
	\
	 $i,j\in I$
	\quad
	\rulelabel{M-TS-Com}
	}
	\\[.7cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\commitType} \typeT_i'
	 }	
	 \quad
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\ \qquad \quad	
	\typered
	\minitConf{\typeT^I}
	\conf{\typeT_i'}{\typeT_i'} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h}
	\end{array}
	$
	 $i\in I$
	 \ , \
	 $
	 \checkpointType{\typeU}_h' \! =\!\! 
	 \left\{
	 \begin{array}{ll}
	 \checkpointType{\typeU}_h & \textrm{if}\ \checkpointType{\typeU}_h = \typeT_h \\[-.1cm]
	 \imposed{\typeT_h} & \textrm{otherwise}
	 \end{array}
	 \right.
	 $
	\quad
	\rulelabel{M-TS-Cmt}
	}
	\\[.7cm]
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\rollType} \typeT_i'
	 }	
	 \quad
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\typered
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeU_i}  
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeU_h}
	\end{array}
	$
	 $i\in I$	 
	\quad
	\rulelabel{M-TS-Rll}
	}
	\\[.7cm]	
	\multicolumn{2}{@{}l@{}}{
	$
	\begin{array}{l}
	{\typeT_i \typeTrans{\abortType} \typeT_i'
	 }	
	 \quad
	\Rightarrow
	\\		
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\typered
	\minitConf{\typeT^I}
	\prod_{k\in I}\conf{\typeT^k}{\typeT^k}
	\end{array}
	$
	 $i\in I$	 
	\quad
	\rulelabel{M-TS-Abt}
	}
	\\[.4cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Semantics of multiparty types and type configurations 
	(excerpt of rules, where $I=\{1,\ldots,n\}$).}
	\label{fig:typeSemantics_ext_multi}
	\vspace*{-.5cm}
\end{figure}


==> tex/multiparty_type_system.tex <==
% !TEX root = ../rev_sessions@esop19.tex
\begin{figure}[!t]
	\centering
	\small
	\begin{tabular}{c}
	$
	\infer[$\rulelabel{M-T-Req}$]{\mrequestAct{a}{\role{p}}{x}{P} \hasType \{\ce{a}\mendpoint{\role{p}}:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$		
	\qquad
	$
	\infer[$\rulelabel{M-T-Acc}$]{\macceptAct{a}{\role{p}}{x}{P} \hasType \{a\mendpoint{\role{p}}:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$
	\\[.4cm]
        $
	\infer[$\rulelabel{M-T-Snd}$]{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
	$
        \\[.4cm]
        $
	\infer[$\rulelabel{M-T-Rcv}$]{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
	$
        \\[.4cm]
	$
	\infer[$\rulelabel{M-T-Sel}$]{\basis;\sorting \judge \mselectAct{x}{\role{p}}{l}{P} \hasType 
	x:\mselType{\_}{\role{p}}{l}.\typeT}
	{\basis;\sorting  \judge P \hasType x:\typeT}
	$        
	\\[.4cm]			
	$
	\infer[$\rulelabel{M-T-Br}$]{\basis;\sorting \judge 
	\mbranchAct{x}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}
	\hasType 
	x:\mbranchType{\_}{\role{p}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}}
	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
	$
	\\[.1cm]	        
	\hline
	\end{tabular}
	\vspace*{-.3cm}
	\caption{Multiparty \cherry\ typing system (the omitted rules are as in
	Fig.~\ref{fig:typingSystem_coll}, \ref{fig:typingSystem_proc} and \ref{fig:typingSystem_exp_omitted}).}
	%\vspace*{-.1cm}	
	\label{fig:typingSystem_multi}
\end{figure}
	
	

==> tex/omitted_rules.tex <==
% !TEX root = ../rev_sessions@coord19.tex

\section{Omitted Rules}
\label{app:omitted}
For reviewers' convenience, we report in this appendix those rules that have been
omitted in the paper. 

The omitted operational rules of the auxiliary labelled relation $\auxrel{\actionLab}$
are in Fig.~\ref{fig:semantics_cherry_pi_aux_omitted}.
\begin{figure*}[!h]
	\centering
	\small
	\begin{tabular}{@{}l@{\quad\ \ }l@{}}
	$
	\infer{P_1 \ \auxrel{\actionLab}\ P_2}
	{P_1 \congr P_1'\ \auxrel{\actionLab}\ P_2' \congr P_2}
	$
	\ \raisebox{.4cm}{\rulelabel{P-Str}}
	&
	\raisebox{.4cm}{
	\begin{tabular}{@{}l@{}}
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_2$ 
	\quad ($\expreval{e}{\cfalse}$) 
	\end{tabular}
	}
	\quad
	\raisebox{.4cm}{
	\begin{tabular}{@{\!}l}
	\rulelabel{P-IfF}
	\end{tabular}
         }
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{\Cherry\ semantics: auxiliary labelled relation (omitted rules).}
	\label{fig:semantics_cherry_pi_aux_omitted}
	%\vspace*{-.2cm}	
\end{figure*}



%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{}}
%        $\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2}$
%	$\fwred$
%	$\singleSession{s}{(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})}$
%	\hspace*{2.6cm}
%	\rulelabel{F-Con}
%	\\ 
%	\hspace*{3.1cm}
%        $(\loggedShort{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}
%        \mid 
%	\loggedShort{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )\ $
%	\\[.3cm]	
%	$
%	\infer[$\rulelabel{F-Com}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{\ce{k}}{v}} P_1'
%	\qquad
%	P_2 \auxrel{\receive{k}{x}} P_2'	
%	}
%	$	
%       	\\[.3cm]	
%	$
%	\infer[$\rulelabel{F-Lab}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'
%	}
%	{
%	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
%	\qquad
%	P_2 \auxrel{\branching{k}l} P_2'	
%	}
%	$
%	\\[.3cm]		
%	$
%	\infer[$\rulelabel{F-Cmt}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{P_2} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{F-Str}$]{C_1 \ \fwred\ C_2}
%	{C_1 \congr C_1'\ \fwred\ C_2' \congr C_2}
%	$
%        \qquad\qquad\quad\ \
%	$
%	\infer[$\rulelabel{F-If}$]{
%	\logged{\genSession}{Q} P
%	\ \fwred\ 
%	\logged{\genSession}{Q} P' 
%	}
%	{
%	P \auxrel{\ite} P'
%	}
%	$	
%	\\[.3cm]	
%        $
%	\infer[$\rulelabel{F-Res}$]{\singleSession{s}{C_1}\,C_2 \ \fwred\ \singleSession{s}{C_1}\,C_2'}
%	{C_2 \ \fwred\ C_2'}
%	$
%        \qquad\ \	
%	$
%	\infer[$\rulelabel{F-Par}$]{C_1 \!\mid\! C_2 \ \fwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \fwred\ C_1'}
%	$	
%	\\[.3cm]	
%	$
%	\infer[$\rulelabel{B-Rll}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \bwred\ 
%	\logged{\ce{\genSession}}{Q_1} Q_1
%	\ \mid \ 
%	\logged{\genSession}{Q_2} Q_2
%	}
%	{
%	P_1 \auxrel{\rollLab} P_1'
%	}
%	$	
%	\\[.4cm]		
%	$
%	\infer[$\rulelabel{B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2)
%	\ \bwred\ C
%	}
%	{
%	P_1 \auxrel{\abortLab} P_1'
%	}
%	$	
%	\qquad
%	$
%	\infer[$\rulelabel{B-Str}$]{C_1 \ \bwred\ C_2}
%	{C_1 \congr C_1'\, \bwred\, C_2' \congr C_2}
%	$	
%	\\[.4cm]				
%	$
%	\infer[$\rulelabel{B-Res}$]{\singleSession{s}{C_1}C_2 \ \bwred\ \singleSession{s}{C_1}C_2'}
%	{
%	C_2 \ \bwred\ C_2'
%	}
%	$
%	\qquad\quad
%	$
%	\infer[$\rulelabel{B-Par}$]{C_1 \!\mid\! C_2 \ \bwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \bwred\ C_1'}
%	$
%	\\[.1cm]
%	\hline
%	\end{tabular}	
%	\vspace*{-.3cm}	
%	\caption{\Cherry\ semantics: forward and backward reduction relations. }
%	\label{fig:semantics_cherry_pi_omitted}
%	%\vspace*{-.2cm}	
%\end{figure*}




The omitted rules defining the typing system for \cherry\ processes and expressions
are given in Fig.~\ref{fig:typingSystem_proc_omitted} and \ref{fig:typingSystem_exp_omitted}. 
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
%		$
%	\infer[$\rulelabel{T-Snd}$]{\basis;\sorting \judge \sendAct{x}{e}{P} \hasType x:\outType{S}.\typeT}
%	{\sorting \judge e \hasType S & \basis;\sorting \judge P \hasType x:\typeT}
%	$		
%	\quad
%	$
%	\infer[$\rulelabel{T-Rcv}$]{\basis;\sorting \judge \receiveAct{x}{y:S}{P} \hasType x:\inpType{S}.\typeT}
%	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
%	$	
%	\\[.3cm]	
%	\qquad\quad
%	\raisebox{.2cm}{$\basis;\sorting\! \judge\! \inact\! \hasType\! x:\inactType$\ \ \rulelabel{T-Inact}}
%	\qquad
	$
	\infer[$\rulelabel{T-Sel}$]{\basis;\sorting \judge \selectAct{x}{l}{P} \hasType 
	x:\selType{l}.\typeT}
	{\basis;\sorting  \judge P \hasType x:\typeT}
	$        
	\\[.3cm]			
	$
	\infer[$\rulelabel{T-Br}$]{\basis;\sorting \judge \branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType 
	x:\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}}
	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
	$
%	\\[.4cm]	
%       	$
%	\infer[$\rulelabel{T-If}$]{\basis;\sorting \judge \ifthenelseAct{e}{P_1}{P_2} \hasType 
%	x:\typeT_1 \choiceType \typeT_2}
%	{\sorting \! \judge\! e \!\hasType\! \boolType &
%	\basis;\sorting  \judge P_1 \hasType x:\typeT_1 & \basis;\sorting  \judge P_2 \hasType x:\typeT_2}
%	$
%	\\[.3cm]	
%	\raisebox{.2cm}{$\basis\comp X:t;\sorting \judge X \!\hasType\! t$\ \rulelabel{T-Pvar}}			
%	\qquad
%	\infer[$\rulelabel{T-Rec}$]{\basis;\sorting \judge \recAct{X}{P} \hasType \recAct{t}{\typeT}}
%	{\basis\comp X:t;\sorting  \judge P \hasType \typeT}	
%	\\[.3cm]
%	$
%	\infer[$\rulelabel{T-Cmt}$]{\basis;\sorting \judge \commitAct{P}  \hasType 
%	x:\commitType.\typeT}
%	{
%	\basis;\sorting  \judge P \hasType x:\typeT 
%	}
%	$
%	\\[.3cm]
%	$\basis;\sorting \judge \roll \hasType x:\rollType$\ \ \rulelabel{T-Rll}	
%	\qquad
%	$\basis;\sorting \judge \abort \hasType x:\abortType$\ \ 
%	\rulelabel{T-Abt}
	\\[.1cm]	
	\hline
	\end{tabular}
	\vspace*{-.4cm}
	\caption{Typing system for \cherry\ processes (omitted rules).}
	\label{fig:typingSystem_proc_omitted}
	%\vspace*{.3cm}
\end{figure}

\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{tt}}$}
	\qquad
	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{ff}}$}
	\\[.4cm]	
	$\sorting\comp x:S \judge x \hasType S$\ \ \rulelabel{T-Var}	
	\qquad
	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{T-Int}	
	\qquad
	$\sorting \judge\!\!``a" \hasType \strType$\ \ \rulelabel{T-Str}	
	\\[.4cm]
	$
	\infer[$\!\rulelabel{T-Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
	{\sorting \judge e_1 \hasType \intType &  \sorting \judge e_2 \hasType \intType}
	\quad
	\infer[$\!\rulelabel{T-And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
	{\sorting \judge e_1 \hasType \boolType  & \sorting \judge e_2 \hasType \boolType}
	$		
        \\[.2cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}
	\caption{Typing system for \cherry\ expressions (excerpt of omitted
          rules).}
	%\vspace*{.2cm}
	\label{fig:typingSystem_exp_omitted}
\end{figure}


The omitted rules defining the semantics of types and type configurations are given in Fig.~\ref{fig:typeSemantics_ext_omitted} (symmetric rules for configurations are omitted).
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}l@{\hspace*{.8cm}}l@{\hspace*{.6cm}}r@{}}
	$\outType{S}.\typeT \typeTrans{\outType{S}} \typeT$\ \ \rulelabel{TS-Snd}	
	&
	$\inpType{S}.\typeT \typeTrans{\inpType{S}} \typeT$\ \ \rulelabel{TS-Rcv}  
	&
	$\selType{l}.\typeT \typeTrans{\selTypeLabel{l}} \typeT$\ \ \rulelabel{TS-Sel}
	\\[.4cm]
	\multicolumn{2}{@{}l@{}}{
	\raisebox{.8cm}{$\!\!
	\branchType{\branch{l_1\!\!}{\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\typeT_n}}
	\typeTrans{\branchTypeLabel{l_i}} \typeT_i$ \ \ $(1 \!\leq\! i \!\leq\! n)$\ \ \rulelabel{TS-Br}
	}
	}
	&
	$
	\infer[$\rulelabel{TS-rec}$]
	{\recType{t}.\typeT \typeTrans{\typeLab} \typeT'}
	{\typeT\subst{\recType{t}.\typeT}{t} \typeTrans{\typeLab} \typeT'}
	$
\\[-.3cm]
	$
	\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_1$\ \ \rulelabel{TS-If$_1$}
	&
	$\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_2$\ \ \rulelabel{TS-If$_2$}
	&
%	\\[.4cm]
%	$\commitType.\typeT \typeTrans{\commitLab} \typeT$\ \ \rulelabel{TS-Cmt}
%	&
%	$\rollType \typeTrans{\rollLab} \inactType$\ \ \rulelabel{TS-Rll}
%	&
%	$\abortType \typeTrans{\abortLab} \inactType$\ \ \rulelabel{TS-Abt}
	\\[.4cm]
	\end{tabular}
	\begin{tabular}{@{}c@{}}
%	$
%	\infer[$\rulelabel{TS-Tau}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	{\typeT_1 \typeTrans{\tau} \typeT_1'}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Com}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	{\typeT_1 \typeTrans{\!\outType{S}\!} \typeT_1'
%	& &
%	 \typeT_2 \typeTrans{\!\!\inpType{S}\!} \typeT_2'}	
%	$	
%	\\[.4cm]
	$
	\infer[$\rulelabel{TS-Lab}$]
	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
	\typered
	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
	{\typeT_1 \typeTrans{\selTypeLabel{l}} \typeT_1'
	& & 
	 \typeT_2 \typeTrans{\branchTypeLabel{l}} \typeT_2'}
	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Cmt$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%	{\typeT_1 \typeTrans{\commitLab} \typeT_1' & & \checkpointType{\typeU}_2 \neq \typeT_2}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Cmt$_2$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%	{\typeT_1 \typeTrans{\commitLab} \typeT_1' & & \checkpointType{\typeU}_2 = \typeT_2}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Rll$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeU_2}}
%	{\typeT_1 \typeTrans{\rollLab} \typeT_1'}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Abt$_1$}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\typeT}{\typeT} \confcomp \conf{\typeT'}{\typeT'}}
%	{\typeT_1 \typeTrans{\abortLab} \typeT_1'}
%	$	
	\\[-.1cm]
	\hspace*{12.1cm}\\
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Semantics of types and type configurations 
	(omitted rules).
	}
	\label{fig:typeSemantics_ext_omitted}
	%\vspace*{-.2cm}
\end{figure}



The omitted rules defining the error semantics are given 
in Fig.~\ref{tab:error_red_omitted}.
%
\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{@{}c@{}}
%	$
%	\infer{
%	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred
%	\comError
%	}
%	{
%	P_1 \auxrel{\send{{k}}{v}} P_1'
%	\qquad
%	\neg P_2 \BarbInp{k}
%	\quad\qquad 
%	$\rulelabel{E-Com1}$
%	}
%	$	
%	\qquad 
	$
	\infer{
	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\comError
	}
	{
	P_1 \auxrel{\receive{{k}}{x}} P_1'
	\quad
	\neg P_2 \BarbOut{k}
	\qquad
	$\rulelabel{E-Com2}$
	}
	$	
	\\[.3cm]	
	$\quad
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\select{{k}}{l}} P_1'
	\quad
	\neg P_2\BarbBranching{k}{l}
	\qquad 
	$\rulelabel{E-Lab$_1$}$
	}
	$			
	\qquad\quad
	$
	\infer{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid 
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred
	\comError
	}
	{
	P_1 \auxrel{\branching{k}l} P_1'
	\quad
	\neg P_2\BarbSelect{k}{l}
	\qquad 
	$\rulelabel{E-Lab$_2$}$
	}
	$
		\\[.3cm]	
	$
	\infer[$\rulelabel{E-Cmt$_1$}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\imposed{P_2}} P_2
	}
	{
	P_1 \auxrel{\commitLab} P_1'
	& & 
	\checkpointType{Q_2} \neq P_2	
	}
	$	
	\\[.3cm]
	$
	\infer[$\rulelabel{E-Cmt$_2$}$]{
	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\fwred 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	}
	{
	P_1 \auxrel{\commitLab} P_1'
	& & 
	\checkpointType{Q_2} = P_2
	}
	$	
	\\[.3cm]		
	$
	\infer[$\rulelabel{E-Rll$_1$}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} P_2
	\bwred
	\logged{\ce{\genSession}}{Q_1} Q_1
	\mid
	\logged{\genSession}{\checkpointType{Q_2}} Q_2
	}
	{	
	P_1 \auxrel{\rollLab} P_1'		
	}
	$	
%	\\[.3cm]	
%	$
%	\infer[$\rulelabel{E-Rll$_2$}$]{
%	\logged{\ce{\genSession}}{\imposed{Q_1}} P_1 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\rollError
%	}
%	{
%	P_1 \auxrel{\rollLab} P_1'	
%	}
%	$	
	\\[.1cm]
	\hline
	\end{tabular}	
	\vspace*{-.3cm}	
	\caption{\Cherry\ semantics: error reductions (omitted rules).}
	\label{tab:error_red_omitted}
	%\vspace*{-.2cm}
\end{figure*}
%
The semantics of \cherry\ is extended by the additional rules, 
where \rulelabel{E-Cmt$_1$} and \rulelabel{E-Cmt$_2$} replace \rulelabel{F-Cmt},
and \rulelabel{E-Rll$_1$} replaces  \rulelabel{B-Rll},
and $\checkpointType{\ }$ is used in the checkpoints of the other rules.
%
The definition of these rules relies  on the notion of \emph{barb} predicates, whose straightforward 
definition is: 
$P\Barb{\mu}$ holds if there exists $P'$ such that $P \Rightarrow P'$ and 
$P'$ can perform an action $\mu$, 
where $\mu$ stands for $k?$, $k!$ ,$k\triangleleft l$ or $k\triangleright l$
(i.e., input, output, select and branching action along session channel $k$);
$\Rightarrow$ is the reflexive and transitive closure of $\auxrel{\ite}$.




\newpage
%%%%%%%%%%%%%%%%%%%% MULTIPARTY
The omitted syntax of multiparty \cherry\ and of multiparty session types 
are in Fig.~\ref{fig:syntax_cherry_pi_multi_omitted} and~\ref{fig:typeSyntax_cherry_multi_omitted},
respectively.
\begin{figure}[h]
\small
	\begin{tabular}{@{}r@{ }c@{\ }l@{\ \ }l@{}}
	$C$ & ::= & $\cdots$    $\mid$ 
	                   $\mrequestAct{a}{\role{p}}{x}{P}$  $\mid$  $\macceptAct{a}{\role{p}}{x}{P}$
	                   & \!\!\!\!\!\!\!\!\!\textbf{Collaborations}
	\\[.3cm]
	$P$ & ::= &  $\cdots$  $\mid$ 
                                        $\msendAct{\sessId}{\role{p}}{e}{P}$ 
		         $\mid$  $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ 	
		         $\mid$  $\mselectAct{\sessId}{\role{p}}{l}{P}$ 
		         $\mid$  $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
			& \ \ \ \textbf{Processes}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Multiparty \cherry\ runtime syntax; the omitted parts are as in Fig.~\ref{fig:syntax_cherry_pi_ext} (omitted rules).}
	%\vspace*{.2cm}	
	\label{fig:syntax_cherry_pi_multi_omitted}
\end{figure}

\clearpage 

%
\begin{figure}[h]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
	$\typeT\!$ & ::= &  &\!\!  \ldots   $\mid$  
	$\moutType{\role{p}}{\role{q}}{S}.\typeT$  $\,\mid\,$ 
	$\minpType{\role{p}}{\role{q}}{S}.\typeT$   $\,\mid\,$ 
	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	$\,\mid\,$  
	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}$
	\ \ \textbf{Types}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.6cm}	
	\caption{Multiparty \Cherry\ type syntax; 
	the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry} (omitted rules).
	}
	\label{fig:typeSyntax_cherry_multi_omitted}
	%\vspace*{.5cm}
\end{figure}

The omitted rules of the multiparty semantics are reported in 
Fig.~\ref{fig:reduction_pic_multi_omitted}.
\begin{figure*}[!h]
	\centering
	\small
        \begin{tabular}{@{ }c@{}}
	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
	\auxrel{\!\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}\!} \!P$
	\ ($\expreval{e}{v}$)
	 \rulelabel{M-P-Snd}
	\qquad
	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y\!:\!S}{P}
	 \auxrel{\!\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}\!\!} \!P$
	\rulelabel{M-P-Rcv}
	\\[.5cm]
	\end{tabular}	
	\\
	\begin{tabular}{@{}l@{}}
		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
	$\ \ \fwred\ \ $
	\\[.1cm]
	\quad 	
	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$
	\qquad\quad\qquad\qquad\qquad\ \
	$I\!=\!\{1,..,n\!-\!1\}$\quad
	\rulelabel{M-F-Con}	
	\\[.1cm] 	
	\quad 	
        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
        \!\mid\! 
        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
	\\[.5cm]
	\end{tabular}
	\begin{tabular}{@{}c@{}}	
	$
	\infer[$\rulelabel{M-F-Com}$]{
	\loggedShort{\ce{\genSession}}{Q_1} P_1 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2
	\ \fwred\ 
	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
	\mid 
	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
	}
	{
	P_1 \auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P_1'
	& & 
	P_2 \auxrel{\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}} P_2'	
	}
	$
	\\[.4cm]
	$
	\infer[$\rulelabel{M-F-Cmt}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \fwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{P'} P' 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
	}
	{
	P \auxrel{\commitLab} P'
	}
	$
	\\[.4cm]
	$
	\infer[$\rulelabel{M-B-Rll}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \bwred\ 
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} Q 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
	}
	{
	P \auxrel{\rollLab} P'
	}
	$
	\\[.4cm]
	$
	\infer[$\rulelabel{M-B-Abt}$]{
	\singleSession{s}{C}(
	\logged{\ce{\genSession}}{Q} P 
	\ \mid \ 
	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
	\ \bwred\ 
	C}
	{
	P \auxrel{\abortLab} P'
	}
	$
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Multiparty \cherry\ semantics: forward and backward reductions (excerpt of omitted rules).}
	\label{fig:reduction_pic_multi_omitted}
	\vspace*{.7cm}	
\end{figure*}

\clearpage
The omitted rules of the multiparty type system  are reported in 
Fig.~\ref{fig:typingSystem_multi_omitted}.
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{c}
	$
	\infer[$\rulelabel{M-T-Req}$]{\mrequestAct{a}{\role{p}}{x}{P} \hasType \{\ce{a}\mendpoint{\role{p}}:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$		
	\qquad
	$
	\infer[$\rulelabel{M-T-Acc}$]{\macceptAct{a}{\role{p}}{x}{P} \hasType \{a\mendpoint{\role{p}}:\typeT\}}
	{\emptyset;\emptyset \judge P \hasType x:\typeT}
	$
	\\[.4cm]
        $
	\infer[$\rulelabel{M-T-Snd}$]{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
	$
        \\[.4cm]
        $
	\infer[$\rulelabel{M-T-Rcv}$]{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
	$
        \\[.4cm]
	$
	\infer[$\rulelabel{M-T-Sel}$]{\basis;\sorting \judge \mselectAct{x}{\role{p}}{l}{P} \hasType 
	x:\mselType{\_}{\role{p}}{l}.\typeT}
	{\basis;\sorting  \judge P \hasType x:\typeT}
	$        
	\\[.4cm]			
	$
	\infer[$\rulelabel{M-T-Br}$]{\basis;\sorting \judge 
	\mbranchAct{x}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}
	\hasType 
	x:\mbranchType{\_}{\role{p}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}}
	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
	$
	\\[.1cm]	        
	\hline
	\end{tabular}
	\vspace*{-.3cm}
	\caption{Multiparty \cherry\ typing system (the omitted rules are as in
	Fig.~\ref{fig:typingSystem_coll}, \ref{fig:typingSystem_proc} and \ref{fig:typingSystem_exp_omitted}).}
	%\vspace*{-.1cm}	
	\label{fig:typingSystem_multi_omitted}
\end{figure}

Finally, the omitted rules of the multiparty type configurations semantics are reported in 
Fig.~\ref{fig:typeSemantics_ext_multi_omitted}.
\begin{figure}[!h]
	\centering
	\small
	\begin{tabular}{@{}l@{\qquad\quad}l@{}}
	$\moutType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Snd}	
	& 
	$\minpType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\minpType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Rcv}  
	\\[.5cm]
	\multicolumn{2}{@{}c@{}}{
	$
	\infer[$\rulelabel{M-TS-Com}$]
	{\begin{array}{l}
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\[.1cm] 
	\quad
	\typered
	\ \
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i'} 
	\confcomp 
	\conf{\checkpointType{\typeU}_j}{\typeT_j'}
	\confcomp 	
	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\end{array}}
	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
	& &
	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
	$
	}
	\\[.8cm]
	\multicolumn{2}{@{}c@{}}{
	$
	\infer[\ \	
	 \checkpointType{\typeU}_h' \! =\!\! 
	 \left\{
	 \begin{array}{ll}
	 \checkpointType{\typeU}_h & \textrm{if}\ \checkpointType{\typeU}_h = \typeT_h \\
	 \imposed{\typeT_h} & \textrm{otherwise}
	 \end{array}
	 \right.
	\ \
	$\rulelabel{M-TS-Cmt}$
	]	
	{
	\begin{array}{l}
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\\
	\quad
	\typered
	\ \
	\minitConf{\typeT^I}
	\conf{\typeT_i'}{\typeT_i'} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h}
	\end{array}
	}
	{\typeT_i \typeTrans{\commitLab} \typeT_i'}	
	$
	}
	\\[.8cm]
	\multicolumn{2}{@{}c@{}}{
	$
	\infer
	{
	\begin{array}{l}
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\
	\typered
	\
	\minitConf{\typeT^I}
	\conf{\typeU_i}{\typeU_i}  
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeU_h}
	\end{array}
	}
	{\hspace*{4cm}
	\typeT_i \typeTrans{\rollLab} \typeT_i' 
	\hspace*{4cm}
	$\rulelabel{M-TS-Rll}$
	}	
	$
	}
	\\[.8cm]	
	\multicolumn{2}{@{}c@{}}{
	$
	\infer[$\rulelabel{M-TS-Abt}$]
	{
	\begin{array}{l}
	\minitConf{\typeT^I}
	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
	\confcomp 
	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
	\
	\typered
	\
	\minitConf{\typeT^I}
	\prod_{k\in I}\conf{\typeT^k}{\typeT^k}
	\end{array}
	}
	{\typeT_i \typeTrans{\abortLab} \typeT_i' }	
	$	
	}
	\\[.4cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Multiparty \cherry\ type semantics (excerpt of rules, 
	where $I=\{1,\ldots,n\}$, $i,j\in I$, and $\typeT^{I}$ denotes $\typeT^1,\ldots,\typeT^n$).}
	\label{fig:typeSemantics_ext_multi_omitted}
	%\vspace*{-.2cm}
\end{figure}
\clearpage


==> tex/omitted_rules_shorts.tex <==
% !TEX root = ../rev_sessions@coord19.tex

\section{Omitted Rules}
\label{app:omitted}
%For reviewers' convenience, we report in this appendix those rules that have been
%omitted in the paper. 
%
%The omitted operational rules of the auxiliary labelled relation $\auxrel{\actionLab}$
%are in Fig.~\ref{fig:semantics_cherry_pi_aux_omitted}.
%\begin{figure*}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{\quad\ \ }l@{}}
%	$
%	\infer{P_1 \ \auxrel{\actionLab}\ P_2}
%	{P_1 \congr P_1'\ \auxrel{\actionLab}\ P_2' \congr P_2}
%	$
%	\ \raisebox{.4cm}{\rulelabel{P-Str}}
%	&
%	\raisebox{.4cm}{
%	\begin{tabular}{@{}l@{}}
%	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_2$ 
%	\quad ($\expreval{e}{\cfalse}$) 
%	\end{tabular}
%	}
%	\quad
%	\raisebox{.4cm}{
%	\begin{tabular}{@{\!}l}
%	\rulelabel{P-IfF}
%	\end{tabular}
%         }
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\caption{\Cherry\ semantics: auxiliary labelled relation (omitted rules).}
%	\label{fig:semantics_cherry_pi_aux_omitted}
%\end{figure*}
%


%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{}}
%        $\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2}$
%	$\fwred$
%	$\singleSession{s}{(\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2})}$
%	\hspace*{2.6cm}
%	\rulelabel{F-Con}
%	\\ 
%	\hspace*{3.1cm}
%        $(\loggedShort{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}
%        \mid 
%	\loggedShort{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )\ $
%	\\[.3cm]	
%	$
%	\infer[$\rulelabel{F-Com}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{\ce{k}}{v}} P_1'
%	\qquad
%	P_2 \auxrel{\receive{k}{x}} P_2'	
%	}
%	$	
%       	\\[.3cm]	
%	$
%	\infer[$\rulelabel{F-Lab}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'
%	}
%	{
%	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
%	\qquad
%	P_2 \auxrel{\branching{k}l} P_2'	
%	}
%	$
%	\\[.3cm]		
%	$
%	\infer[$\rulelabel{F-Cmt}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\ \mid \ 
%	\logged{\genSession}{P_2} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	}
%	$	
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{F-Str}$]{C_1 \ \fwred\ C_2}
%	{C_1 \congr C_1'\ \fwred\ C_2' \congr C_2}
%	$
%        \qquad\qquad\quad\ \
%	$
%	\infer[$\rulelabel{F-If}$]{
%	\logged{\genSession}{Q} P
%	\ \fwred\ 
%	\logged{\genSession}{Q} P' 
%	}
%	{
%	P \auxrel{\ite} P'
%	}
%	$	
%	\\[.3cm]	
%        $
%	\infer[$\rulelabel{F-Res}$]{\singleSession{s}{C_1}\,C_2 \ \fwred\ \singleSession{s}{C_1}\,C_2'}
%	{C_2 \ \fwred\ C_2'}
%	$
%        \qquad\ \	
%	$
%	\infer[$\rulelabel{F-Par}$]{C_1 \!\mid\! C_2 \ \fwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \fwred\ C_1'}
%	$	
%	\\[.3cm]	
%	$
%	\infer[$\rulelabel{B-Rll}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2
%	\ \bwred\ 
%	\logged{\ce{\genSession}}{Q_1} Q_1
%	\ \mid \ 
%	\logged{\genSession}{Q_2} Q_2
%	}
%	{
%	P_1 \auxrel{\rollLab} P_1'
%	}
%	$	
%	\\[.4cm]		
%	$
%	\infer[$\rulelabel{B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\ \mid \ 
%	\logged{\genSession}{Q_2} P_2)
%	\ \bwred\ C
%	}
%	{
%	P_1 \auxrel{\abortLab} P_1'
%	}
%	$	
%	\qquad
%	$
%	\infer[$\rulelabel{B-Str}$]{C_1 \ \bwred\ C_2}
%	{C_1 \congr C_1'\, \bwred\, C_2' \congr C_2}
%	$	
%	\\[.4cm]				
%	$
%	\infer[$\rulelabel{B-Res}$]{\singleSession{s}{C_1}C_2 \ \bwred\ \singleSession{s}{C_1}C_2'}
%	{
%	C_2 \ \bwred\ C_2'
%	}
%	$
%	\qquad\quad
%	$
%	\infer[$\rulelabel{B-Par}$]{C_1 \!\mid\! C_2 \ \bwred\ C_1' \!\mid\! C_2}
%	{C_1 \ \bwred\ C_1'}
%	$
%	\\[.1cm]
%	\hline
%	\end{tabular}	
%	\vspace*{-.3cm}	
%	\caption{\Cherry\ semantics: forward and backward reduction relations. }
%	\label{fig:semantics_cherry_pi_omitted}
%	%\vspace*{-.2cm}	
%\end{figure*}



%
%%The omitted rules defining the typing system for \cherry\ processes and expressions
%%are given in Fig.~\ref{fig:typingSystem_proc_omitted} and \ref{fig:typingSystem_exp_omitted}. 
%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}c@{}}
%		$
%	\infer[$\rulelabel{T-Snd}$]{\basis;\sorting \judge \sendAct{x}{e}{P} \hasType x:\outType{S}.\typeT}
%	{\sorting \judge e \hasType S & \basis;\sorting \judge P \hasType x:\typeT}
%	$		
%	\quad
%	$
%	\infer[$\rulelabel{T-Rcv}$]{\basis;\sorting \judge \receiveAct{x}{y:S}{P} \hasType x:\inpType{S}.\typeT}
%	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
%	$	
%	\\[.3cm]	
%	\qquad\quad
%	\raisebox{.2cm}{$\basis;\sorting\! \judge\! \inact\! \hasType\! x:\inactType$\ \ \rulelabel{T-Inact}}
%	\qquad
%	$
%	\infer[$\rulelabel{T-Sel}$]{\basis;\sorting \judge \selectAct{x}{l}{P} \hasType 
%	x:\selType{l}.\typeT}
%	{\basis;\sorting  \judge P \hasType x:\typeT}
%	$        
%	\\[.3cm]			
%	$
%	\infer[$\rulelabel{T-Br}$]{\basis;\sorting \judge \branchAct{x}{\branch{l_1}{P_1} \branchSep \ldots \branchSep \branch{l_n}{P_n}} \hasType 
%	x:\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}}
%	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
%	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
%	$
%	\\[.4cm]	
%       	$
%	\infer[$\rulelabel{T-If}$]{\basis;\sorting \judge \ifthenelseAct{e}{P_1}{P_2} \hasType 
%	x:\typeT_1 \choiceType \typeT_2}
%	{\sorting \! \judge\! e \!\hasType\! \boolType &
%	\basis;\sorting  \judge P_1 \hasType x:\typeT_1 & \basis;\sorting  \judge P_2 \hasType x:\typeT_2}
%	$
%	\\[.3cm]	
%	\raisebox{.2cm}{$\basis\comp X:t;\sorting \judge X \!\hasType\! t$\ \rulelabel{T-Pvar}}			
%	\qquad
%	\infer[$\rulelabel{T-Rec}$]{\basis;\sorting \judge \recAct{X}{P} \hasType \recAct{t}{\typeT}}
%	{\basis\comp X:t;\sorting  \judge P \hasType \typeT}	
%	\\[.3cm]
%	$
%	\infer[$\rulelabel{T-Cmt}$]{\basis;\sorting \judge \commitAct{P}  \hasType 
%	x:\commitType.\typeT}
%	{
%	\basis;\sorting  \judge P \hasType x:\typeT 
%	}
%	$
%	\\[.3cm]
%	$\basis;\sorting \judge \roll \hasType x:\rollType$\ \ \rulelabel{T-Rll}	
%	\qquad
%	$\basis;\sorting \judge \abort \hasType x:\abortType$\ \ 
%	\rulelabel{T-Abt}
%	\\[.1cm]	
%	\hline
%	\end{tabular}
%	\caption{Typing system for \cherry\ processes (omitted rules).}
%	\label{fig:typingSystem_proc_omitted}
%	%\vspace*{.3cm}
%\end{figure}

%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}c@{}}
%	$\sorting \judge \ctrue \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{tt}}$}
%	\qquad
%	$\sorting \judge \cfalse \hasType \boolType$\ \ \rulelabel{T-Bool$_{\mathit{ff}}$}
%	\\[.4cm]	
%	$\sorting\comp x:S \judge x \hasType S$\ \ \rulelabel{T-Var}	
%	\qquad
%	$\sorting \judge 1 \hasType \intType$\ \ \rulelabel{T-Int}	
%	\qquad
%	$\sorting \judge\!\!``a" \hasType \strType$\ \ \rulelabel{T-Str}	
%	\\[.4cm]
%	$
%	\infer[$\!\rulelabel{T-Sum}$]{\sorting \judge +(e_1,e_2) \hasType \intType}
%	{\sorting \judge e_1 \hasType \intType &  \sorting \judge e_2 \hasType \intType}
%	\quad
%	\infer[$\!\rulelabel{T-And}$]{\sorting \judge \wedge(e_1,e_2) \hasType \boolType}
%	{\sorting \judge e_1 \hasType \boolType  & \sorting \judge e_2 \hasType \boolType}
%	$		
%        \\[.2cm]
%	\hline
%	\end{tabular}
%	\caption{Typing system for \cherry\ expressions (excerpt of omitted
%          rules).}
%	%\vspace*{.2cm}
%	\label{fig:typingSystem_exp_omitted}
%\end{figure}

%The syntax of the \cherry\ \emph{session types} is defined 
%in Fig.~\ref{fig:typeSyntax_cherry_omitted}. 
%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}r@{\ }c@{\ }l@{\quad}l@{}}
%	\\[-.7cm]
%	$S$ & ::= & $\boolType$ \quad $\mid$ \quad $\intType$ \quad $\mid$ \quad $\strType$  
%	& \textbf{Sorts}	
%	\\[.2cm]	
%	$\typeT$ & ::= & $\outType{S}.\typeT$ \ \ $\mid$ \ \
%	$\inpType{S}.\typeT$ \ \  $\mid$ \ \ 
%	$\selType{l}.\typeT$ 	 \ \  $\mid$ \ \ 
%	$\branchType{\branch{l_1}{\typeT_1}, \ldots, \branch{l_n}{\typeT_n}}$	
%	&  \textbf{Session types}
%	\\[.05cm]
%	& $\mid$ &  
%	$\typeT_1 \choiceType \typeT_2$ \ \ $\mid$ \ \ 
%	$t$ \ \ $\mid$ \ \ $\recType{t}.\typeT$ \ \ $\mid$ \ \ 
%	$\inactType$ \ \ $\mid$ \ \ 
%        \added{$\errType$} \ \ $\mid$ \ \ 
%	$\commitType.\typeT$ \ \ $\mid$ \ \ 
%	$\rollType$ \ \ $\mid$ \ \ 
%	$\abortType$
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\caption{\Cherry\ type syntax. 
%	}
%	\label{fig:typeSyntax_cherry_omitted}
%\end{figure}


%The omitted rules defining the semantics of types and type configurations are given in Fig.~\ref{fig:typeSemantics_ext_omitted} (symmetric rules for configurations are omitted).
%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{\hspace*{.8cm}}l@{\hspace*{.6cm}}r@{}}
%	$\outType{S}.\typeT \typeTrans{\outType{S}} \typeT$\ \ \rulelabel{TS-Snd}	
%	&
%	$\inpType{S}.\typeT \typeTrans{\inpType{S}} \typeT$\ \ \rulelabel{TS-Rcv}  
%	&
%	$\selType{l}.\typeT \typeTrans{\selTypeLabel{l}} \typeT$\ \ \rulelabel{TS-Sel}
%	\\[.4cm]
%	\multicolumn{2}{@{}l@{}}{
%	\raisebox{.8cm}{$\!\!
%	\branchType{\branch{l_1\!\!}{\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\typeT_n}}
%	\typeTrans{\branchTypeLabel{l_i}} \typeT_i$ \ \ $(1 \!\leq\! i \!\leq\! n)$\ \ \rulelabel{TS-Br}
%	}
%	}
%	&
%	$
%	\infer[$\rulelabel{TS-rec}$]
%	{\recType{t}.\typeT \typeTrans{\typeLab} \typeT'}
%	{\typeT\subst{\recType{t}.\typeT}{t} \typeTrans{\typeLab} \typeT'}
%	$
%\\[-.3cm]
%	$
%	\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_1$\ \ \rulelabel{TS-If$_1$}
%	&
%	$\typeT_1 \choiceType \typeT_2 \typeTrans{\tau} \typeT_2$\ \ \rulelabel{TS-If$_2$}
%	&
%%	\\[.4cm]
%%	$\commitType.\typeT \typeTrans{\commitLab} \typeT$\ \ \rulelabel{TS-Cmt}
%%	&
%%	$\rollType \typeTrans{\rollLab} \inactType$\ \ \rulelabel{TS-Rll}
%%	&
%%	$\abortType \typeTrans{\abortLab} \inactType$\ \ \rulelabel{TS-Abt}
%	\\[.4cm]
%	\end{tabular}
%	\begin{tabular}{@{}c@{}}
%%	$
%%	\infer[$\rulelabel{TS-Tau}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%%	{\typeT_1 \typeTrans{\tau} \typeT_1'}
%%	$	
%%	\\[.4cm]
%%	$
%%	\infer[$\rulelabel{TS-Com}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%%	{\typeT_1 \typeTrans{\!\outType{S}\!} \typeT_1'
%%	& &
%%	 \typeT_2 \typeTrans{\!\!\inpType{S}\!} \typeT_2'}	
%%	$	
%%	\\[.4cm]
%	$
%	\infer[$\rulelabel{TS-Lab}$]
%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%	\typered
%	\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2'}}
%	{\typeT_1 \typeTrans{\selTypeLabel{l}} \typeT_1'
%	& & 
%	 \typeT_2 \typeTrans{\branchTypeLabel{l}} \typeT_2'}
%	$	
%%	\\[.4cm]
%%	$
%%	\infer[$\rulelabel{TS-Cmt$_1$}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\imposed{\typeT_2}}{\typeT_2}}
%%	{\typeT_1 \typeTrans{\commitLab} \typeT_1' & & \checkpointType{\typeU}_2 \neq \typeT_2}
%%	$	
%%	\\[.4cm]
%%	$
%%	\infer[$\rulelabel{TS-Cmt$_2$}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeT_1'}{\typeT_1'} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}}
%%	{\typeT_1 \typeTrans{\commitLab} \typeT_1' & & \checkpointType{\typeU}_2 = \typeT_2}
%%	$	
%%	\\[.4cm]
%%	$
%%	\infer[$\rulelabel{TS-Rll$_1$}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeU_1}{\typeU_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeU_2}}
%%	{\typeT_1 \typeTrans{\rollLab} \typeT_1'}
%%	$	
%%	\\[.4cm]
%%	$
%%	\infer[$\rulelabel{TS-Abt$_1$}$]
%%	{\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeU}_1}{\typeT_1} \confcomp \conf{\checkpointType{\typeU}_2}{\typeT_2}
%%	\typered
%%	\initConf{\typeT}{\typeT'}\conf{\typeT}{\typeT} \confcomp \conf{\typeT'}{\typeT'}}
%%	{\typeT_1 \typeTrans{\abortLab} \typeT_1'}
%%	$	
%	\hspace*{12.1cm}\\
%	\hline
%	\end{tabular}
%	\caption{Semantics of types and type configurations 
%	(omitted rules).
%	}
%	\label{fig:typeSemantics_ext_omitted}
%	%\vspace*{-.2cm}
%\end{figure}
%
%
%
%The omitted rules defining the error semantics are given 
%in Fig.~\ref{tab:error_red_omitted}.
%%
%\begin{figure*}[t]
%	\centering
%	\small
%	\begin{tabular}{@{}c@{}}
%%	$
%%	\infer{
%%	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
%%	\mid 
%%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%%	\fwred
%%	\comError
%%	}
%%	{
%%	P_1 \auxrel{\send{{k}}{v}} P_1'
%%	\qquad
%%	\neg P_2 \BarbInp{k}
%%	\quad\qquad 
%%	$\rulelabel{E-Com1}$
%%	}
%%	$	
%%	\qquad 
%	$
%	\infer{
%	\logged{{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\comError
%	}
%	{
%	P_1 \auxrel{\receive{{k}}{x}} P_1'
%	\quad
%	\neg P_2 \BarbOut{k}
%        \ \ 
%        \added{\neg P_2 \Barb{roll}}
%	\qquad
%	$\rulelabel{E-Com2}$
%	}
%	$	
%	\\[.3cm]
% \hspace*{-.9cm}
%	$\quad
%	\infer{
%	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred
%	\comError
%	}
%	{
%	P_1 \auxrel{\select{{k}}{l}} P_1'
%	\quad
%	\neg P_2\BarbBranching{k}{l}
%        \ \ \added{\neg P_2 \Barb{roll}}
%	\  \
%	$\rulelabel{E-Lab$_1$}$
%	}
%	$			
%	\quad
%	$
%	\infer{
%	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid 
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred
%	\comError
%	}
%	{
%	P_1 \auxrel{\branching{k}l} P_1'
%	\quad
%	\neg P_2\BarbSelect{k}{l}
%        \ \ \added{\neg P_2 \Barb{roll}}
%	\ \ 
%	$\rulelabel{E-Lab$_2$}$
%	}
%	$
%		\\[.3cm]	
%	$
%	\infer[$\rulelabel{E-Cmt$_1$}$]{
%	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\mid
%	\logged{\genSession}{\imposed{P_2}} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	& & 
%	\checkpointType{Q_2} \neq P_2	
%	}
%	$	
%	\\[.3cm]
%	$
%	\infer[$\rulelabel{E-Cmt$_2$}$]{
%	\logged{\ce{\genSession}}{\checkpointType{Q_1}} P_1 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\fwred 
%	\logged{\ce{\genSession}}{P_1'} P_1' 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	}
%	{
%	P_1 \auxrel{\commitLab} P_1'
%	& & 
%	\checkpointType{Q_2} = P_2
%	}
%	$	
%	\\[.3cm]		
%	$
%	\infer[$\rulelabel{E-Rll$_1$}$]{
%	\logged{\ce{\genSession}}{Q_1} P_1 
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%	\bwred
%	\logged{\ce{\genSession}}{Q_1} Q_1
%	\mid
%	\logged{\genSession}{\checkpointType{Q_2}} Q_2
%	}
%	{	
%	P_1 \auxrel{\rollLab} P_1'		
%	}
%	$	
%%	\\[.3cm]	
%%	$
%%	\infer[$\rulelabel{E-Rll$_2$}$]{
%%	\logged{\ce{\genSession}}{\imposed{Q_1}} P_1 
%%	\mid
%%	\logged{\genSession}{\checkpointType{Q_2}} P_2
%%	\fwred 
%%	\rollError
%%	}
%%	{
%%	P_1 \auxrel{\rollLab} P_1'	
%%	}
%%	$	
%	\\[.1cm]
%	\hline
%	\end{tabular}	
%	\caption{\Cherry\ semantics: error reductions (omitted rules).}
%	\label{tab:error_red_omitted}
%	%\vspace*{-.2cm}
%\end{figure*}
%%
%The semantics of \cherry\ is extended by the additional rules, 
%where \rulelabel{E-Cmt$_1$} and \rulelabel{E-Cmt$_2$} replace \rulelabel{F-Cmt},
%and \rulelabel{E-Rll$_1$} replaces  \rulelabel{B-Rll},
%and $\checkpointType{\ }$ is used in the checkpoints of the other rules.
%%
%%The definition of these rules relies  on the notion of \emph{barb} predicates, whose straightforward definition is: $P\Barb{\mu}$ holds if there exists $P'$ such that $P \Rightarrow P'$ and $P'$ can perform an action $\mu$, where $\mu$ stands for $k?$, $k!$ ,$k\triangleleft l$ or $k\triangleright l$ (i.e., input, output, select and branching action along session channel $k$); $\Rightarrow$ is the reflexive and transitive closure of $\auxrel{\ite}$.




%\newpage
%%%%%%%%%%%%%%%%%%%%% MULTIPARTY
%The omitted syntax of multiparty \cherry\ and of multiparty session types 
%are in Fig.~\ref{fig:syntax_cherry_pi_multi_omitted} and~\ref{fig:typeSyntax_cherry_multi_omitted},
%respectively.
%\begin{figure}[h]
%\small
%	\begin{tabular}{@{}r@{ }c@{\ }l@{\ \ }l@{}}
%	$C$ & ::= & $\cdots$    $\mid$ 
%	                   $\mrequestAct{a}{\role{p}}{x}{P}$  $\mid$  $\macceptAct{a}{\role{p}}{x}{P}$
%	                   & \!\!\!\!\!\!\!\!\!\textbf{Collaborations}
%	\\[.3cm]
%	$P$ & ::= &  $\cdots$  $\mid$ 
%                                        $\msendAct{\sessId}{\role{p}}{e}{P}$ 
%		         $\mid$  $\mreceiveAct{\sessId}{\role{p}}{y:S}{P}$ 	
%		         $\mid$  $\mselectAct{\sessId}{\role{p}}{l}{P}$ 
%		         $\mid$  $\mbranchAct{\sessId}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
%		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}$ 
%			& \ \ \ \textbf{Processes}
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.4cm}	
%	\caption{Multiparty \cherry\ runtime syntax; the omitted parts are as in Fig.~\ref{fig:syntax_cherry_pi_ext} (omitted rules).}
%	%\vspace*{.2cm}	
%	\label{fig:syntax_cherry_pi_multi_omitted}
%\end{figure}
%
%\clearpage 
%
%%
%\begin{figure}[h]
%	\centering
%	\small
%	\begin{tabular}{@{}r@{\ }c@{\ }l@{}l@{}}
%	$\typeT\!$ & ::= &  &\!\!  \ldots   $\mid$  
%	$\moutType{\role{p}}{\role{q}}{S}.\typeT$  $\,\mid\,$ 
%	$\minpType{\role{p}}{\role{q}}{S}.\typeT$   $\,\mid\,$ 
%	$\mselType{\role{p}}{\role{q}}{l}.\typeT$ 	$\,\mid\,$  
%	$\mbranchType{\role{p}}{\role{q}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}$
%	\ \ \textbf{Types}
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.6cm}	
%	\caption{Multiparty \Cherry\ type syntax; 
%	the omitted parts are as in  Fig.~\ref{fig:typeSyntax_cherry} (omitted rules).
%	}
%	\label{fig:typeSyntax_cherry_multi_omitted}
%	%\vspace*{.5cm}
%\end{figure}
%
%The omitted rules of the multiparty semantics are reported in 
%Fig.~\ref{fig:reduction_pic_multi_omitted}.
%\begin{figure*}[!h]
%	\centering
%	\small
%        \begin{tabular}{@{ }c@{}}
%	$\msendAct{s\mendpoint{\role{p}}}{\role{q}}{e}{P} 
%	\auxrel{\!\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}\!} \!P$
%	\ ($\expreval{e}{v}$)
%	 \rulelabel{M-P-Snd}
%	\qquad
%	$\mreceiveAct{s\mendpoint{\role{p}}}{\role{q}}{y\!:\!S}{P}
%	 \auxrel{\!\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{y}\!\!} \!P$
%	\rulelabel{M-P-Rcv}
%	\\[.5cm]
%	\end{tabular}	
%	\\
%	\begin{tabular}{@{}l@{}}
%		$\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}$ 
%	$\ \ \fwred\ \ $
%	\\[.1cm]
%	\quad 	
%	$\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}$
%	\qquad\quad\qquad\qquad\qquad\ \
%	$I\!=\!\{1,..,n\!-\!1\}$\quad
%	\rulelabel{M-F-Con}	
%	\\[.1cm] 	
%	\quad 	
%        $(\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
%        \!\mid\! 
%        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})$
%	\\[.5cm]
%	\end{tabular}
%	\begin{tabular}{@{}c@{}}	
%	$
%	\infer[$\rulelabel{M-F-Com}$]{
%	\loggedShort{\ce{\genSession}}{Q_1} P_1 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2
%	\ \fwred\ 
%	\loggedShort{\ce{\genSession}}{Q_1} P_1' 
%	\mid 
%	\loggedShort{\genSession}{Q_2} P_2'\subst{v}{x}	
%	}
%	{
%	P_1 \auxrel{\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}} P_1'
%	& & 
%	P_2 \auxrel{\receive{s\mendpoint{\role{q}}\mendpoint{\role{p}}}{x}} P_2'	
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-F-Cmt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \fwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{P'} P' 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{P_i} P_i)
%	}
%	{
%	P \auxrel{\commitLab} P'
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-B-Rll}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} Q 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} Q_i)
%	}
%	{
%	P \auxrel{\rollLab} P'
%	}
%	$
%	\\[.4cm]
%	$
%	\infer[$\rulelabel{M-B-Abt}$]{
%	\singleSession{s}{C}(
%	\logged{\ce{\genSession}}{Q} P 
%	\ \mid \ 
%	\prod_{i\in I}\logged{\genSession}{Q_i} P_i)
%	\ \bwred\ 
%	C}
%	{
%	P \auxrel{\abortLab} P'
%	}
%	$
%	\\[.1cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.4cm}	
%	\caption{Multiparty \cherry\ semantics: forward and backward reductions (excerpt of omitted rules).}
%	\label{fig:reduction_pic_multi_omitted}
%	\vspace*{.7cm}	
%\end{figure*}
%
%\clearpage
%The omitted rules of the multiparty type system  are reported in 
%Fig.~\ref{fig:typingSystem_multi_omitted}.
%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{c}
%	$
%	\infer[$\rulelabel{M-T-Req}$]{\mrequestAct{a}{\role{p}}{x}{P} \hasType \{\ce{a}\mendpoint{\role{p}}:\typeT\}}
%	{\emptyset;\emptyset \judge P \hasType x:\typeT}
%	$		
%	\qquad
%	$
%	\infer[$\rulelabel{M-T-Acc}$]{\macceptAct{a}{\role{p}}{x}{P} \hasType \{a\mendpoint{\role{p}}:\typeT\}}
%	{\emptyset;\emptyset \judge P \hasType x:\typeT}
%	$
%	\\[.4cm]
%        $
%	\infer[$\rulelabel{M-T-Snd}$]{\basis;\sorting \judge \msendAct{x}{\role{p}}{e}{P}
%	\hasType x:\moutType{\role{\_}}{\role{p}}{S}.\typeT}
%	{\sorting \judge e \hasType S & & \basis;\sorting \judge P \hasType x:\typeT}
%	$
%        \\[.4cm]
%        $
%	\infer[$\rulelabel{M-T-Rcv}$]{\basis;\sorting \judge \mreceiveAct{x}{\role{p}}{y:S}{P}
%	\hasType x:\minpType{\role{\_}}{\role{p}}{S}.\typeT}
%	{\basis;\sorting\comp y:S \judge P \hasType x:\typeT}
%	$
%        \\[.4cm]
%	$
%	\infer[$\rulelabel{M-T-Sel}$]{\basis;\sorting \judge \mselectAct{x}{\role{p}}{l}{P} \hasType 
%	x:\mselType{\_}{\role{p}}{l}.\typeT}
%	{\basis;\sorting  \judge P \hasType x:\typeT}
%	$        
%	\\[.4cm]			
%	$
%	\infer[$\rulelabel{M-T-Br}$]{\basis;\sorting \judge 
%	\mbranchAct{x}{\role{p}}{\branch{l_1\!\!}{\!\!P_1}
%		          \branchSep \ldots \branchSep \branch{l_n\!\!}{\!\!P_n}}
%	\hasType 
%	x:\mbranchType{\_}{\role{p}}{\branch{l_1\!\!}{\!\!\typeT_1}, \ldots, \branch{l_n\!\!}{\!\!\typeT_n}}}
%	{\basis;\sorting  \judge P_1 \hasType x:\typeT_1 && \ldots 
%	 && \basis;\sorting  \judge P_n \hasType x:\typeT_n}
%	$
%	\\[.1cm]	        
%	\hline
%	\end{tabular}
%	\vspace*{-.3cm}
%	\caption{Multiparty \cherry\ typing system (the omitted rules are as in
%	Fig.~\ref{fig:typingSystem_coll}, \ref{fig:typingSystem_proc} and \ref{fig:typingSystem_exp_omitted}).}
%	%\vspace*{-.1cm}	
%	\label{fig:typingSystem_multi_omitted}
%\end{figure}
%
%Finally, the omitted rules of the multiparty type configurations semantics are reported in 
%Fig.~\ref{fig:typeSemantics_ext_multi_omitted}.
%\begin{figure}[!h]
%	\centering
%	\small
%	\begin{tabular}{@{}l@{\qquad\quad}l@{}}
%	$\moutType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Snd}	
%	& 
%	$\minpType{\role{p}}{\role{q}}{S}.\typeT \typeTrans{\minpType{\role{p}}{\role{q}}{S}} \typeT$\ \ \rulelabel{M-TS-Rcv}  
%	\\[.5cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[$\rulelabel{M-TS-Com}$]
%	{\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\conf{\checkpointType{\typeU}_j}{\typeT_j}
%	\confcomp 	
%	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\\[.1cm] 
%	\quad
%	\typered
%	\ \
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i'} 
%	\confcomp 
%	\conf{\checkpointType{\typeU}_j}{\typeT_j'}
%	\confcomp 	
%	\prod_{h\in I-\{i,j\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\end{array}}
%	{\typeT_i \typeTrans{\moutType{\role{p}}{\role{q}}{S}} \typeT_i'
%	& &
%	 \typeT_j \typeTrans{\minpType{\role{q}}{\role{p}}{S}} \typeT_j'}	
%	$
%	}
%	\\[.8cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[\ \	
%	 \checkpointType{\typeU}_h' \! =\!\! 
%	 \left\{
%	 \begin{array}{ll}
%	 \checkpointType{\typeU}_h & \textrm{if}\ \checkpointType{\typeU}_h = \typeT_h \\
%	 \imposed{\typeT_h} & \textrm{otherwise}
%	 \end{array}
%	 \right.
%	\ \
%	$\rulelabel{M-TS-Cmt}$
%	]	
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\\
%	\quad
%	\typered
%	\ \
%	\minitConf{\typeT^I}
%	\conf{\typeT_i'}{\typeT_i'} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h}
%	\end{array}
%	}
%	{\typeT_i \typeTrans{\commitLab} \typeT_i'}	
%	$
%	}
%	\\[.8cm]
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\typeU_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\
%	\typered
%	\
%	\minitConf{\typeT^I}
%	\conf{\typeU_i}{\typeU_i}  
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeU_h}
%	\end{array}
%	}
%	{\hspace*{4cm}
%	\typeT_i \typeTrans{\rollLab} \typeT_i' 
%	\hspace*{4cm}
%	$\rulelabel{M-TS-Rll}$
%	}	
%	$
%	}
%	\\[.8cm]	
%	\multicolumn{2}{@{}c@{}}{
%	$
%	\infer[$\rulelabel{M-TS-Abt}$]
%	{
%	\begin{array}{l}
%	\minitConf{\typeT^I}
%	\conf{\checkpointType{\typeU}_i}{\typeT_i} 
%	\confcomp 
%	\prod_{h\in I-\{i\}}\conf{\checkpointType{\typeU}_h}{\typeT_h}
%	\
%	\typered
%	\
%	\minitConf{\typeT^I}
%	\prod_{k\in I}\conf{\typeT^k}{\typeT^k}
%	\end{array}
%	}
%	{\typeT_i \typeTrans{\abortLab} \typeT_i' }	
%	$	
%	}
%	\\[.4cm]
%	\hline
%	\end{tabular}
%	\vspace*{-.3cm}	
%	\caption{Multiparty \cherry\ type semantics (excerpt of rules, 
%	where $I=\{1,\ldots,n\}$, $i,j\in I$, and $\typeT^{I}$ denotes $\typeT^1,\ldots,\typeT^n$).}
%	\label{fig:typeSemantics_ext_multi_omitted}
%	%\vspace*{-.2cm}
%\end{figure}
\clearpage


==> tex/proofs_multiparty.tex <==
% !TEX root = ../rev_sessions@fsttcs.tex


\subsection{Multiparty session results}
\label{proofs:multiparty}

All notions and concepts of our rollback recovery approach smoothly 
extend to the multiparty case. As consequence, all properties in Sec.~\ref{sec:properties}
still hold in the extended setting.
Their proofs indeed follow the same structure of the binary case and only 
differ for the technicalities concerning the extended definitions. 


\subsubsection{Decidability result}

\theoremApp{\ref{th:decidability}}
Let $\typeT_1,\ldots,\typeT_n$ be filled multiparty session types,
checking if \mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$}
holds
is decidable.
\begin{proof} 
By definition of Compliance in Sec.~\ref{sec:multiparty}, checking 
\mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$} consists in
checking that types $\typeT_1', \ldots,\typeT_n'$ of each configuration
$\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h'}$
such that 
$\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\typeT_h}{\typeT_h}
\typered^*
\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeU}_h'}{\typeT_h'}
\typered\!\!\!\!\!\!\!\!/\ \ \  $
(i.e., type configurations that are reachable from the initial one and that cannot further evolve)
are $\inactType$ types.
Thus, to prove that the compliance check is decidable we have to show that the number of 
these reachable configurations is finite. 
Let us consider the transition system $TS=\langle \mathcal{S}, \mathcal{R} \rangle$ associated to the type configuration 
$t= \minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\typeT_h}{\typeT_h}$
by the  reduction semantics of types (Fig.~\ref{fig:typeSemantics_ext_multi}):
the set $\mathcal{S}$ of states  corresponds to the set of type configurations reachable from $t$,
i.e. $\mathcal{S}=\{\, t' \ \mid \  t \typered^* t'\,\}$, 
while the set $\mathcal{R}$ of system transitions corresponds to set of the type reductions 
involving configurations in $\mathcal{S}$, i.e.
$\mathcal{R}=\{ (t',t'') \in \mathcal{S} \times \mathcal{S}  \ | \ t' \typered t''\}$.
%
Hence, checking \mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$} boils down to check the type configurations
corresponding to the leaves (i.e., states without outgoing transitions) of $TS$. 
Specifically, given a leaf of $TS$ corresponding to 
$t= \minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in \{1,\ldots,n\}}\conf{\checkpointType{\typeV_h}'}{\typeV_h}$, 
we have to check if $\typeV_1=\ldots=\typeV_n=\inactType$.
The decidability of this check therefore depends on the finiteness of $TS$.
This result is ensured by the fact that: : \emph{(i)} backward reductions connect states of $TS$
only to previously visited states of $TS$ (Theorem~\ref{th:trace_multi}),
and \emph{(ii)} our language of types (Fig.~\ref{fig:typeSyntax_cherry_multi}) 
corresponds to a CCS-like process algebra without 
static operators (i.e., parallel and restriction operators) within recursion (see \cite[Sec.~7.5]{CCS}). 
\end{proof}



\subsubsection{Reversibility results}

As in Appendix~\ref{app:ReversibilityResults}, we will indicate with $C\instr{s}\fwbwred C'$ the fact that the reduction is taking place on session $s$. 

\begin{lemma}[Swap Lemma]\label{lm:swp_multi}
Let $C$ be a  collaboration and $s$ and $r$ two sessions. If $C\instr{s}{\fwbwred} C_1 \instr{r}{\fwbwred} C_2$ then
there exists a collaboration $C_3$ such that $C\instr{r}{\fwbwred} C_3 \instr{s}{\fwbwred} C_2$.
\end{lemma}
\begin{proof}
By case analysis on the reductions $\instr{s}{\fwbwred} $ and $\instr{r}{\fwbwred}$.
\end{proof}

\begin{lemma}\label{lm:rearr_multi}
Let $C$ be a collaboration. 
If $C\fwbwred^{*}C_1$, then for any session $s$ in $C_1$ there exists a collaboration $C_0$
such that 
$C \fwbwred^{*}C_0\instr{s}{\fwbwred}{\!}^*\ C_1$ and $s$ is never used in the trace $C \fwbwred^{*}C_0$.
\end{lemma}
\begin{proof}
By induction on the number $n$ of reduction on $s$. If there are no reductions then the thesis banally holds.
Otherwise we can take the very last reduction on $s$, that is the closest one to $C_1$ and iteratively apply
 Lemma~\ref{lm:swp_multi} in order to bring it to the very end. Then we can conclude by induction on a trace with less occurrences of reductions on $s$.
\end{proof}

As in Appendix~\ref{app:ReversibilityResults}, thanks to Lemma~\ref{lm:rearr_multi} 
without loosing of generality we can focus just on a sigle session, say $s$, and to consider 
collaboration initial for $s$.

\label{reversibility_proofs_multi}

\begin{lemma}\label{lemma:init_multi}
Let $C$ be an initial collaboration such that
$C \fwbwred^{*} C_1$. If $C_1\abt C_2$ then $C_2 \congr C$.
\end{lemma}
\begin{proof}
Since $C$ is \textit{initial}, without losing of generality we can assume
\begin{align*}
 &C\congr \mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i}
 \end{align*}
 with $I=\{1,..,n-1\}$.
% \todo{too informal?}
%{\color{blue}We can consider collaborations only made of two participants because in our framework 
%we focus on binary sessions without delegation, implying that for each session there will be 
%two interacting participants and that multiple sessions running in parallel do not interfere 
%each other. }
 
The first reduction of $C \fwbwred^{*} C_1$ has to be an application of rule \rulelabel{M-F-Con}, that is
\begin{align*}
&C \fwred 	
\singleSession{s\!}{\!(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I}\macceptAct{a}{i}{x}{P_i})}\\
&  \qquad \ \ 
        (\loggedShort{\ce{s}}{P_n\subst{s\mendpoint{n}}{x} }	P_n\subst{s\mendpoint{n}}{x}
        \!\mid\! 
        \prod_{i\in I} \loggedShort{s}{P_i\subst{s\mendpoint{i}}{x}} P_i\subst{s\mendpoint{i}}{x})
= C' 
\end{align*}
and, by hypothesis, $C' \fwbwred^{*} C_1$.	

Now, no matter the shape of processes in $C_1$ by applying rule \rulelabel{M-B-Abt}, 
and possibly \rulelabel{M-B-Str}, we will go back to $C$, that is $C_1 \abt C$, as desired.
\end{proof}


\begin{lemma}\label{lemma:fw_trace_multi}
Let $C$ be a reachable collaboration, such that $C\cmt C_1$. If $C_1\fwred^{*}C_2 \rll C_3$ and there
is no commit in $C_1\fwred^{*}C_2$, then $C_3 \congr C_1$.
\end{lemma}
\begin{proof}
As in Lemma~\ref{lemma:fw_trace}'s proof, 
by hypothesis, there is no commits in $C_1 \fwred^{*} C_2$, and this implies that the log part
of the $C_1$ will never change. Hence, by applying \rulelabel{M-B-Rll} and \rulelabel{M-B-Par} to 
$C_2$we can conclude.
\end{proof}


\begin{theorem}
\label{th:trace_multi}
Let $C_0$ be an initial collaboration. If $C_0 \fwbwred^{*}C_1$ then $C_0 \fwred^{*}C_1$.
\end{theorem}
\begin{proof}
By induction on the number $n$ of backward reductions contained into $C_0 \fwbwred^{*}C_1$.
 The base case
($n=0$)
trivially holds. In the inductive case, let us take the backward reduction which is the
nearest to $C_0$. That is:
$$C_0 \fwred^{*} C' \bwred C''\fwbwred^{*}C_1$$
Depending whether it is an $\abt$ or a $\rll$ we can apply respectively Lemma~\ref{lemma:init_multi}
or Lemma~\ref{lemma:fw_trace_multi} to obtain a forward trace of the form
$$C_0 \fwred^{*} C''\fwbwred^{*}C_1$$
and we can conclude by applying the inductive hypothesis on  the obtained trace which contains
less backward moves with respect to the original one.
\end{proof}


\begin{lemma}
\label{lemma:safe_roll_multi}
Let $C_1$ and $C_2$ be two reachable collaborations. 
$C_1 \bwred C_2$ then $C_2 \fwred^{*} C_1$.
\end{lemma}
\begin{proof}(Skecth)
Since $C_1$ is a reachable collaboration, we have that there exists an initial collaboration $C_0$
such that $C_0\fwbwred^{*}C_1$.
By applying Theorem~\ref{th:trace_multi} we can rearrange the trace 
such that it contains just forward transitions as follows
$$C_0\fwred^{*} C_1$$
%
If the backward reduction is obtained by applying \rulelabel{M-B-Abt},
by Lemma~\ref{lemma:init_multi} we have $C_2\congr C_0$, from which the thesis trivially follows.
Instead, if the backward reduction is obtained by applying \rulelabel{M-B-Rll},
we proceed by case analysis depending on the presence of commit reductions in the trace.
If they are present, we select the last of such commit, that is we can decompose the trace in the following way:
$$C_0 \fwred^{*}\ \cmt C_{cmt} \fwred^{*}C_1\rll C_2$$
and by applying Lemma~\ref{lemma:fw_trace_multi} we have that $C_2 \fwred^{*}\congr C_1$ as desired.
%
In the case there is no commit in the trace, 
%we have to distinguish two cases: 
%either \rulelabel{B-Abt} or \rulelabel{B-Rll}
%is applied.
%without losing of generality we can assume
%\begin{align*}
% &C_0\congr 		\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2} \mid C^{\circ}
%\\
% & C_0 \fwred
% \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2)\mid C^{\circ}
%\end{align*}
%%In the first case we have that $C_2 \congr C_0$ and the thesis trivially follows; in the second case
%%we have $C_2 \congr \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2)$
%%and we can conclude by noticing that $C_0\fwred C_2$.
%By rule \rulelabel{B-Rll}, $C_2 \congr \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2) \mid C^{\circ}$. Thus, 
we can conclude by noticing that $C_0\fwred C_2$
must be the first reduction in $C_0\fwred^{*} C_1$.
\end{proof}


\begin{lemma}
\label{lemma:determinism_multi}
%Let C be a reachable collaboration. If $C\bwred C'$ and $C\bwred C''$ then $C' \congr C''$
Let $C$ be a reachable collaboration. If $C\rll C'$ and $C\rll C''$ then $C' \congr C''$.
\end{lemma}
\begin{proof}(Skecth)
Since $C$ is a reachable collaboration, it is has been generated by an initial collaboration
$C_0$, % of the form $C_0 = \requestAct{a}{x}{P_1}   \mid \acceptAct{a}{x}{P_2}$, 
and by Theorem~\ref{th:trace_multi} we have that
$C_0 \fwred^{*} C$. We distinguish two cases, whether in the trace
there has been at least one commit or not. In the first case, we can decompose the trace in such a way
to single out the last commit as follows:
$$C_0 \fwred^{*}C_{cmt} \fwred^{*} C$$
so that in the reduction $C_{cmt} \fwred^{*} C$ there is no commit. 
If from $C$ the rollbacks $C\rll C'$ and $C\rll C''$ are triggered by the same process, 
the thesis trivially follows.
In the other case, we have that
%:
%$$C_{cmt} \congr 	\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_2 \mid \logged{\genSession}{Q_1} Q_2) \mid C^{\circ}
%$$
at least two processes, say $P$ and $Q$, are able to trigger a rollback. If the roll action is executed by $P$ we have that
$C_{cmt} \rll C'$.
If the roll is triggered by $Q$ we have that $C_{cmt} \rll C''$.
And we can conclude by noticing that $C' \equiv C''$, as desired.
\end{proof}

\theoremApp{\ref{lemma:undoability}}
Let C be a reachable collaboration. 
If $C \cmt C'$ then there exists no $C''$ such that
$C' \fwred^{*}\rll C''$ and $C'' \fwred^{+} C$.
\begin{proof}
We proceed by contradiction. Suppose that there exists $C''$ such that 
$C' \fwred^{*}\rll C''$ and $C'' \fwred^{+} C$.
Since $C$ is a reachable collaboration, thanks to Theorem~\ref{th:trace_multi}
we have that there exists an initial collaboration $C_0$ 
such that $C_0\fwred^{*}C\cmt C'$. Since a rollback brings back the 
collaboration to a point before a commit, this means it has been restored a commit 
previous to the last one (by \rulelabel{M-B-Rll}, indeed, only processes stored in logs 
can be committed). 
This implies that there exist at least two different commits in the trace
such that
$$C_0 \fwred^{*}C_{cmt}\fwred^{*}C \cmt C'\fwred^{*}\rll C''$$
%
with $C'' = C_{cmt}$. We have that $C''\fwred^{+} C \cmt C'\fwred^{*}C_{rl}$, 
where $C_{rl}$ is the collaboration that perform the roll reduction.
Now since the last commit has been done by $C$, supposing that the commit is triggered by
$P^c$, which evolves to ${P^c}'$ in doing that,  we have that:
\begin{align*}
&C \congr 	\singleSession{s}{C_0}(\logged{\genSession}{P} P^c \mid \prod_{i\in I}\logged{\genSession}{Q_i} Q_i^c) 
\end{align*}
and
\begin{align*}
 C'= \singleSession{s}{C_0}(\logged{\genSession}{{P^c}'} {P^c}' \mid \prod_{i\in I}\logged{\genSession}{Q_i^c} Q_i^c)
\end{align*}
Now, by hypothesis we have that $C'\fwred^{*} C_{rl}$ without any commit being present in the trace, hence:
$$C_{rl} \congr 	\singleSession{s}{C_0}(\logged{\genSession}{{P^c}'} P^{rl} \mid \prod_{i\in I}\logged{\genSession}{Q_i^c} Q_i^{rl}) $$
By hypothesis, from $C_{rl}$ a rollback is possible. 
Regardless the rollback is triggered by $P_{rl}$ or  $Q_{rl}$, we have that
$C_{rl} \rll C'$. Now, from $C'$ we cannot reach $C$ ($C'\ \fwred^{+}\!\!\!\!\!\!\!\!\!\!/\ \ \ \  C$), 
as $C'$ is derived from $C$ and the rollback can only bring the collaboration back to $C'$. 
This violates the hypothesis, and hence we conclude. 
\end{proof}



\subsubsection{Soundness results}
\label{soundness_proofs}
%To prove our soundness results, we need to introduce some auxiliary lemmas, which 
%rely on the following definitions:
%\begin{itemize}
%\item a process $\checkpointType{P}$ and  a type $\checkpointType{\typeT}$
%are in \emph{checkpoint accordance} if $\checkpointType{P}=P$ implies $\checkpointType{\typeT}=\typeT$,
%and $\checkpointType{P}=\imposed{P}$ implies $\checkpointType{\typeT}=\imposed{\typeT}$;
%\item let $\actionLab$ a process label, its \emph{dual label} $\bar{\actionLab}$ is defined as follows:
%$\overline{\send{k}{v}}=k?$,
%$\overline{\receive{k}{x}}=k!$,
%$\overline{\select{k}{l}}=\branching{k}l$,
%$\overline{\branching{k}l}=\select{k}{l}$; this notion of duality straightforwardly extends to type labels;
%\item the function $\mFunc{\sorting}{\cdot}$, mapping process labels to type labels under sorting $\sorting$, is defined as follows:
%$\mFunc{\sorting}{\send{k}{v}}=\outType{S}$ with $\sorting \judge v \hasType S$,
%$\mFunc{\sorting}{\receive{k}{x}}=\inpType{S}$ with $\sorting \judge x \hasType S$,
%$\mFunc{\sorting}{\select{k}{l}}=\selTypeLabel{l}$,
%$\mFunc{\sorting}{\branching{k}l}=\branchTypeLabel{l}$,
%$\mFunc{\sorting}{\commitLab}=\commitType$,
%$\mFunc{\sorting}{\rollLab}=\rollType$,
%$\mFunc{\sorting}{\abortLab}=\abortType$, and
%$\mFunc{\sorting}{\ite}=\tau$.
%\end{itemize}
%
%
%The following lemma states that each reduction of a reachable collaboration corresponds 
%to a reduction of its configuration types.
\begin{lemma}\label{lemma:subj_multi}
Let $C=\singleSession{s}{C'}\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i}} P_i$ 
be a reachable collaboration,
with $I=\{1,..,n\}$, 
$C'=(\mrequestAct{a}{n}{x}{R_n}\, \mid \, \prod_{i\in I-\{n\}}\macceptAct{a}{i}{x}{R_i})$,
and for all $i\in I$
{$(\emptyset;\emptyset \judge R_i \hasType x:\typeT_i)$},
\mbox{$\compliant(\typeT_1,\ldots,\typeT_n)$},
{$(\basis_i;\sorting_i \judge Q_i\subst{x}{s\mendpoint{i}} \hasType x:\typeV_i)$},
{$(\basis_i';\sorting_i' \judge P_i\subst{x}{s\mendpoint{i}} \hasType x:\typeU_i)$}.
If $C \fwbwred 
\singleSession{s}{C'}\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i'}} P_i'$
then there exist $\typeV_i'$ and $\typeU_i'$ such that
$\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in I}\conf{\checkpointType{\typeV_h}}{\typeU_h}
\typered
\minitConf{\typeT^1,\ldots,\typeT^n}
\prod_{h\in I}\conf{\checkpointType{\typeV_h'}}{\typeU_h'}
$
with 
$\checkpointType{Q_i'}$ in checkpoint accordance 
with $\checkpointType{\typeV_h'}$, and for all $i\in I$
\mbox{$(\hat{\basis}_i;\hat{\sorting}_i \judge Q_i'\subst{x}{s\mendpoint{i}} \hasType x:\typeV_i')$},
\mbox{$(\hat{\basis}_i';\hat{\sorting}_i' \judge P_i'\subst{x}{s\mendpoint{i}} \hasType x:\typeU_i')$}.
\end{lemma}
\begin{proof}(Skecth)
We have two cases depending whether the reduction $\fwbwred$
has forward or backward direction. 
\begin{description}
\item $(\fwbwred \,=\, \fwred).$
From rule \rulelabel{M-F-Res}, we have 
$\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i}} P_i
\fwred 
\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i'}} P_i'$.
We prove the result by case analysis on the last rule applied in 
the inference of the above reduction.
%
%\begin{itemize}
%\item \rulelabel{F-Com}. 
%In this case we have $P_2 \auxrel{\send{\ce{s}}{v}} P_2'$,
%$Q_2 \auxrel{\receive{s}{z}} Q_2''$, with $Q_2'=Q_2''\subst{v}{z}$,
%$\checkpointType{P_1'}=\checkpointType{P_1}$ and 
%$\checkpointType{Q_1'}=\checkpointType{Q_1}$.
%Thus, $P_2\subst{x}{\ce{s}}=\sendAct{x}{e}{P_2'\subst{x}{\ce{s}}}$
%for some $e$ such that $\expreval{e}{v}$, and 
%$Q_2\subst{y}{{s}}=\receiveAct{y}{z:S'}{Q_2'\subst{y}{{s}}}$.
%By rule \rulelabel{T-Send}, we have that $\typeT_2=\outType{S}.\typeT_2'$,
%with $\sorting_2 \judge e \hasType S$, (hence $\sorting_2 \judge v \hasType S$),
%and $\basis_2;\sorting_2 \judge P_2'\subst{x}{\ce{s}} \hasType x:\typeT_2'$
%(hence $\hat{\basis}_2 = \basis_2$ and $\hat{\sorting}_2 = \sorting_2$).
%Similarly, by rule \rulelabel{T-Rcv}, we have that 
%$\typeU_2=\inpType{S'}.\typeU_2'$ and 
%$\basis_2';\sorting_2'\comp z:S' \judge Q_2''\subst{y}{{s}} \hasType y:\typeU_2'$
%(hence $\hat{\basis}_2' = \basis_2'$ and $\hat{\sorting}_2' = \sorting_2'\comp z:S'$).
%By rules \rulelabel{TS-Snd} and \rulelabel{TS-Rcv}, we get
%$\typeT_2 \typeTrans{\outType{S}} \typeT_2'$ and 	
%$\typeU_2 \typeTrans{\inpType{S'}} \typeU_2$.
%Now, reasoning by contradiction, let us suppose that $S\neq S'$. Thus, the term 
%$\initConf{\typeT}{\typeT'}\conf{\checkpointType{\typeT_1}}{\typeT_2} \confcomp \conf{\checkpointType{\typeU_1}}{\typeU_2}
%\typered\!\!\!\!\!\!\!\!\!/\ \ \ $, since no rule in Fig.~\ref{fig:typeSemantics_ext}
%can be applied. However, since $C$ is a reachable collaboration, 
%this type configuration is originated from 
%$\initConf{\typeT}{\typeT'}\conf{{\typeT}}{\typeT} \confcomp \conf{{\typeT'}}{\typeT'}$.
%By Def.~\ref{def:compliance}, $\typeT \compliant \typeT'$ implies 
%$\typeT_2=\typeU_2=\inactType$, which is a contradiction.
%Therefore, it holds that $S=S'$. Hence, by applying rule \rulelabel{TS-Com} we can 
%conclude.
%\item \rulelabel{F-Lab}, \rulelabel{E-Cmt$_1$} and \rulelabel{E-Cmt$_2$}.
%Similar to the previous case.
%\item \rulelabel{F-Str}. The use of $\congr$ leads us back to one of the other cases. 
%\item \rulelabel{F-Par}.
%In this case we have that
%$\logged{{\genSession}}{\checkpointType{P_1}} P_2
%\fwred 
%\logged{{\genSession}}{\checkpointType{P_1'}} P_2'$.
%Since this transition involves only one log term, it can be inferred only by applying rule \rulelabel{F-If},
%from which we have $P_2 \auxrel{\ite} P_2'$ and $\checkpointType{P_1'}=\checkpointType{P_1}$.
%By rule \rulelabel{P-IfT} (the case of rule \rulelabel{P-IfF} is similar), we have $P_2\subst{x}{\ce{s}}=
%\ifthenelseAct{e}{P_2'\subst{x}{\ce{s}}}{R}$ with $\expreval{e}{\ctrue}$.
%By rule \rulelabel{T-If} we get $\typeT_2=\typeT_2' \choiceType \typeV$
%and $\basis_2;\sorting_2 \judge P_2'\subst{x}{\ce{s}} \hasType x:\typeT_2'$.
%By rule \rulelabel{TS-If$_1$}, $\typeT_2 \typeTrans{\tau} \typeT_2'$.
%By applying rule \rulelabel{TS-Tau} we can conclude.
%\end{itemize}

\item $(\fwbwred \,=\, \bwred).$
From rule \rulelabel{B-Res}, we have 
$\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i}} P_i
\bwred 
\prod_{i\in I} \logged{{\genSession}}{\checkpointType{Q_i'}} P_i'$.
We prove the result by case analysis on the last rule applied in 
the inference of the above reduction.
%
%\begin{itemize}
%\item \rulelabel{B-Rll}. 
%In this case $P_2 \auxrel{\rollLab} P_2'$,
%$\checkpointType{P_1'}=\checkpointType{P_1}$,
%$\checkpointType{Q_1'}= Q_1$
%and $Q_2'=Q_1$.
%By rule \rulelabel{P-Rll}, we have $P_2\subst{x}{\ce{s}}=\roll$
%and $P_2'\subst{x}{\ce{s}}=\inact$. 
%By rule \rulelabel{T-Rll} we get $\typeT_2=\rollType$.
%By rule \rulelabel{TS-Rll}, $\typeT_2 \typeTrans{\rollType} \typeT_2'$,
%with $\typeT_2'=\inactType$.
%By rule \rulelabel{T-Inact}, we have 
%$\basis_2;\sorting_2 \judge P_2'\subst{x}{\ce{s}} \hasType x:\typeT_2'$.		
%Finally, by applying rule \rulelabel{TS-Rll$_1$} we can conclude.
%\item \rulelabel{B-Str} and \rulelabel{B-Par}. Similarly to the forward cases.
%\end{itemize}
\end{description}
\end{proof}

\begin{lemma}\label{lemma:typeCorrespondence_multi}
Let 
$
C= \mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I-\{n\}}\macceptAct{a}{i}{x}{P_i}
$,
with $I=\{1,..,n\}$,
such that
$C \hasType \{\ce{a}\mendpoint{\role{n}}:\typeV_n,\ldots,a\mendpoint{\role{1}}:\typeV_1\}$,
$\typeT_i=\typeV_i\cdot\role{i}$ for all $i\in I$,
and 
$\compliant(\typeT_n,\ldots,\typeT_1)$.
If $C \fwbwred^* \singleSession{s}{C}(\logged{\ce{\genSession}}{\imposed{R_1}} Q_1 
\ \mid \ \prod_{i\in\{2,..,n\}}\logged{\genSession}{\checkpointType{R_i}} Q_i)$
and $Q_1 \auxrel{\rollLab} Q_1'$, 
then there exist
$\{\typeU_i\}_{i\in I}$, $\{\typeU_i'\}_{i\in I}$ and $\typeU_1''$ such that
$\minitConf{\typeT_1,\ldots,\typeT_n}
\prod_{i\in I}
\conf{\typeT_i}{\typeT_i} 
\typered^*
\minitConf{\typeT_1,\ldots,\typeT_n}
\conf{\imposed{\typeU_1}}{\typeU_1'} 
\confcomp \prod_{i\in\{2,..,n\}} \conf{\checkpointType{\typeU_i}}{\typeU_i'}$
and 
$\typeU_1' \typeTrans{\rollType} \typeU_1''$.
\end{lemma}
\begin{proof}(Sketch)
As in Lemma~\ref{lemma:typeCorrespondence}'s proof, 
this result can be obtained by repeatedly applying Lemma~\ref{lemma:subj_multi}.
\end{proof}

\begin{lemma}\label{lemma:typeCorrespondenceCom_multi}
Let Let 
$
C= \mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in I-\{n\}}\macceptAct{a}{i}{x}{P_i}
$,
with $I=\{1,..,n\}$,
such that
$C \hasType \{\ce{a}\mendpoint{\role{n}}:\typeV_n,\ldots,a\mendpoint{\role{1}}:\typeV_1\}$,
$\typeT_i=\typeV_i\cdot\role{i}$ for all $i\in I$,
and 
$\compliant(\typeT_n,\ldots,\typeT_1)$.
%
If $C \fwbwred^* \singleSession{s}{C}\prod_{i\in I}\logged{\ce{\genSession}}{\checkpointType{Q_i}} P_i$,
$P_1 \auxrel{\actionLab} P_1'$ and
there is no $P_j$ with $j \in \{2,..,n\}$ such that 
$P_j \Barb{\bar{\actionLab}}$
with $\actionLab$ of the form 
$\send{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{v}$,
$\receive{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{x}$,
$\select{s\mendpoint{\role{p}}\mendpoint{\role{q}}}{l}$ or
$\branching{s\mendpoint{\role{p}}\mendpoint{\role{q}}}l$, 
then there exist
$\{\typeU_i\}_{i\in I}$, $\{\typeU_i'\}_{i\in I}$ and $\typeU_1''$ such that
$
\minitConf{\typeT_1,\ldots,\typeT_n}
\prod_{i\in I}
\conf{\typeT_i}{\typeT_i} 
\typered^*
\minitConf{\typeT_1,\ldots,\typeT_n}
\prod_{i\in I}
\conf{\checkpointType{\typeU_i}}{\typeU_i'} 
$
with
$\checkpointType{Q_i}$
in checkpoint accordance with $\checkpointType{\typeU_i}$,
$\typeU_1' \typeTrans{\mFunc{\sorting}{\actionLab}} \typeU_1''$, with
$\sorting$ sorting for typing $P_1'$,
and for all $\typeU_i''$ such that $\typeU_i' \typeTrans{\tau}^* \typeU_i''$
we have 
$\typeU_i'' \typeTrans{\overline{\mFunc{\sorting}{{\actionLab}}}}\!\!\!\!\!\!/\ $.
\end{lemma}
\begin{proof}(Skecth)
As in Lemma~\ref{lemma:typeCorrespondenceCom}'s proof, 
this result can be obtained by repeatedly applying Lemma~\ref{lemma:subj_multi}
and reasoning by case analysis on the rule for deriving the transition 
$P_1 \auxrel{\actionLab} P_1'$.
\end{proof}

\begin{theorem}\label{th:roll_soundness_multi}
If $C$ is a rollback safe collaboration, then $C\ {\fwbwred\!\!\!\!\!\!/\ }^*\ \collContext[\rollError]$.
\end{theorem}
\begin{proof}(Skecth) 
The proof proceeds by contradiction and relies on 
Lemma~\ref{lemma:typeCorrespondence_multi}.
\end{proof}


\begin{theorem}\label{th:com_soundness_multi}
If $C$ is a rollback safe collaboration, then $C\ {\fwbwred\!\!\!\!\!\!/\ }^*\ \collContext[\comError]$.
\end{theorem}
\begin{proof}(Skecth) 
The proof proceeds by contradiction and relies on 
Lemma~\ref{lemma:typeCorrespondenceCom_multi}.
\end{proof}



\theoremApp{\ref{th:deadlock_freedom_multi}}
Let $C=(\mrequestAct{a}{n}{x}{P_n}\, \mid \, \prod_{i\in \{1,..,n-1\}}\macceptAct{a}{i}{x}{P_i})$ be a \rollSafe\ collaboration.
If $C \!\fwbwred^*\! C'$ then either $C' \!\fwbwred\! C''$ for some $C''$ or 
$C' \congr \singleSession{s}{C}$ 
$\prod_{i\in \{1,..,n\}}
\logged{{\genSession}}{\checkpointType{Q_i}} \inact\, 
$ for some $\checkpointType{Q_1}, \ldots,\checkpointType{Q_n}$.
\begin{proof} 
The proof proceeds by contradiction.
Suppose that $C$ is rollback safe and 
$C \fwbwred^* C'$ with $C' \fwbwred\!\!\!\!\!\!/\ \ $ and 
$C' \congr\!\!\!\!\!/\ \  
\singleSession{s}{C}$ 
$\prod_{i\in \{1,..,n\}}
\logged{{\genSession}}{\checkpointType{Q_i}} \inact\, 
$
for any $Q_1, \ldots,Q_n$.
The only situations that prevents $C'$ from progressing 
are $C'= \collContext[\rollError]$ and $C'= \collContext[\comError]$. 
However, from Theorems~\ref{th:roll_soundness_multi} and~\ref{th:com_soundness_multi}, respectively, 
we have $C'\neq \collContext[\rollError]$ and $C'\neq \collContext[\comError]$, 
which is a contradiction.  
\end{proof}




==> tex/proofs_reversibility_results.tex <==
% !TEX root = ../main.tex

\subsection{Reversibility results}



\label{reversibility_proofs}



\bigskip


Any reachable collaboration is also a \textit{forward only} reachable collaboration. Formally:

\theoremApp{\ref{th:trace}}
Let $C_0$ be an initial collaboration. If $C_0 \fwbwred^{*}C_1$ then $C_0 \fwred^{*}C_1$.
\begin{proof}
By induction on the number $n$ of backward reductions contained into $C_0 \fwbwred^{*}C_1$.
 The base case
($n=0$)
trivially holds. In the inductive case, let us take the backward reduction which is the
nearest to $C_0$. That is:
$$C_0 \fwred^{*} C' \bwred C''\fwbwred^{*}C_1$$
Depending whether it is an $\abt$ or a $\rll$ we can apply respectively Lemma~\ref{lemma:init}
or Lemma~\ref{lemma:fw_trace} to obtain a forward trace of the form
$$C_0 \fwred^{*} C''\fwbwred^{*}C_1$$
and we can conclude by applying the inductive hypothesis on  the obtained trace which contains
less backward moves with respect to the original one.
\end{proof}


\lemmaApp{\ref{lemma:safe_roll}}
Let $C_1$ and $C_2$ be two reachable collaborations. 
$C_1 \bwred C_2$ then $C_2 \fwred^{*} C_1$.
\begin{proof}
Since $C_1$ is a reachable collaboration, we have that there exists an initial collaboration $C_0$
such that $C_0\fwbwred^{*}C_1$.
By applying Theorem~\ref{th:trace} we can rearrange the trace 
such that it contains just forward transitions as follows
$$C_0\fwred^{*} C_1$$
%
If the backward reduction is obtained by applying \rulelabel{B-Abt},
by Lemma~\ref{lemma:init} we have $C_2\congr C_0$, from which the thesis trivially follows.
Instead, if the backward reduction is obtained by applying \rulelabel{B-Rll},
we proceed by case analysis depending on the presence of commit reductions in the trace.
If they are present, we select the last of such commit, that is we can decompose the trace in the following way:
$$C_0 \fwred^{*}\ \cmt C_{cmt} \fwred^{*}C_1\rll C_2$$
and by applying Lemma~\ref{lemma:fw_trace} we have that $C_2 \fwred^{*}\congr C_1$ as desired.

In the case there is no commit in the trace, 
%we have to distinguish two cases: 
%either \rulelabel{B-Abt} or \rulelabel{B-Rll}
%is applied.
without losing of generality we can assume
\begin{align*}
 &C_0\congr 		\requestAct{a}{x_1}{P_1} \mid \acceptAct{a}{x_2}{P_2} \mid C^{\circ}
\\
 & C_0 \fwred
 \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2)\mid C^{\circ}
\end{align*}
%In the first case we have that $C_2 \congr C_0$ and the thesis trivially follows; in the second case
%we have $C_2 \congr \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2)$
%and we can conclude by noticing that $C_0\fwred C_2$.
By rule \rulelabel{B-Rll}, $C_2 \congr \singleSession{s}{C_0}(\logged{\genSession}{P_2} P_2 \mid \logged{\genSession}{Q_2} Q_2) \mid C^{\circ}$. Thus, we can conclude by noticing that $C_0\fwred C_2$
must be the first reduction in $C_0\fwred^{*} C_1$.
\end{proof}


\lemmaApp{\ref{lemma:determinism}}
%Let C be a reachable collaboration. If $C\bwred C'$ and $C\bwred C''$ then $C' \congr C''$
Let $C$ be a reachable collaboration. If $C\rlls{s} C'$ and $C\rlls{s} C''$ then $C' \congr C''$.
\begin{proof}
Since $C$ is a reachable collaboration, it is has been generated by an initial collaboration
$C_0$ of the form $C_0 = \requestAct{a}{x}{P_1}   \mid \acceptAct{a}{x}{P_2}$, 
and by Theorem~\ref{th:trace} we have that
$C_0 \fwred^{*} C$. We distinguish two cases, whether in the trace
there has been at least one commit or not. In the first case, we can decompose the trace in such a way
to single out the last commit as follows:
$$C_0 \fwred^{*}C_{cmt} \fwred^{*} C$$
so that in the reduction $C_{cmt} \fwred^{*} C$ there is no commit. 
If from $C$ the rollbacks $C\rll C'$ and $C\rll C''$ are triggered by the same process, 
the thesis trivially follows.
In the other case, we have that:
$$C_{cmt} \congr 	\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_2 \mid \logged{\genSession}{Q_1} Q_2) \mid C^{\circ}
$$
with both $P_2$ and $Q_2$ are able to trigger a rollback. If the roll action is executed by $P_2$ we have that
$$\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_2 \mid \logged{\genSession}{Q_1} Q_2)\mid C^{\circ} \rll 
	\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_1 \mid \logged{\genSession}{Q_1} Q_1) \mid C^{\circ}= C'$$
If the roll is triggered by $Q_2$ we have that
$$	\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_2 \mid \logged{\genSession}{Q_1} Q_2) \mid C^{\circ} \rll 
	\singleSession{s}{C_0}(\logged{\genSession}{P_1} P_1 \mid \logged{\genSession}{Q_1} Q_1) \mid C^{\circ} = C''
	$$
And we can conclude by noticing that $C' \equiv C''$, as desired.
\end{proof}

\theoremApp{\ref{lemma:undoability}}
Let C be a reachable collaboration. 
If $C \cmt C'$ then there exists no $C''$ such that
$C' \fwred^{*}\rll C''$ and $C'' \fwred^{+} C$.
\begin{proof}
We proceed by contradiction. Suppose that there exists $C''$ such that 
$C' \fwred^{*}\rll C''$ and $C'' \fwred^{+} C$.
Since $C$ is a reachable collaboration, thanks to Theorem~\ref{th:trace}
we have that there exists an initial collaboration $C_0$ 
such that $C_0\fwred^{*}C\cmt C'$. Since a rollback brings back the 
collaboration to a point before a commit, this means it has been restored a commit 
previous to the last one (by \rulelabel{B-Rll}, indeed, only processes stored in logs 
can be committed). 
This implies that there exist at least two different commits in the trace
such that
$$C_0 \fwred^{*}C_{cmt}\fwred^{*}C \cmt C'\fwred^{*}\rll C''$$
%
with $C'' = C_{cmt}$. We have that $C''\fwred^{+} C \cmt C'\fwred^{*}C_{rl}$, 
where $C_{rl}$ is the collaboration that perform the roll reduction.
Now since the last commit has been done by $C$, supposing that the commit is triggered by
$P_c$, which evolves to $P'_c$ in doing that,  we have that:
\begin{align*}
%&C\cmt C' \text{ with }\\
&C \congr 	\singleSession{s}{C_0}(\logged{\genSession}{P} P_c \mid \logged{\genSession}{Q} Q_c) 
\;\text{ and }\; C'= \singleSession{s}{C_0}(\logged{\genSession}{P'_c} P'_c \mid \logged{\genSession}{Q_c} Q_c)
\end{align*}
Now, by hypothesis we have that $C'\fwred^{*} C_{rl}$ without any commit being present in the trace, hence:
$$C_{rl} \congr 	\singleSession{s}{C_0}(\logged{\genSession}{P'_c} P_{rl} \mid \logged{\genSession}{Q_c} Q_{rl}) $$
By hypothesis, from $C_{rl}$ a rollback is possible. 
Regardless the rollback is triggered by $P_{rl}$ or  $Q_{rl}$, we have that
$C_{rl} \rll C'$. Now, from $C'$ we cannot reach $C$ ($C'\ \fwred^{+}\!\!\!\!\!\!\!\!\!\!/\ \ \ \  C$), 
as $C'$ is derived from $C$ and the rollback can only bring the collaboration back to $C'$. 
This violates the hypothesis, and hence we conclude. 
\end{proof}



==> tex/singleSession.tex <==
% !TEX root = ../checkpoint-based rollback recovery in session-based pi-calculus.tex
\section{Binary Single Session Calculus with checkpoint-based primitives}

\begin{figure}[t]
\centering
\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ \ \ \ }l@{}}
	$P$ & ::= & $\ldots$ & \textbf{Checkpointed Processes} \\
	& $\mid$ &  $\singleSession{s}{P_1}\ P_2$ 
	\quad $\mid$ \quad $\logged{\genSession}{P_1}P_2$ 
	& \quad single session, log\\
	& $\mid$ &  $\commitAct{P}$
	\quad $\mid$ \quad $\roll$
	\quad $\mid$ \quad $\abort$  & \quad log, commit, roll, abort\\
	\\[-.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Binary single session calculus with checkpoints: syntax}
	\label{fig:syntax_pi_ext}
\end{figure}

We consider the extension of the binary session calculus with checkpoint-based primitives 
for committing, rolling back and aborting sessions. The extended syntax is reported in 
Figure~\ref{fig:syntax_pi_ext}.
%
The term \mbox{$\singleSession{s}{P_1}\ P_2$ } represents a \emph{single session} along the channel $s$ 
with associated starting checkpoint $P_1$ (corresponding to the term that initialised the session)
and code $P_2$. 
The term \mbox{$\logged{\genSession}{P_1}P_2$} represents a log, identified by the session endpoint
$\genSession$, storing the checkpoint $P_1$, and associated to the code $P_2$.
Terms \mbox{$\singleSession{s}{P_1}\ P_2$ } and \mbox{$\logged{\genSession}{P_1}P_2$}  are binders, i.e. they bind session channel $s$ and session endpoint $\genSession$, respectively, in $P_2$.
In this respect, they act similarly to operator $\res s P$, but their scope cannot be extended 
in order to avoid involving processes that do not belong to the session in the rollback effect.

Not all processes allowed by the syntax corresponds to meaningful
processes in the reversible single sessions setting. 
Indeed, on the one hand, the syntax allows terms violating the single sessions 
limitation. 
On the other hand, in a general term of the calculus the processes stored in logs 
may not be consistent with the computation that has taken place.
%
We address these issues by only considering a class of well-formed processes, called 
\emph{reachable} processes. In the definition of this class of processes, 
to ensure the use of single sessions only, as in \cite{HYCJACM15} we resort to 
the notion of \emph{simple} process. 
\begin{definition}[Simple binary process]\label{def:simple}
A process is \emph{simple} if (i)~it is generated by the grammar in Figure~\ref{fig:syntax_pi} and
(ii)~it is typable with a type derivation using prefix rules
where the session typings in the premise and the conclusion are restricted to at most a 
singleton\footnote{Using the standard typing system for the binary session \pic\ 
\iftr
(Figure~\ref{fig:typingSysytem} in Appendix~\ref{app:background}), 
\else
(see \cite[Figure~13]{RC_TR}), 
\fi
point (ii) boils down to:  $\typing$ of rules 
\rulelabel{Req}, 
\rulelabel{Acc},
\rulelabel{Send},
\rulelabel{Rcv},
\rulelabel{Sel}
and \rulelabel{Br} are empty; 
neither \rulelabel{Thr} nor \rulelabel{Cat} is used;
$\typing\comp \typing'$ in \rulelabel{Conc} contains at most a singleton; 
and $\typing$ of the remaining rules contain at most a singleton.}. 
\end{definition}
The point (i) of the above definition states that a simple process has no log, while 
point (ii) states that each prefixed subterm in a simple process uses only a single session. 
Notably, in a simple process, delegation and subordinate sessions 
(i.e., new sessions initialised within the single session) are disallowed.

Now, to ensure history consistency, as in~\cite{CristescuKV13} we only consider \emph{reachable} 
processes, i.e. processes obtained by means of forward reductions from simple processes. 

\begin{definition}[Reachable binary processes]\label{def:reachable}
The set of \emph{reachable} binary processes is the closure under relation $\fwred$ (see below)  
of the set of simple processes. 
\end{definition}

In the extended calculus,  processes can perform, besides standard 
\emph{forward computations}, also  \emph{backward computations} 
that restore the last committed checkpoints, thus undoing the effect of 
the forward computations. 
%
As usual, the operational semantics is given in terms of a structural congruence and 
a reduction relation. The laws defining the structural congruence 
are the same of the binary session calculus.
Instead, the \emph{reduction} relation, written $\fwbwred$, 
is given as the union of the corresponding \emph{forward reduction} relation $\fwred$ and \emph{backward reduction} relations $\bwred$.
%
The semantics is only defined for closed, reachable terms, 
where now the definition of \emph{closed} term extends to session endpoints, 
in the sense that all occurrences of an endpoint $\genSession$
have to be bound by a log term $\logged{\genSession}{\cdot}\cdot$. 
%This latter requirement is needed for ensuring that
%every running session in the considered process can be reverted; 
%for example, in the reachable process $(\send{\ce{s}}{1}\mid\receive{s}{x} \mid Q)$
%there is a running session $s$ that cannot be reverted because no computation history 
%information (i.e., no log) is available for it. 


The definition of the forward reduction relation $\fwred$ over checkpointed processes relies on an auxiliary labelled relation $\auxrel{\actionLab}$ over \pic\ processes that specifies \emph{commitments}, i.e. the actions that processes can initially perform and the continuation process obtained after each such action. The operational rules defining such auxiliary relation are reported in Figure~\ref{fig:semantics_pi_ext_aux}, 
where action label $\actionLab$ stands for either 
%$\requestPrefix{u}{x}$,
%$\acceptPrefix{u}{x}$,
%$\send{\sessId}{e}$,
%$\receive{\sessId}{x}$,
%$\select{\sessId}{l}$,
%$\branching{\sessId}l$, 
$\send{k}{v}$,
$\receive{k}{x}$,
$\select{k}{l}$,
$\branching{k}l$, 
$\commitLab$,
$\rollLab$,
$\abortLab$,
or $\ite$.
%
The meaning of these rules is straightforward, as they just produce as labels the actions currently 
enabled in the process. In doing that, expressions of sending actions and conditional choices are 
evaluated. Notably, since we are considering the single session setting, connecting actions, 
i.e. request and accept, are dealt with as the inaction. 

\begin{figure*}[t]
	\centering
	\small
	\begin{tabular}{l@{\qquad}l@{\qquad }l}
	$\sendAct{k}{e}{P} \auxrel{\send{k}{v}} P$
	& $\expreval{e}{v}$ & \rulelabel{Snd}
	\\[.2cm]	
	$\receiveAct{k}{x}{P} \auxrel{\receive{k}{x}} P$
	&  & \rulelabel{Rec}
	\\[.2cm]
	$\selectAct{{k}}{l}{P} \auxrel{\select{k}{l}} P$
	&  & \rulelabel{Sel}
	\\[.2cm]	
	$\branchAct{k}{\branch{l_1}{P_1}  \branchSep \ldots \branchSep \branch{l_n}{P_n}}
	\auxrel{\branching{k}l_i} P_i$
	& $1 \leq i \leq n$ & \rulelabel{Brn}
	\\[.2cm]
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_1$
	& $\expreval{e}{\ctrue}$ & \rulelabel{IfT}
	\\[.2cm]
	$\ifthenelseAct{e}{P_1}{P_2} \auxrel{\ite} P_2$ 
	& $\expreval{e}{\cfalse}$ & \rulelabel{IfF}
	\\[.2cm]
	$\commitAct{P} \auxrel{\commitLab} P$ 
	&  & \rulelabel{Cmt}
	\\[.2cm]	
	$\roll \auxrel{\rollLab} \inact$ 
	&  & \rulelabel{Rll}
	\\[.2cm]	
	$\abort \auxrel{\commitLab} \inact$ 
	&  & \rulelabel{Abt}
	\\[.1cm]
	\end{tabular}
	\begin{tabular}{c}
	$
	\infer[$\,\rulelabel{Par}$]{P_1 \!\mid\! P_2 \ \auxrel{\actionLab}\ P_1' \!\mid\! P_2}
	{P_1 \ \auxrel{\actionLab}\ P_1'}
	$	
	\qquad
	$
	\infer[$\,\rulelabel{Res}$]{\res{c}P \ \auxrel{\actionLab}\ \res{c}P'}
	{P \ \auxrel{\actionLab}\ P'}
	$
	\qquad
	$
	\infer[$\,\rulelabel{Str}$]{P_1 \ \auxrel{\actionLab}\ P_2}
	{P_1 \congr P_1'\ \auxrel{\actionLab}\ P_2' \congr P_2}
	$
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.4cm}	
	\caption{Binary single session calculus with checkpoints: auxiliary commitment relation}
	\label{fig:semantics_pi_ext_aux}
\end{figure*}

Now, the operational rules defining the reduction relation $\fwbwred$
are reported in Figure~\ref{fig:semantics_pi_ext}. 
We comment on salient points.
%
Once a session is created, the initial configuration is stored in the single
session construct (rule \rulelabel{F-Con}).
Conditional choices taken outside sessions are not revertible, 
as they are not subject to checkpointing  (rules \rulelabel{F-IfT} and \rulelabel{F-IfF}).
Communication, branching selection and internal conditional choices proceed as usual, without affecting 
logs (rules \rulelabel{F-Com}, \rulelabel{F-Lab} and \rulelabel{F-If}).  
A commit action updates the checkpoint of a session, by replacing the processes stored in the logs of the two involved parties (rule \rulelabel{F-Cmt}). 
Reversely, a rollback action restores the processes in the two logs (rule \rulelabel{B-Rll}). 
The abort action, instead, restores the initial configuration stored in the single session 
construct (rule \rulelabel{B-Abt}). Finally, the other rules simply extend the standard parallel, 
restriction, structural congruence rules to forward and backward relations. 

\begin{figure*}[p]
	\centering
	\small
	\begin{tabular}{l@{\hspace*{-4cm}}l@{\qquad }l}
	$P$
	$\ \fwred\ $
	$\singleSession{s}{P}\ 
	(\logged{\ce{s}}{P_1\subst{\ce{s}}{x_1} }	P_1\subst{\ce{s}}{x_1}$ 
        & $P=(\requestAct{a}{x_1}{P_1}\ \mid \ \acceptAct{a}{x_2}{P_2})$ & \rulelabel{F-Con}
        \\
        \qquad\qquad\qquad\quad
        $\mid\ 
	\logged{s}{P_2\subst{s}{x_2}}	P_2\subst{s}{x_2} )$ 
	\\[.4cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \fwred\ $
	$P_1$
	& $\expreval{e}{\ctrue}$ & \rulelabel{F-IfT}
	\\[.2cm]
	$\ifthenelseAct{e}{P_1}{P_2}$
	$\ \fwred\ $
	$P_2$
	& $\expreval{e}{\cfalse}$ & \rulelabel{F-IfF}
	\\[.3cm]	
	$\logged{\ce{\genSession}}{Q_1} \sendAct{\ce{\genSession}}{e}{P_1} 
	\ \mid \ 
	\logged{\genSession}{Q_2} \receiveAct{\genSession}{x}{P_2}$
	$\ \fwred\ $
	$\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2\subst{v}{x}$
	\quad $\expreval{e}{v}$
	&  & \rulelabel{F-Com}
	\\[.2cm]
	$
	\infer[$\,\rulelabel{F-Com}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \fwred\ 
	\logged{\ce{\genSession}}{Q_1} P_1' 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2'\subst{v}{x}	
	}
	{
	P_1 \auxrel{\send{\ce{k}}{v}} P_1'
	\qquad
	P_2 \auxrel{\receive{k}{x}} P_2'	
	}
	$	
       &  & 
		\\[.3cm]
	$
	\infer[$\,\rulelabel{F-Lab}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \fwred\ 
	\logged{\ce{\genSession}}{Q_1} P_1' 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2'
	}
	{
	P_1 \auxrel{\select{\ce{k}}{l}} P_1'
	\qquad
	P_2 \auxrel{\branching{k}l} P_2'	
	}
	$	
       &  & 
		\\[.3cm]		
	$
	\infer[$\,\rulelabel{F-Cmt}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \fwred\ 
	\logged{\ce{\genSession}}{P_1'} P_1' 
	\ \mid \ 
	\logged{\genSession}{P_2} P_2
	}
	{
	P_1 \auxrel{\commitLab} P_1'
	}
	$	
       &  & 
		\\[.3cm]					
	\end{tabular}
	\begin{tabular}{l}
		$
	\infer[$\,\rulelabel{F-If}$]{
	\logged{\genSession}{Q} P
	\ \fwred\ 
	\logged{\genSession}{Q} P' 
	}
	{
	P \auxrel{\ite} P'
	}
	$	
\qquad\qquad\qquad\qquad
	$
	\infer[$\,\rulelabel{F-Par}$]{P_1 \!\mid\! P_2 \ \fwred\ P_1' \!\mid\! P_2}
	{P_1 \ \fwred\ P_1'}
	$	
	\\[.4cm]	
	$
	\infer[$\,\rulelabel{F-Res1}$]{\res{c}P \ \fwred\ \res{c}P'}
	{P \ \fwred\ P'}
	$
\qquad\qquad\qquad\qquad
	$
	\infer[$\,\rulelabel{F-Res2}$]{\singleSession{s}{Q}P \ \fwred\ \singleSession{s}{Q}P'}
	{P \ \fwred\ P'}
	$
	\\[.4cm]	
	$
	\infer[$\,\rulelabel{F-Str}$]{P_1 \ \fwred\ P_2}
	{P_1 \congr P_1'\ \fwred\ P_2' \congr P_2}
	$
	\\[.1cm]
	\end{tabular}
	%%%% BACKWARD RULES
	\begin{tabular}{l}
	$
	\infer[$\,\rulelabel{B-Rll}$]{
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2
	\ \bwred\ 
	\logged{\ce{\genSession}}{Q_1} Q_1
	\ \mid \ 
	\logged{\genSession}{Q_2} Q_2
	}
	{
	P_1 \auxrel{\rollLab} P_1'
	}
	$	
		\\[.4cm]				
	$
	\infer[$\,\rulelabel{B-Abt}$]{
	\singleSession{s}{P}(
	\logged{\ce{\genSession}}{Q_1} P_1 
	\ \mid \ 
	\logged{\genSession}{Q_2} P_2)
	\ \bwred\ P
	}
	{
	P_1 \auxrel{\abortLab} P_1'
	}
	$	
	\\[.3cm]
	\end{tabular}	
	\begin{tabular}{c@{\qquad\qquad\qquad}c}		
		$
	\infer[$\,\rulelabel{B-Par}$]{P_1 \!\mid\! P_2 \ \bwred\ P_1' \!\mid\! P_2}
	{P_1 \ \bwred\ P_1'}
	$	
	&
	$
	\infer[$\,\rulelabel{B-Res1}$]{\res{c}P \ \bwred\ \res{c}P'}
	{P \ \bwred\ P'}
	$
	\\[.4cm]	
	$
	\infer[$\,\rulelabel{B-Res2}$]{\singleSession{s}{Q}P \ \bwred\ \singleSession{s}{Q}P'}
	{P \ \bwred\ P'}
	$
	&
	$
	\infer[$\,\rulelabel{B-Str}$]{P_1 \ \bwred\ P_2}
	{P_1 \congr P_1'\ \bwred\ P_2' \congr P_2}
	$
	\\[.1cm]
	\hline
	\end{tabular}	
	\vspace*{-.2cm}	
	\caption{Binary single session calculus with checkpoints: forward and backward reduction relations }
	\label{fig:semantics_pi_ext}
\end{figure*}



\bigskip

The operational semantics provides a description of the low-level implementation of the 
primitives for programming a checkpoint-based rollback recovery in a session-based language. 
However, it does not guarantee high-level properties about the correct execution of 
the rollback. As mentioned in Section~\ref{sec:intro}, in our approach a party executing a 
rollback action expects that it is restored the last checkpoint she has committed, not one committed 
by the other session party. The undesired situation is instead allowed by the semantics, as illustrated by the following example. 

\begin{example}\label{example}
Let us consider a client/server scenario where the server offers a service with two different quality levels, H and L: 
$$
\begin{array}{lcl}
S & = & \acceptPrefix{a}{y}.\
\branchAct{y}{
\branch{l_H}{\commitAct{\receiveAct{y}{z}{\sendAct{y}{e_H(z)}{P_H}}}} 
\ \branchSep \\
& & \qquad\qquad\ \
\branch{l_L}{\commitAct{\receiveAct{y}{z}{\sendAct{y}{e_L(z)}{P_L}}}}}
\\
\\
C & = & \requestPrefix{a}{x}.\ \commitAct{}\ \ifPi\ (e)\ \thenPi\ \selectAct{{x}}{l_H}{\sendAct{x}{v}{}}
\ifPi\ (e')\ \thenPi\ \receiveAct{x}{w}{Q_H}\ \elsePi\ \roll\\
&& \qquad\qquad\qquad\qquad\quad\ \
\elsePi\ \selectAct{{x}}{l_L}{\sendAct{x}{v}{}}
\ifPi\ (e'')\ \thenPi\ \receiveAct{x}{w}{Q_L}\ \elsePi\ \roll
\end{array}
$$
After the client selection, the server commits. After sending the service request data (value $v$), 
the client decides whether proceedings on the session or rolling back to the beginning of the session 
to possibly change the service quality. However, when the client activate the rollback, she is not able 
to go back to the beginning of the session, because the rollback effect is blocked by the 
server's commit as shown in Figure~\ref{fig:scenario}.
\begin{figure}[t]
\centering
\includegraphics[scale=.4]{img/scenario}
\vspace*{-.4cm}
\caption{Undesired rollback recovery scenario}
\label{fig:scenario}
\end{figure}
\end{example}


\subsection{Rollback compliance relation}
To prevent undesired rollback recovery situations, like the one described in Example~\ref{example}, we propose the use of compliance checking, to be performed at design time before actually executing the system. This check is not done on the full system specification, but only at the more abstract level of session types. 

\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{@{}r@{\ }c@{\ }l@{\ \ \quad }l@{}}
	$\alpha$ & ::= & \ldots &  \textbf{Types}\\
	& $\mid$ & $\commitType.\alpha$ 
	\ \  $\mid$ \ \ $\rollType$
	& \quad commit, roll
	\\
	\\
	$C$ & ::= & $\conf{\checkpointType{\alpha}_1}{\alpha_2} \confcomp \conf{\checkpointType{\alpha}_3}{\alpha_4}$  &  \textbf{Configurations}\\
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Binary single session calculus with checkpoints: type syntax}
	\label{fig:typeSyntax_ext}
	\vspace*{-.2cm}
\end{figure}

The standard binary session types are here extended as shown in Figure~\ref{fig:typeSyntax_ext}.
%
To check compliance between two parties, we consider a \emph{configuration} consisting in the parallel composition of two pairs $\conf{\checkpointType{\alpha}_1}{\alpha_2}$, where $\alpha_2$ is the session type of a participant and $\checkpointType{\alpha}_1$ is the type of the party's checkpoint. 
We use $\checkpointType{\alpha}$ to denote either a type $\alpha$, representing a checkpoint committed by 
the party, or $\imposed{\alpha}$, representing a checkpoint imposed by the other party of the session. 

\todo[inline]{FT: here there is some technicalities concerning types to be fixed. In particular,
in this context we should relax the duality between types used in \cite{YoshidaV07},
as we rely indeed in a compliance relation. In particular, we should revise the typing of 
if-then-else (perhaps using a choice operator at type level). }


Their semantics, necessary for the definition of the compliance relation, is given in Figure~\ref{fig:typeSemantics_ext}, where label $\typeLab$ stands for either 
$\outType{S}$,
$\inpType{S}$,
$\selTypeLabel{l}$,
$\branchTypeLabel{l}$,
$\commitType$,
or $\rollType$.
The only relevant rules are those for commit and roll synchronisations. 
In the former case, the checkpoints of both parties are updated, but the one 
of the passive party (i.e., the party that has not performed the commit action) 
is marked as `imposed'. In the latter case, the rollback (i.e., the reduction step)
is allowed only when the active party (i.e., the party that has performed the rollback 
action) has a non-imposed checkpoint and the passive party has an imposed checkpoint;
in all other cases, the configuration cannot proceed with the rollback.

\begin{figure}[t]
	\centering
	\small
	\begin{tabular}{l@{\qquad\qquad\qquad}l}
	$\outType{S}.\alpha \typeTrans{\outType{S}} \alpha$
	&
	$\inpType{S}.\alpha \typeTrans{\inpType{S}} \alpha$  
	\\
	\\
	\multicolumn{2}{l}{
	$\selType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}
	\typeTrans{\selTypeLabel{l_i}} \alpha_i$ \qquad $1 \leq i \leq n$
	}\\
	\\
	\multicolumn{2}{l}{
	$\branchType{\branch{l_1}{\alpha_1}, \ldots, \branch{l_n}{\alpha_n}}
	\typeTrans{\branchTypeLabel{l_i}} \alpha_i$ \qquad $1 \leq i \leq n$
	}\\
	\\
	$\commitType.\alpha \typeTrans{\commitType} \alpha$ 
	&
	$\rollType \typeTrans{\rollType} \inactType$
	\\
	\\
	$
	\infer[]
	{\recType{t}.\alpha \typeTrans{\typeLab} \alpha'}
	{\alpha\subst{\recType{t}.\alpha}{t} \typeTrans{\typeLab} \alpha'}
	$	
	\\
	\\
	\multicolumn{2}{l}{
	$
	\infer[]
	{\conf{\checkpointType{\beta}_1}{\alpha_1} \confcomp \conf{\checkpointType{\beta}_2}{\alpha_2}
	\typered
	\conf{\checkpointType{\beta}_1}{\alpha_1'} \confcomp \conf{\checkpointType{\beta}_2}{\alpha_2'}}
	{\alpha_1 \typeTrans{\outType{S}} \alpha_1'
	\qquad\qquad
	 \alpha_2 \typeTrans{\inpType{S}} \alpha_2'}
	$	
	}\\
	\\
        \multicolumn{2}{l}{
	$
	\infer[]
	{\conf{\checkpointType{\beta}_1}{\alpha_1} \confcomp \conf{\checkpointType{\beta}_2}{\alpha_2}
	\typered
	\conf{\checkpointType{\beta}_1}{\alpha_1'} \confcomp \conf{\checkpointType{\beta}_2}{\alpha_2'}}
	{\alpha_1 \typeTrans{\selTypeLabel{l}} \alpha_1'
	\qquad\qquad
	 \alpha_2 \typeTrans{\branchTypeLabel{l}} \alpha_2'}
	$	
	}\\
	\\
        \multicolumn{2}{l}{
	$
	\infer[]
	{\conf{\checkpointType{\beta}_1}{\alpha_1} \confcomp \conf{\checkpointType{\beta}_2}{\alpha_2}
	\typered
	\conf{\alpha_1'}{\alpha_1'} \confcomp \conf{\imposed{\alpha_2}}{\alpha_2}}
	{\alpha_1 \typeTrans{\commitType} \alpha_1'}
	$	
	}\\
	\\
        \multicolumn{2}{l}{
	$
	\infer[]
	{\conf{\beta_1}{\alpha_1} \confcomp \conf{\imposed{\beta}_2}{\alpha_2}
	\typered
	\conf{\beta_1}{\beta_1} \confcomp \conf{\imposed{\beta_2}}{\beta_2}}
	{\alpha_1 \typeTrans{\rollType} \alpha_1'}
	$	
	}
	\\[.1cm]
	\hline
	\end{tabular}
	\vspace*{-.3cm}	
	\caption{Binary single session calculus with checkpoints: type semantics (symmetric rules for configurations are omitted)}
	\label{fig:typeSemantics_ext}
	\vspace*{-.2cm}
\end{figure}

We can now define the compliance relation.
\begin{definition}[Compliance]
Two types $\alpha_1$ and $\alpha_2$ are \emph{compliant}, written 
$\alpha_1 \compliant \alpha_2$, if  
$\conf{\alpha_1}{\alpha_1} \compliant \conf{\alpha_2}{\alpha_2}$.
Relation $\compliant$ on configurations is defined as follows:\\
$\conf{\beta_1}{\alpha_1} \compliant \conf{\beta_2}{\alpha_2}$
whenever 
$\conf{\beta_1}{\alpha_1} \confcomp \conf{\beta_2}{\alpha_2}
\typered^*$
$\conf{\beta_1'}{\alpha_1'} \confcomp \conf{\beta_2'}{\alpha_2'}
\typered\!\!\!\!\!\!\!\!/$
implies $\alpha_1'=\alpha_2'=\inactType$.
\end{definition}


\begin{example}
Let us consider again the scenario described in Example~\ref{example}. 
As expected, the types of the two parties are not compliant, because 
their configuration can evolve to
$
\conf{\imposed{\alpha}}{\rollType} \confcomp \conf{\beta}{\outType{\mathsf{int}}.\beta'}
$,
which is deadlocked and not in a final state. 
\end{example}





